The Validity of Evaluation Results: Assessing Concurrence Across Compositionality Benchmarks

NLP models have progressed drastically in recent years, according to numerous datasets proposed to evaluate performance. Questions remain, however, about how particular dataset design choices may impact the conclusions we draw about model capabilities. In this work, we investigate this question in the domain of compositional generalization. We examine the performance of six modeling approaches across 4 datasets, split according to 8 compositional splitting strategies, ranking models by 18 compositional generalization splits in total. Our results show that: i) the datasets, although all designed to evaluate compositional generalization, rank modeling approaches differently; ii) datasets generated by humans align better with each other than they with synthetic datasets, or than synthetic datasets among themselves; iii) generally, whether datasets are sampled from the same source is more predictive of the resulting model ranking than whether they maintain the same interpretation of compositionality; and iv) which lexical items are used in the data can strongly impact conclusions. Overall, our results demonstrate that much work remains to be done when it comes to assessing whether popular evaluation datasets measure what they intend to measure, and suggest that elucidating more rigorous standards for establishing the validity of evaluation sets could benefit the field.

==> CompositionalitySub_arXiv/1_Introduction.tex <==

\input{figures/default_conf_matrix}

Over the past few years, NLP has made astonishing progress on almost all language-related tasks proposed by the community. %
Concurrently, %
a plethora of benchmark datasets has emerged for evaluating the skills of NLP models and exposing their strengths and weaknesses (\citealt{chowdhery-etal-2022-scaling}, \textit{inter alia}).
These datasets focus on a variety of different aspects of model capabilities, that are increasingly not mutually exclusive: oftentimes, multiple benchmarks are available that target the same capability or skill, using (slightly) different metrics, design choices, and/or conceptual approaches. 
For instance, \citet{Hupkes2023} report that many recent studies on generalization  used  different \emph{shift sources} to study the same types of \emph{generalization} (see \cref{fig:generalisation_vs_source}).\footnote{Plot generated using the visualisation tool on \url{https://genbench.org/visualisations}.} 

However, somewhat surprisingly, despite a wealth of work in the domain of evaluation and generalization, there is very little research that assesses whether multiple datasets designed to measure the same ability also yield the same conclusions.
This makes it difficult for practitioners to conduct informed evaluation dataset selection and, perhaps even more concerning, impedes our understanding of how well different datasets measure what they intend to measure.
While establishing \emph{construct validity} and \emph{construct reliability} -- for instance through comparing the results of tests with other tests that intend to measure the same thing -- is common practice in the social sciences \citep{westen2003quantifying, jacobs-wallach-2021-measurement}, it is not the standard in the field of NLP.

In this work, we argue that establishing such standards is much needed in our field, and we present a detailed set of experiments that assesses construct validity in the domain of \emph{compositional generalization}. 
Following \citet{liu2021question}, we use \emph{concurrence} to measure the extent to which 8 different \emph{compositional splitting strategies} for 4 different datasets -- SCAN, GeoQuery, COGS, and Spider -- %
provide similar rankings for 6 different modeling approaches -- BART, T5, Transformer, uni- and biLSTMS, and Neural-BTG.
We find that, in general, the conclusions drawn from one dataset split typically do not align with the results from another dataset split.
In a range of experiments, we explore if that could be attributed to whether the underlying data are synthetic or human-generated, to the compositional splitting strategy is used to create the data (a.k.a.\ what interpretation of compositionality), or to uncontrolled exposure to lexical items that also occurred during pretraining.

We find that concurrence values are generally low: only 10 out of 153 pairs of dataset splits have a concurrence value that surpasses the threshold for high concurrence.
Furthermore, results from human-authored datasets concur much more than results from synthetic datasets.
On the contrary, dataset splits that share the same interpretation of compositionality -- as defined by their splitting strategy -- hardly concur with each other:  the underlying data plays a more important role in model rankings.
Lastly, aligned with the findings of \citet{kim2022uncontrolled}, we find that carefully controlling the lexical items in a compositional split has a positive impact on concurrence.
Overall, our results suggest that much work remains to be done to evaluate compositional generalization, and more generally that having more rigorous standards for establishing the validity of evaluation sets should be prioritized in the future.


\input{figures/generalization_studies}





==> CompositionalitySub_arXiv/2_RelatedWork.tex <==
In this section, we provide an overview of datasets commonly used for assessing compositional generalization, and we discuss previous attempts to compare performance across benchmarks.

\paragraph{Datasets for Compositional Generalization}
Since the introduction of \emph{SCAN} in 2018 \citep{lake2018generalization}, many datasets have been proposed to assess compositional generalization in neural networks.
Several of them were direct follow-ups to SCAN that aimed to extend the original dataset or mitigate various issues perceived with it.
For instance, \citet{bastings-etal-2018-jump} introduced NACS, a `reversed' version of SCAN; \citet{loula-etal-2018-rearranging} introduced new splits using the original dataset; \citet{ruis-etal-2020-gscan} introduced a multimodal, grounded version of the benchmark; and \citet{patel-etal-2022-revisiting} increased the number of primitives.
Recently, \citet{valvoda-etal-2022-benchmarking} proposed a transducer-based procedure for generating myriad synthetic datasets similar to SCAN to investigate which formal properties impact the results.
Other artificially generated datasets available to evaluate compositionality are PCFG SET \citep{hupkes2020compositionality}, %
COGS \citep{kim-linzen-2020-cogs}, %
and the dataset proposed by \citet{oren-etal-2021-finding}.

Datasets that use more natural (but often still templated) data are typically situated in the domain of machine translation -- such as \citet{li-etal-2021-compositional}, \citet{dankers-etal-2022-paradox} and \citet{raunak2019compositionality} -- or semantic parsing -- e.g.\ \citet{finegan2018improving,keysers2019measuring,shaw-etal-2021-compositional,cui-etal-2022-compositional}.
Finally, \citet{thrush-etal-2022-winoground} introduce Winoground, aimed to assess compositionality in text-to-image models.
In our work, we focus on datasets that target compositionality in the domain of semantic parsing, with the addition of SCAN for its sheer popularity.


\paragraph{Performance across benchmarks}
Several recent works across NLP have been interested in the extent to which strong performance on one task, setting, or dataset transfers to strong performance on another.
Typically, such experiments are motivated by transfer learning, rather than establishing the validity of evaluation results.
For instance, \citet{vu-etal-2020-exploring}, \citet{ye-etal-2021-crossfit}, \citet{luo-etal-2022-cogtaskonomy}, \citet{padmakumar-etal-2022-exploring}, and \citet{weber-etal-2021-language} all investigate to what extent performance transfers across tasks.
More closely related to our study, is the work presented by \citet{liu2021question}, who quantify the measurement of benchmark agreement on model rankings and compare it in question answering.
In our work, we adopt their definition of comparability across datasets.

In the context of compositional generalization, the work most closely related to ours is the study presented by \citet{chaabouni-etal-2021-transformers}, in which they investigate whether the performance improvements on the synthetic dataset SCAN transfer to the naturalistic setting.
We largely confirm their results, but consider compositionality benchmarks more broadly, not only considering the synthetic v.s\ natural dimension, but also interpretations of compositionality and lexical items exposed during pretraining.







==> CompositionalitySub_arXiv/4_ExperimenalSetup.tex <==
We compare how the conclusions drawn from 18 different compositional generalization splits -- defined over 4 different datasets with 8 compositional splitting strategies -- compare across 6 modeling approaches.
In this section, we describe the datasets and modeling approaches we consider and provide details on training and hyperparameter selection.

\subsection{Models}\label{subsec:models}
For our experiments, we consider both pretrained and train-from-scratch approaches that have previously been considered in the context of compositional generalization.

\paragraph{BART \& T5}
We use the pretrained seq2seq models BART \cite{lewis-etal-2020-bart} and T5 \cite{raffel2020exploring} to enable easy comparison with prior work. 
In the case of BART, order-based noising strategies are used, which may encourage the model to learn to better represent linguistic structure. 

\paragraph{LSTM \& Transformer} 
To ensure coverage of models without pre-trained knowledge, we use a uni-directional LSTM \cite{hochreiter1997long}, a bi-directional LSTM, and a vanilla transformer \cite{vaswani2017attention}.

\paragraph{Neural-BTG}
We include one modeling approach specifically designed to address compositionality: Neural-BTG \cite{wang-etal-2022-hierarchical-phrase}, %
composed of a discriminative parser based on a bracketing transduction grammar (BTG; \citealp{wu-1997-stochastic}) %
and a neural seq2seq model. %


\subsection{Data}\label{subsec:data}
We consider four different datasets designed to test compositional generalization.
We focus on datasets for semantic parsing and include SCAN as the most commonly used dataset for compositionality overall.
Three of these datasets contain different curated \emph{splits} that target different interpretations of compositionality.
Two of the datasets (SCAN and COGS) are synthetic datasets that are generated with rules, while the other two (Spider and GeoQuery) are natural datasets, authored by humans.
Examples for all datasets and descriptions of all curated splits can be found in \cref{app:sec:data}.

\input{tables/data_examples}

\paragraph{SCAN} Consisting of a set of commands and the corresponding action sequences, SCAN \cite{lake2018generalization} is one of the most popular synthetic datasets to study compositional generalization.
We include the \textit{simple}, \textit{length}, \textit{add primitive}, \textit{template} splits from \citet{lake2018generalization}.
In addition to original SCAN splits, we also use the maximum compound divergence (MCD) splits of SCAN proposed by \citet{keysers2020measuring}.

\paragraph{COGS} 
\citet{kim-linzen-2020-cogs} introduced COGS, a synthetic semantic parsing dataset generated by a rule-based approach, which covers a larger variety of grammar rules than SCAN does.
The inputs in COGS are English sentences, generated by a probabilistic context-free grammar. 
The corresponding output, which is the semantic interpretation of the input, is annotated with the logical formalism of \citet{reddy-etal-2017-universal}.
COGS includes a randomly sampled test set and an out-of-distribution compositional generalization set.

\paragraph{GeoQuery} GeoQuery \cite{tang2001using, zelle1996learning} is a text-to-QL dataset containing naturalistic examples.
We use the four compositional generalization splits defined on this dataset by \citet{shaw-etal-2021-compositional}: 
\textit{random/standard}, \textit{length}, \textit{template}, and \textit{Target Maximum Compound Divergence (TMCD)}.

\paragraph{Spider} Spider \cite{yu-etal-2018-Spider} is originally designed for cross-domain semantic parsing. %
We use the compositional generalization splits for Spider defined by \citet{shaw-etal-2021-compositional}, which match their splits for GeoQuery: 
\textit{random/standard}, \textit{length}, \textit{template}, and \textit{TMCD}.

\subsection{Training Setup}
We train/fine-tune the models on the train partition of each dataset described above and evaluate them on the corresponding test set.
For T5 on GeoQuery and Spider as well as LSTM and Transformers on COGS, we use the hyperparameters provided in \citet{shaw-etal-2021-compositional} and \citet{kim-linzen-2020-cogs}, respectively. 
We followed \citet{orhan2021compositional} to train T5 and \citet{yao-koller-2022-structural} to train BART on COGS. 
For the remaining model-dataset combinations, we perform a hyperparameter search for each dataset, with 10\% of instances randomly chosen to be used for tuning. 
Details can be found in \cref{app:hp_tuning}. 
We use three different random seeds for each training run and use five random seeds for each training run of LSTM, to compensate for LSTM's higher variation in performance across seeds.
For models with existing evaluations on a dataset, we compare to these previous measures of performance to ensure that our replication results align with previously reported numbers \cite{keysers2020measuring, kim-linzen-2020-cogs, orhan2021compositional, shaw-etal-2021-compositional, yao-koller-2022-structural, sun-etal-2023-resp}.

\subsection{Evaluation}
\label{sec:expsetup:eval}
For most datasets, we use exact match (EM) accuracy.
EM is a binary metric that only counts an output as correct if it matches the target output exactly, and is most frequently used for the datasets we consider.
During initial experiments, we found that, in many cases, EM accuracy may be too strict for our purposes.
In some cases, models' tokenizers may prefer slightly different spacing -- a phenomenon also reported by \citet{sun2022tokenization} -- in others, models lack specific tokens in their vocabulary.
Neither of these things is indicative of a model's compositional generalization capability, and we therefore choose to normalize model outputs before applying EM accuracy.
In \cref{app:sec:EM}, we include examples of such cases, and we report the differences between EM scores with and without our normalization step.
For Spider, the original dataset also uses a more lenient EM implementation.
For consistency reasons, we use the same implementation across all datasets, but we report Spider EM scores in \cref{app:sec:spider} to compare with previous work. 

\subsection{Measuring Concurrence}
To measure how similarly different dataset splits rank different modeling approaches, we use the concept of \emph{concurrence} introduced by \citet{liu2021question}.
The concurrence between two dataset splits is defined as the correlation between the performances of different modeling approaches for those splits.
More specifically, the concurrence $\text{CONCUR}(D_1, D_2; \mathcal{A}, \text{Eval})$ between two dataset splits $D_1$ and $D_2$, given a set of modeling approaches $\mathcal{A}$ and evaluation function $\text{Eval}$, is defined as:%
\begin{equation*}
    \text{CONCUR}(D_1, D_2; \mathcal{A}, \text{Eval})=\text{CORR}(P_1, P_2),
\end{equation*}
where $\text{CORR}$ is some correlation function and $P_i$ is the variable that holds the scores of Eval($a, D_i$) for all $a\in\mathcal{A}$.
For \text{CORR}, \citet{liu2021question} considered both Pearson ($r$) and Kendall rank ($\tau$). 
Because we are interested in how benchmarks rank model performance, we report the concurrence values under Kendall's $\tau$ unless specified otherwise.
We refer to the concurrence between the dataset split and itself as \emph{self-concurrence}, the value of which is purely affected by seed variation across training runs. 
We see self-concurrence, which would be $1.0$ if there is no variation across seeds, as an upper bound for the concurrence values across dataset splits.



==> CompositionalitySub_arXiv/5_Findings.tex <==

We now present our results, starting with a discussion of the performance of models on the datasets (\cref{sec:overall_perf}) and the concurrence scores between the performances (\cref{sec:predictivity}), we then proceed to look at the relationship between synthetic and natural compositionality datasets (\cref{sec:synvnat}), and how this interacts with the choice of definition of compositionality and underlying dataset (\cref{sec:comp_def}). We finish our results section with a short investigation into the impact of the choice of lexical items in data (\cref{sec:lex_exposure}).

\input{tables/perf_table_v2}
\subsection{Overall Performance}
\input{Results/1_OverallPerf}


\subsection{Overall Concurrence}
\input{Results/2_Predictivity}

\subsection{Synthetic vs natural data}\label{sec:synvnat}
\input{Results/3_Synthetic_vs_natural}

\subsection{Interpretations of compositionality}
\input{Results/4_CompType}

\subsection{The influence of lexical items}
\label{sec:lex_exposure}
\input{figures/std_v_lex}
\input{tables/lexical_split}
\input{Results/5_Lex_Exposure}

\subsection{Other confounding factors}\label{sec:confounding_factors}
\input{Results/7_other_confounding_factors.tex}










==> CompositionalitySub_arXiv/7_Conclusion.tex <==
In this paper, we explored how different evaluation choices impact the conclusions drawn from the experiments evaluating compositionality.
Using compositional generalization datasets and models ranging from trained-from-scratch to pretrained, we conduct a series of experiments to understand whether datasets consistently rank models in terms of their generalizability, and we find little consistency. When we perform further analysis to try to better understand this inconsistency, we find that comparing within the training setting (pretrained v.s.\ trained-from-scratch) or data creation type (synthetically generated v. naturally generated) does not increase consistency.
However, better controlling the lexical items can help us draw more consistent conclusions, at least for datasets that share the same notion of compositionality.
We leave the investigation into how task selection might affect evaluation results for compositional generalization to further research.
Overall, our results suggest that to evaluate compositional generalization consistently, clearer definitions of compositionality are needed, as well as %
more careful consideration of evaluation design and more thorough dataset evaluations.



==> CompositionalitySub_arXiv/8_Limitations.tex <==


While we explore the consequences of the modeling approach on concurrence, we have focused mainly on models trained from scratch to perform compositional generalization or pretrained models which have been finetuned. Another possible area of investigation would be to explore the extent to which a model's compositional generalization abilities also transfer to in-context evaluations \citep{hosseini-etal-2022-compositional}. We leave this question for future work.  


==> CompositionalitySub_arXiv/Results/1_OverallPerf.tex <==
\label{sec:overall_perf}
In \cref{tab:perfStd}, we show the performance of all models on all dataset splits under consideration, as well as the average performance per dataset split (last column).
Our scores are generally close to the scores reported in previous work, for the (dataset split, architecture) combinations for which previous results exist \citep{sun-etal-2023-resp}, with the exception of the results for Spider, for which we use a different metric.
All models perform reasonably well on the random splits of each datasets (first row for each dataset in \cref{tab:perfStd}), but most struggle with various generalization splits. 
While some splits are difficult across the board, other difficulties appear more model-dependent.
For instance, while all models are weak on the \textit{length} and \textit{MCD} splits of SCAN and \textit{length} split of Spider, COGS is difficult for some models (e.g., BTG) but much less for others (e.g., T5).
Similarly, some models perform well on one of the datasets or one of the splits, but perform poorly on the others. 
BART, for instance, maintains high performance on GeoQuery and COGS, but performs even worse than non-pretrained models on some splits of SCAN, while BTG performs well on GeoQuery but fails on many splits of SCAN.
T5 has high performance on most datasets, but is outperformed by the unidirectional LSTM on the \textit{length} split of SCAN.
SCAN, in particular, appears to be challenging for all models, with the \textit{TurnLeft} split being the only exception.%
\footnote{While architectures exist that obtain high scores on SCAN, such as the ones introduced by \citet{shaw-etal-2021-compositional} and \citet{kim2021sequencetosequence}, they are too narrowly scoped for our current study and we thus do not consider them.}



==> CompositionalitySub_arXiv/Results/2_Predictivity.tex <==
\label{sec:predictivity}
\input{tables/concurrence_table}

It is not difficult to tell from Table~\ref{tab:perfStd} that the performance of a model on one dataset is not predictive of its performance on the others.  
To quantitatively substantiate this observation, we compute the concurrences between the different dataset splits, which we visualize in \cref{fig:default_conf_matrix}.
On average, the concurrence between dataset splits is low: a mere $0.22$, far below the average self-concurrence of $0.76$ that (model, split) combinations have across different seeds.
Interestingly, even these average self-concurrence values are lower than the $0.8$ that \citet{liu2021question} used as a threshold for ``high'' concurrence, indicating that performance on the same compositional dataset is not very stable across runs.\footnote{This finding is in line with results reported by \citet{liska2018memorize}, who find a range of different generalization performances on a simple but highly compositional look-up table task.}
Consequently, we lower the threshold to $0.7$ here, which is approximately 90\% of the average self-concurrence.
Of the 153 pairs of dataset split we compare in this experiment, only 10 pairs surpass this threshold.
Somewhat surprisingly, perhaps, many of the highest values (reported in \cref{tab:concurrence}), are concurrences between i.i.d.\ splits and compositional splits.

Considering the concurrence of each dataset with all other datasets (excluding self-concurrence, values are reported below \cref{fig:default_conf_matrix}), we can see that performance COGS, with an average $\tau$ of $0.36$ is most predictive of performance on other datasets.
Furthermore, the three semantic parsing datasets have much higher average concurrence than SCAN, suggesting that compositionality on one task may not be predictive of compositionality on another.







==> CompositionalitySub_arXiv/Results/3_Synthetic_vs_natural.tex <==
\input{figures/perf_v_perf}

Why are these concurrence values so low? %
The first hypothesis that we explore is that performance on strongly structured templated data may not correlate with performance on datasets that are authored by humans. To this end, we compute the average concurrence values of three combinations of dataset split pairs, natural-natural, natural-synthetic and synthetic-synthetic, and include an example of each pair type in \cref{fig:perfvperf}. 
We find that splits of natural datasets concur much better than splits of synthetic datasets ($0.54$ v.s.\ $0.22$); the worst is concurrence between synthetic and natural dataset splits ($0.19$).
The same finding can be observed in \cref{fig:perfvconcur}, which we will use later to explore the relationship between concurrence values and performance in \cref{sec:perf:confounding}.

These results are in line with earlier studies that suggested that performance on synthetic compositionality datasets may not transfer to more realistic scenarios \citep{chaabouni-etal-2021-transformers, shaw-etal-2021-compositional}, and underline the point made by \citet{dankers-etal-2022-paradox}, who argue that compositionality should be studied in its natural habitat.
Also the concurrence between dataset splits with naturalistic data is well below the threshold for high concurrence, suggesting that there exist factors beyond dataset creation strategy that can affect how compositionality benchmarks rank modeling approaches.




==> CompositionalitySub_arXiv/Results/4_CompType.tex <==
\input{figures/pair_type_bar_plot}
\label{sec:comp_def}

The next hypothesis that we consider is that concurrence values are low because different dataset splits investigate different types of compositionality \citep[cf.][]{hupkes2020compositionality}.
In compositional evaluation datasets, the interpretation of compositionality is operationalized through its \emph{splitting strategy}.
One splitting strategy may, for instance, define compositional generalization as generalization to longer lengths, whereas another instead focuses on generalization to novel vocabulary items.
These different interpretations of compositionality could potentially require different model capabilities.
Could it be that our concurrence values are low because different splits in fact focus on different types of compositional generalization?


To investigate this, we group the concurrence values by four dataset pair types -- different datasets with the same splitting strategy, the same dataset with different splitting strategies, different datasets with different splitting strategies, and the same dataset with the same splitting strategy -- and plot them in \cref{fig:pairtype-bar}.
Predictably, datasets concur most with themselves (red line).
We also see that which data a splitting approach is applied to is more important than the interpretation of compositionality (cyan and dark blue lines, respectively): concurrence between experiments that share the same source of data averages at $0.38$, whereas different data but the same splitting strategy results in an average concurrence of $0.32$.
However, when both the source of data and splitting strategy are different (yellow line), the concurrence values  shift leftward, suggesting that the data type and splitting strategy pose different kinds of difficulties for the modelling approaches considered.

\input{tables/length_split_concurrences}

\paragraph{Length Generalization}
Because not every dataset in previous work applied all the splitting strategies, we follow-up with a small experiment in a split shared across all datasets: \emph{length generalization} splits.\footnote{As the original COGS dataset did not come with a length generalization split, we generate one ourselves.}
The concurrence values between the different length splits, shown in \cref{tab:length}, are generally low, ranging from $-0.09$ to $0.54$ and averaging at 0.16.
This additional experiment confirms that even when benchmarks maintain the same interpretation of compositionality, there may still be substantial differences in model rankings, depending on the underlying data.



==> CompositionalitySub_arXiv/Results/5_Lex_Exposure.tex <==

In \cref{tab:perfStd}, we can see that pretrained models achieve the highest accuracies and in \cref{tab:concurrence} that the highest concurrence values are between two natural datasets. 
In this section, we dive into the differences between pretrained and trained-from-scratch models,  and investigate the extent to which those differences affect the concurrence results.
In particular, we investigate whether the presence of uncontrolled lexical exposure during pretraining may impact the performance of pretrained models, implying their accuracy numbers may not solely reflect their compositional abilities, as suggested by \citet{kim2022uncontrolled}.
Were this to happen, a misalignment in the evaluation between pretrained and non-pretrained models would contribute to variation in the concurrence values, where the performance of pretrained models is overestimated due to lexical exposure in pretraining.

To test for possible effects of lexical exposure, we extend the experiment from \citet{kim2022uncontrolled} -- who conducted it for COGS -- to the TMCD and Std split of GeoQueory, and the TurnLeft split of SCAN\footnote{In both these cases, particular lexical items are purposefully left out of the training set, to be evaluated at test time. If those lexical items were also present in the uncontrolled pretraining corpus, this would thus break the test.}
In both cases, we swap out lexical items with strings of similar length that act as ``wug words'' \citep{berko-1958-child}, or, in other words, previously unattested and therefore meaningless lexical items.
Following \citet{kim2022uncontrolled}, we generate the strings in two ways:
\begin{compactitem}
    \item \textit{Rstr:} We randomly sample lowercase characters from the Latin script with replacements.
    \item \textit{Rcvcv:} We alternately sample a vowel after a consonant from the Latin script.
\end{compactitem}

\noindent We train the models on all modified splits and compute the performance (\cref{fig:std_v_lex}). 
We also compute the concurrence between the original split and the modified split (\cref{tab:sub:lex-concur} and \cref{tab:sub:lex-high-concur}).

In \cref{fig:std_v_lex}, we see that the performance of the pretrained models drops drastically when the lexical items are replaced, while the non-pretrained models' performance does not, confirming the results of \citet{kim2022uncontrolled}.
In addition, the concurrence between the original splits and the modified splits for all datasets is below our set threshold -- albeit higher than other comparisons we have seen before (Table~\ref{tab:sub:lex-concur}) -- implying that replacing lexical items results in yet another new ranking of modeling approaches for compositionality.

We then compute the concurrence between the same set of splits before and after the lexical exposure edits: \emph{within} the group of splits that are selected for the lexical changes, the concurrence values decrease from $0.49$ to $0.41$, while the average concurrence values of these splits with \emph{other} splits that haven't undergone lexical edits slightly increase from $0.25$ to $0.26$ (e.g. concurrence between GeoQuery and Spider TMCD splits increases when GeoQuery TMCD split applies the lexical changes), with many more dataset split pairs surpassing the $\tau=0.7$ bar for high concurrence (\cref{tab:sub:lex-high-concur}).

A closer look explains this apparent contrast: the overall low-concurring dataset SCAN -- which makes up 12.5\% of the lexically edited splits, drags down the concurrence values within that group.
Excluding SCAN, the within-group concurrence values also increase, from $0.63$ to $0.66$.
These results do thus not only confirm that controlling lexical exposure is important when evaluating compositionality in pretrained models, but also further exemplify our earlier finding that compositionality scores -- for neural models -- strongly depend task and dataset. We further analyze the influence of tasks to compositionality results in \cref{app:sec:nacs}.




==> CompositionalitySub_arXiv/Results/6_Eval_Metric.tex <==



Despite of data source and exposed lexical items, other confounding factors can appear during the evaluation of compositionality.
As we have observed in \cref{fig:default_conf_matrix}, splits of SCAN obtain low concurrence with most of splits from other datasets.
In the mean time, the task of SCAN, grounded navigation, is most distant from the others, which are based on semantic parsing.
This and our finding in \cref{sec:comp_def} are \textit{in pari materia}: the source of data (regardless of the task) contributes more to the resulting model rankings compared to the interpretation of generalization, and gives hints about the degree to which datasets disagree with each other when considering two more distant pairs of datasets in terms of their task.
We leave the investigation on how the selection of specific tasks affect evaluation result of compositionality to further research.

The in-distribution performance may also become a confounder when model performs poorly on the random split of the data.
Qualitatively, we observe that models sometimes make the same trivial mistakes in both a random split and a generalization split, making the evaluation result unrepresentative of compositionality.
We leave such examples in \cref{app:sec:mistakes}.





==> CompositionalitySub_arXiv/Results/7_other_confounding_factors.tex <==
\label{sec:perf:confounding}
We have explored a range of factors that may impact the evaluation of compositionality, such as the nature of the underlying data and task, the interpretation of compositionality, and the choice of lexical items.
We wrap up our analysis by verifying that our results are not driven by specific performance scores: we verify that concurrence values are not skewed by datasets for which performances are saturated or close to random.
To assess this, we compute the correlation between the average performance between two datasets and their concurrence, as plotted in \cref{fig:perfvconcur}.
As can be seen, there is no apparent relation between average performance and concurrence: difficult datasets do not concur less or more than easier ones, and dataset saturation (or the opposite: random performance) appears not to impact the results.
A correlation test confirms this visually observed pattern: the Pearson correlation coefficient between performance and concurrence is near zero ($r=0.026$).

\input{figures/perf_vs_concur}


==> CompositionalitySub_arXiv/Results/8_app_NACS.tex <==
\label{app:sec:nacs}
As briefly mentioned in \cref{sec:lex_exposure}, task formulation can be another factor that affects the agreement between datasets.
To understand the effect of task similarity on the conclusion obtained from compositionality benchmarks, we add in the NACS dataset \cite{bastings-etal-2018-jump} for existing experiments, as all three datasets except for SCAN are semantic parsing tasks, while SCAN falls under a navigation task.
NACS is introduced as a dataset that is similar to SCAN but requires mapping actions back to the original commands, and it is thus more complex for models compared to SCAN and will not allow simple models to gain unintended high performance.
We train models on NACS with the same hyperparameter tuning and training strategy as in \cref{sec:Methods}, compute the concurrence between NACS and other datasets, and look at the effect of different splitting strategy between SCAN and NACS. 
The results are discussed below.

\subsection{Overall Performance and Concurrence}
\input{figures/app_NACS/conf_matrix_nacs}
\input{figures/app_NACS/density_by_type}
\input{tables/app_NACS/NACS_high_concur}
The overall performance and concurrence including NACS are shown in \cref{app:tab:all-perf} and \cref{app:fig:nacs-default_conf_matrix}.
The concurrence values between NACS and SCAN is surprisingly low compared to the concurrence values between NACS and other datasets, with the \textit{length} split being the only exception, suggesting that even when the underlying tasks are the same, the datasets may provide very different model rankings.
In terms of the distribution of concurrence values by type of data split pairs (\cref{app:fig:nacs-pairtype-bar}), the conclusion in \cref{sec:comp_def} persists: the source of the dataset matters more than the interpretation of compositonality (splitting strategy).

\subsection{Length Split of NACS}
\input{tables/app_NACS/NACS_length}
Out of the four splits of NACS, the \textit{length} split is the only split that results in a high concurrence with tsplits of SCAN (\cref{app:fig:nacs-default_conf_matrix}).
The \textit{length} split of SCAN and NACS is also the only length splits pair that exceed the boundary set for high concurrence (\cref{app:tab:nacs-length}).
It is likely because that both \textit{length} split of NACS and the splits that it has high concurrence with are extremely difficult split that many models fail on.


==> CompositionalitySub_arXiv/abstract.tex <==
\begin{abstract}
NLP models have progressed drastically in recent years, according to numerous datasets proposed to evaluate performance.
Questions remain, however, about how particular dataset design choices may impact the conclusions we draw about model capabilities.
In this work, we investigate this question in the domain of compositional generalization. 
We examine the performance of six modeling approaches across 4 datasets, split according to 8 compositional splitting strategies, ranking models by 18 compositional generalization splits in total.
Our results show that:
i) the datasets, although all designed to evaluate compositional generalization, rank modeling approaches differently;
ii) datasets generated by humans align better with each other than they with synthetic datasets, or than synthetic datasets among themselves;
iii) generally, whether datasets are sampled from the same source is more predictive of the resulting model ranking than whether they maintain the same interpretation of compositionality; and
iv) which lexical items are used in the data can strongly impact conclusions.
Overall, our results demonstrate that much work remains to be done when it comes to assessing whether popular evaluation datasets measure what they intend to measure, and suggests that elucidating more rigorous standards for establishing the validity of evaluation sets could benefit the field.\footnote{Code to reproduce the experiments can be found at \url{https://github.com/facebookresearch/CompositionalityValidity}.}
\end{abstract}


==> CompositionalitySub_arXiv/figures/app_NACS/conf_matrix_nacs.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\the\columnwidth]{figures/app_NACS/conf_matrix_default.pdf}
    \caption{Distribution of concurrence values between each dataset and split pairs.}
\label{app:fig:nacs-default_conf_matrix}
\end{figure}

==> CompositionalitySub_arXiv/figures/app_NACS/density_by_type.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.85\columnwidth]{figures/app_NACS/density_by_type_app.pdf}
\caption{Distribution of concurrence values among all dataset splits. The color of the bar indicates whether the splits in the pair share the same dataset origin and/or the same splitting strategy.}
\label{app:fig:nacs-pairtype-bar}
\end{figure}

==> CompositionalitySub_arXiv/figures/app_NACS/perf_vs_concur.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.85\columnwidth]{figures/app_NACS/perf_vs_concur_app.pdf}
\caption{Values of concurrences with respect to pairwise averaged performance among the splits shown in \cref{app:tab:nacs-all-perf}. The color of dots indicates the type of split pairs. The triangle-shape dots indicates the values of self-concurrence.}
\label{fig:perfvconcur}
\end{figure}

==> CompositionalitySub_arXiv/figures/app_overall_concur.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=0.9\textwidth]{figures/fig_files/conf_matrix.pdf}
\caption{Distribution of concurrence values between each dataset and split pairs.}
\label{fig:app:conf_matrix}
\end{figure*}

==> CompositionalitySub_arXiv/figures/default_conf_matrix.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\the\columnwidth]{figures/fig_files/default_conf_matrix_avg.pdf}
    \caption{Pairwise concurrence values averaged across models for each dataset--split pair. Values closer to 1.0 (blue) denote a more similar ranking of models according to their performance on the dataset and split. The dataset and split font color indicate whether the data was generated by humans (purple) or synthetically using rules (green).}
\label{fig:default_conf_matrix}
\end{figure}


==> CompositionalitySub_arXiv/figures/generalization_studies.tex <==
\begin{figure}
\centering
\includegraphics[width=0.8\columnwidth]{figures/fig_files/pub_count.pdf}
    \caption{Generalization studies published in the ACL anthology (2015-2022), across different \emph{shift sources}.}\label{fig:generalisation_vs_source}
\end{figure}


==> CompositionalitySub_arXiv/figures/pair_type_bar_plot.tex <==

\begin{figure}[t]
\centering
\includegraphics[width=0.85\columnwidth]{figures/fig_files/density_by_type.pdf}
\caption{Distribution of concurrence values among all dataset splits. The color of the bar indicates whether the splits in the pair share the same dataset origin and/or the same splitting strategy.}
\label{fig:pairtype-bar}
\end{figure}

==> CompositionalitySub_arXiv/figures/perf_v_perf.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{figures/fig_files/pretrained_nonpretrained.pdf}
\caption{Performance of one dataset split versus another. Upper left is an example of high concurrence pair between a synthetic and a natural dataset; upper right is an example of low concurrence within synthetic datasets; lower left is an example of high concurrence within natural datasets; lower right is an example of low concurrence between natural and synthetic datasets.}
\label{fig:perfvperf}
\end{figure}

==> CompositionalitySub_arXiv/figures/perf_vs_concur.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.85\columnwidth]{figures/fig_files/perf_alignment.pdf}
\caption{Values of concurrences with respect to pairwise averaged performance among the splits shown in Table~\ref{tab:perfStd}. The color of dots indicates the type of split pairs. The triangle-shape dots indicates the values of self-concurrence.}
\label{fig:perfvconcur}
\end{figure}

==> CompositionalitySub_arXiv/figures/std_v_lex.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.85\columnwidth]{figures/fig_files/std_vs_lex.pdf}
\caption{Performance of the original split versus the splits with lexical items replaced. Performance of pretrained models decreases when train on the splits with lexical items that are not previously seen in pretraining.}
\label{fig:std_v_lex}
\end{figure}

==> CompositionalitySub_arXiv/tables/app_NACS/NACS_high_concur.tex <==
\begin{table}[t]
\centering
\scriptsize
\begin{tabular}{llllc}
\toprule
\textbf{Dataset A} & \textbf{Dataset B} & \textbf{Split A} & \textbf{Split B} & \textbf{Concur} \\ \midrule
Spider   & Spider   & \textit{Template} & \textit{TMCD}     & 0.88 \\
GeoQuery & Spider   & \textit{Std}      & \textit{Template} & 0.84 \\
GeoQuery & Spider   & \textit{Std}      & \textit{TMCD}     & 0.83 \\
SCAN     & Spider   & \textit{Template} & \textit{Rand}     & 0.76 \\
SCAN     & Spider   & \textit{Template} & \textit{Length}   & 0.76 \\
Spider   & Spider   & \textit{Rand}     & \textit{Length}   & 0.75 \\
GeoQuery & Spider   & \textit{Template} & \textit{Template} & 0.74 \\
SCAN     & NACS     & \textit{MCD2}     & \textit{Length}   & 0.74 \\
GeoQuery & Spider   & \textit{Template} & \textit{TMCD}     & 0.73 \\
SCAN     & NACS     & \textit{Length}   & \textit{Length}   & 0.73 \\
GeoQuery & GeoQuery & \textit{Std}      & \textit{Template} & 0.73 \\
SCAN     & SCAN     & \textit{Length}   & \textit{MCD3}     & 0.72 \\
\bottomrule
\end{tabular}
\caption{High concurrence values ($\geq 0.7$) among all pairs of dataset splits, excluding self-concurrence.}
\label{app:tab:NACS:concurrence}
\end{table}

==> CompositionalitySub_arXiv/tables/app_NACS/NACS_length.tex <==

\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{llllll}
\toprule
\textbf{Dataset A} & \textbf{Dataset B} & \textbf{Concur} & \textbf{Dataset A} & \textbf{Dataset B} & \textbf{Concur} \\ 
\cmidrule(lr){1-3} \cmidrule(lr){4-6}

SCAN      & NACS      & \phstar 0.73   & GeoQuery & NACS   & \phstar 0.08  \\
COGS      & GeoQuery  & \phstar 0.54   & Spider   & NACS   & \phstar 0.04  \\
COGS      & Spider    & \phstar 0.26   & SCAN     & Spider & \phstar 0.01  \\
COGS      & NACS      & \phstar 0.24   & COGS     & SCAN   & \phstar 0.01  \\
GeoQuery  & Spider    & \phstar 0.23   & GeoQuery & SCAN   & \phstar -0.09 \\
 \bottomrule
\end{tabular}
\caption{Concurrence between length splits of datasets.}
\label{app:tab:nacs-length}
\end{table}

==> CompositionalitySub_arXiv/tables/app_all_concur.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lllllllllc}
\toprule
\textbf{Dataset A} &
  \textbf{Dataset B} &
  \textbf{Split B} &
  \textbf{Split A} &
  \textbf{Concur} &
  \textbf{Dataset A} &
  \textbf{Dataset B} &
  \textbf{Split A} &
  \textbf{Split B} &
  \textbf{Concur} \\ \midrule
Spider   & Spider   & \textit{TMCD}          & \textit{Template}      & 0.88 & COGS     & GeoQuery & \textit{RandStr}    & \textit{TMCD-Rstr}     & 0.54 \\
COGS     & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{Length}        & 0.84 & GeoQuery & SCAN     & \textit{Std-Rstr}   & \textit{TurnLeft}      & 0.54 \\
GeoQuery & Spider   & \textit{Template}      & \textit{Std}           & 0.84 & COGS     & SCAN     & \textit{Std}        & \textit{TurnLeft}      & 0.53 \\
GeoQuery & Spider   & \textit{Template}      & \textit{TMCD-Rstr}     & 0.84 & COGS     & SCAN     & \textit{Randcvcv}   & \textit{TurnLeft}      & 0.52 \\
GeoQuery & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{Std-Rcvcv}     & 0.83 & SCAN     & SCAN     & \textit{MCD1}       & \textit{MCD2}          & 0.52 \\
GeoQuery & Spider   & \textit{TMCD}          & \textit{Std}           & 0.83 & SCAN     & SCAN     & \textit{Length}     & \textit{MCD1}          & 0.52 \\
COGS     & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{Std}           & 0.82 & COGS     & GeoQuery & \textit{Randcvcv}   & \textit{TMCD-Rcvcv}    & 0.51 \\
COGS     & COGS     & \textit{RandStr}       & \textit{Randcvcv}      & 0.82 & GeoQuery & SCAN     & \textit{TMCD-Rcvcv} & \textit{TurnLeft}      & 0.51 \\
GeoQuery & Spider   & \textit{Template}      & \textit{TMCD-Rcvcv}    & 0.81 & SCAN     & SCAN     & \textit{MCD1}       & \textit{MCD3}          & 0.51 \\
COGS     & Spider   & \textit{Template}      & \textit{Length}        & 0.81 & COGS     & SCAN     & \textit{Std}        & \textit{Jump}          & 0.5  \\
GeoQuery & Spider   & \textit{TMCD}          & \textit{TMCD-Rstr}     & 0.81 & GeoQuery & GeoQuery & \textit{Std-Rstr}   & \textit{Template}      & 0.5  \\
GeoQuery & GeoQuery & \textit{TMCD-Rstr}     & \textit{TMCD-Rcvcv}    & 0.81 & GeoQuery & SCAN     & \textit{TMCD-Rcvcv} & \textit{Jump}          & 0.49 \\
COGS     & GeoQuery & \textit{TMCD-Rstr}     & \textit{Length}        & 0.8  & COGS     & GeoQuery & \textit{Randcvcv}   & \textit{Std-Rcvcv}     & 0.49 \\
COGS     & GeoQuery & \textit{Std-Rcvcv}     & \textit{Length}        & 0.8  & GeoQuery & GeoQuery & \textit{Std-Rcvcv}  & \textit{Length}        & 0.48 \\
COGS     & Spider   & \textit{TMCD}          & \textit{Length}        & 0.79 & COGS     & Spider   & \textit{RandStr}    & \textit{Template}      & 0.47 \\
GeoQuery & Spider   & \textit{TMCD}          & \textit{TMCD-Rcvcv}    & 0.79 & COGS     & SCAN     & \textit{RandStr}    & \textit{TurnLeft}      & 0.47 \\
GeoQuery & GeoQuery & \textit{TMCD-Rstr}     & \textit{Std}           & 0.79 & COGS     & COGS     & \textit{Randcvcv}   & \textit{Length}        & 0.47 \\
GeoQuery &
  GeoQuery &
  \textit{TMCD-Rstr} &
  \textit{Std-Rcvcv} &
  0.78 &
  GeoQuery &
  GeoQuery &
  \textit{Std-Rstr} &
  \textit{TMCD} &
  0.46 \\
COGS     & GeoQuery & \textit{Std-Rcvcv}     & \textit{Std}           & 0.78 & COGS     & GeoQuery & \textit{Randcvcv}   & \textit{TMCD-Rstr}     & 0.46 \\
COGS     & COGS     & \textit{Length}        & \textit{Std}           & 0.76 & COGS     & Spider   & \textit{RandStr}    & \textit{TMCD}          & 0.46 \\
SCAN     & Spider   & \textit{Rand}          & \textit{Template}      & 0.76 & GeoQuery & GeoQuery & \textit{Std-Rstr}   & \textit{Length}        & 0.44 \\
SCAN     & Spider   & \textit{Length}        & \textit{Template}      & 0.76 & GeoQuery & SCAN     & \textit{Std-Rcvcv}  & \textit{TurnLeft}      & 0.43 \\
COGS     & GeoQuery & \textit{Std}           & \textit{Length}        & 0.75 & COGS     & SCAN     & \textit{Length}     & \textit{Jump}          & 0.43 \\
GeoQuery & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{Std}           & 0.75 & GeoQuery & SCAN     & \textit{Std-Rcvcv}  & \textit{Jump}          & 0.42 \\
Spider   & Spider   & \textit{Length}        & \textit{Rand}          & 0.75 & COGS     & GeoQuery & \textit{RandStr}    & \textit{Std}           & 0.42 \\
GeoQuery & Spider   & \textit{Template}      & \textit{Template}      & 0.74 & COGS     & SCAN     & \textit{Randcvcv}   & \textit{Jump}          & 0.41 \\
GeoQuery & Spider   & \textit{TMCD}          & \textit{Template}      & 0.73 & GeoQuery & SCAN     & \textit{TMCD-Rstr}  & \textit{TurnLeft}      & 0.41 \\
GeoQuery & Spider   & \textit{Template}      & \textit{Std-Rcvcv}     & 0.73 & COGS     & SCAN     & \textit{Length}     & \textit{TurnLeft}      & 0.41 \\
GeoQuery & GeoQuery & \textit{Template}      & \textit{Std}           & 0.73 & COGS     & SCAN     & \textit{RandStr}    & \textit{Jump}          & 0.41 \\
COGS     & GeoQuery & \textit{Std-Rstr}      & \textit{RandStr}       & 0.73 & COGS     & GeoQuery & \textit{RandStr}    & \textit{Template}      & 0.4  \\
COGS     & GeoQuery & \textit{TMCD-Rstr}     & \textit{Std}           & 0.72 & GeoQuery & SCAN     & \textit{TMCD-Rstr}  & \textit{Jump}          & 0.4  \\
SCAN     & SCAN     & \textit{MCD3}          & \textit{Length}        & 0.72 & SCAN     & Spider   & \textit{Jump}       & \textit{Length}        & 0.4  \\
COGS     & GeoQuery & \textit{Std-Rstr}      & \textit{Std}           & 0.72 & SCAN     & SCAN     & \textit{Jump}       & \textit{TurnLeft}      & 0.4  \\
GeoQuery & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{Std-Rstr}      & 0.71 & COGS     & Spider   & \textit{Randcvcv}   & \textit{Template}      & 0.39 \\
GeoQuery & Spider   & \textit{TMCD}          & \textit{Std-Rcvcv}     & 0.71 & GeoQuery & SCAN     & \textit{Length}     & \textit{Jump}          & 0.39 \\
COGS     & GeoQuery & \textit{Std-Rstr}      & \textit{Randcvcv}      & 0.7  & SCAN     & SCAN     & \textit{Jump}       & \textit{Template}      & 0.39 \\
GeoQuery & GeoQuery & \textit{TMCD-Rstr}     & \textit{Template}      & 0.7  & SCAN     & Spider   & \textit{Jump}       & \textit{Template}      & 0.39 \\
COGS     & Spider   & \textit{Template}      & \textit{Std}           & 0.69 & SCAN     & Spider   & \textit{Jump}       & \textit{Rand}          & 0.38 \\
GeoQuery & GeoQuery & \textit{Std-Rcvcv}     & \textit{Std}           & 0.69 & SCAN     & Spider   & \textit{Jump}       & \textit{TMCD}          & 0.38 \\
SCAN     & SCAN     & \textit{TurnLeftRStr}  & \textit{Simple}        & 0.68 & COGS     & Spider   & \textit{Randcvcv}   & \textit{TMCD}          & 0.38 \\
GeoQuery & GeoQuery & \textit{Std-Rstr}      & \textit{Std-Rcvcv}     & 0.68 & GeoQuery & SCAN     & \textit{Std-Rcvcv}  & \textit{MCD2}          & 0.37 \\
GeoQuery & Spider   & \textit{Template}      & \textit{TMCD}          & 0.68 & Spider   & Spider   & \textit{Rand}       & \textit{TMCD}          & 0.36 \\
GeoQuery & Spider   & \textit{TMCD}          & \textit{TMCD}          & 0.68 & GeoQuery & SCAN     & \textit{TMCD-Rstr}  & \textit{MCD2}          & 0.36 \\
SCAN     & SCAN     & \textit{TurnLeftRcvcv} & \textit{Simple}        & 0.68 & GeoQuery & Spider   & \textit{Length}     & \textit{Rand}          & 0.35 \\
GeoQuery & GeoQuery & \textit{TMCD}          & \textit{Std}           & 0.68 & GeoQuery & SCAN     & \textit{TMCD-Rcvcv} & \textit{MCD2}          & 0.35 \\
COGS     & Spider   & \textit{TMCD}          & \textit{Std}           & 0.67 & Spider   & Spider   & \textit{Rand}       & \textit{Template}      & 0.35 \\
COGS     & GeoQuery & \textit{Std-Rstr}      & \textit{Length}        & 0.67 & GeoQuery & SCAN     & \textit{Length}     & \textit{Template}      & 0.35 \\
COGS     & GeoQuery & \textit{Template}      & \textit{Length}        & 0.67 & GeoQuery & SCAN     & \textit{Std}        & \textit{Jump}          & 0.35 \\
GeoQuery & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{Template}      & 0.66 & GeoQuery & Spider   & \textit{Std}        & \textit{Rand}          & 0.35 \\
GeoQuery & GeoQuery & \textit{TMCD}          & \textit{Template}      & 0.65 & SCAN     & SCAN     & \textit{MCD2}       & \textit{Jump}          & 0.35 \\
GeoQuery & GeoQuery & \textit{TMCD-Rstr}     & \textit{TMCD}          & 0.65 & COGS     & GeoQuery & \textit{RandStr}    & \textit{TMCD}          & 0.34 \\
GeoQuery & GeoQuery & \textit{TMCD-Rstr}     & \textit{Std-Rstr}      & 0.65 & Spider   & Spider   & \textit{Length}     & \textit{TMCD}          & 0.34 \\
SCAN     & SCAN     & \textit{MCD2}          & \textit{Length}        & 0.64 & Spider   & Spider   & \textit{Length}     & \textit{Template}      & 0.34 \\
SCAN     & SCAN     & \textit{TurnLeftRStr}  & \textit{TurnLeftRcvcv} & 0.64 & COGS     & GeoQuery & \textit{Randcvcv}   & \textit{Std}           & 0.34 \\
COGS     & GeoQuery & \textit{Std}           & \textit{Std}           & 0.64 & SCAN     & Spider   & \textit{TurnLeft}   & \textit{Template}      & 0.34 \\
GeoQuery & Spider   & \textit{TMCD}          & \textit{Length}        & 0.63 & COGS     & GeoQuery & \textit{Randcvcv}   & \textit{Length}        & 0.34 \\
GeoQuery & GeoQuery & \textit{TMCD}          & \textit{Length}        & 0.63 & GeoQuery & SCAN     & \textit{TMCD}       & \textit{Jump}          & 0.33 \\
GeoQuery & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{TMCD}          & 0.63 & COGS     & SCAN     & \textit{Std}        & \textit{MCD2}          & 0.33 \\
COGS     & GeoQuery & \textit{TMCD}          & \textit{Length}        & 0.63 & COGS     & GeoQuery & \textit{Randcvcv}   & \textit{Template}      & 0.33 \\
GeoQuery & Spider   & \textit{Template}      & \textit{Length}        & 0.63 & COGS     & GeoQuery & \textit{RandStr}    & \textit{Length}        & 0.32 \\
GeoQuery & GeoQuery & \textit{Length}        & \textit{Std}           & 0.62 & SCAN     & Spider   & \textit{TurnLeft}   & \textit{TMCD}          & 0.32 \\
GeoQuery & GeoQuery & \textit{Template}      & \textit{Length}        & 0.62 & GeoQuery & Spider   & \textit{Std}        & \textit{Length}        & 0.32 \\
GeoQuery & GeoQuery & \textit{Template}      & \textit{Std-Rcvcv}     & 0.62 & SCAN     & Spider   & \textit{Template}   & \textit{TMCD}          & 0.32 \\
GeoQuery & Spider   & \textit{Template}      & \textit{Std-Rstr}      & 0.6  & SCAN     & Spider   & \textit{MCD1}       & \textit{Length}        & 0.31 \\
COGS     & COGS     & \textit{RandStr}       & \textit{Std}           & 0.6  & GeoQuery & Spider   & \textit{Template}   & \textit{Rand}          & 0.31 \\
GeoQuery & GeoQuery & \textit{TMCD}          & \textit{Std-Rcvcv}     & 0.6  & GeoQuery & SCAN     & \textit{Template}   & \textit{Jump}          & 0.31 \\
COGS     & COGS     & \textit{Randcvcv}      & \textit{Std}           & 0.59 & GeoQuery & Spider   & \textit{TMCD}       & \textit{Rand}          & 0.31 \\
GeoQuery & Spider   & \textit{TMCD}          & \textit{Std-Rstr}      & 0.58 & SCAN     & Spider   & \textit{Template}   & \textit{Template}      & 0.31 \\
GeoQuery & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{Length}        & 0.57 & GeoQuery & SCAN     & \textit{Std}        & \textit{Template}      & 0.3  \\
COGS     & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{RandStr}       & 0.57 & GeoQuery & Spider   & \textit{Std-Rstr}   & \textit{Rand}          & 0.3  \\
SCAN     & SCAN     & \textit{MCD3}          & \textit{MCD2}          & 0.57 & COGS     & SCAN     & \textit{Randcvcv}   & \textit{TurnLeftRStr}  & 0.29 \\
COGS     & GeoQuery & \textit{Length}        & \textit{Std}           & 0.56 & SCAN     & SCAN     & \textit{TurnLeft}   & \textit{TurnLeftRcvcv} & 0.29 \\
COGS     & GeoQuery & \textit{TMCD}          & \textit{Std}           & 0.56 & GeoQuery & SCAN     & \textit{Template}   & \textit{Template}      & 0.28 \\
COGS     & GeoQuery & \textit{Template}      & \textit{Std}           & 0.56 & SCAN     & SCAN     & \textit{MCD2}       & \textit{TurnLeft}      & 0.28 \\
COGS     & GeoQuery & \textit{Std-Rcvcv}     & \textit{RandStr}       & 0.56 & COGS     & GeoQuery & \textit{Randcvcv}   & \textit{TMCD}          & 0.28 \\
GeoQuery & GeoQuery & \textit{TMCD-Rstr}     & \textit{Length}        & 0.55 & GeoQuery & SCAN     & \textit{Std}        & \textit{TurnLeft}      & 0.28 \\
COGS     & COGS     & \textit{Length}        & \textit{RandStr}       & 0.55 & COGS     & SCAN     & \textit{Length}     & \textit{MCD2}          & 0.28 \\
GeoQuery & SCAN     & \textit{Jump}          & \textit{Std-Rstr}      & 0.54 & GeoQuery & SCAN     & \textit{Length}     & \textit{TurnLeft}      & 0.28 \\
COGS     & GeoQuery & \textit{Length}        & \textit{Length}        & 0.54 & GeoQuery & SCAN     & \textit{TMCD}       & \textit{Template}      & 0.28 \\
GeoQuery & GeoQuery & \textit{Std-Rstr}      & \textit{Std}           & 0.54 & GeoQuery & Spider   & \textit{Std-Rstr}   & \textit{Length}        & 0.27      \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Concurrence Values.}
\label{tab:app:Concurrence}
\end{table*}

\begin{table*}[ht]
\centering
\scriptsize
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{llllllllll}
\toprule
\textbf{Dataset A} &
  \textbf{Dataset B} &
  \textbf{Split A} &
  \textbf{Split B} &
  \textbf{Concur} &
  \textbf{Dataset A} &
  \textbf{Dataset B} &
  \textbf{Split A} &
  \textbf{Split B} &
  \textbf{Concur} \\ \midrule
COGS     & Spider & \textit{Length}     & \textit{Rand}          & 0.27 & SCAN     & SCAN   & \textit{Jump}          & \textit{TurnLeftRcvcv} & 0.02  \\
GeoQuery & SCAN   & \textit{Std-Rstr}   & \textit{Template}      & 0.27 & COGS     & SCAN   & \textit{Std}           & \textit{MCD1}          & 0.02  \\
GeoQuery & SCAN   & \textit{Std-Rstr}   & \textit{MCD2}          & 0.27 & SCAN     & Spider & \textit{MCD3}          & \textit{Length}        & 0.02  \\
COGS     & SCAN   & \textit{RandStr}    & \textit{TurnLeftRStr}  & 0.27 & COGS     & SCAN   & \textit{Length}        & \textit{MCD3}          & 0.02  \\
COGS     & Spider & \textit{Length}     & \textit{Length}        & 0.26 & GeoQuery & SCAN   & \textit{TMCD-Rcvcv}    & \textit{TurnLeftRStr}  & 0.02  \\
SCAN     & SCAN   & \textit{Length}     & \textit{TurnLeft}      & 0.25 & SCAN     & SCAN   & \textit{MCD1}          & \textit{TurnLeft}      & 0.02  \\
GeoQuery & SCAN   & \textit{TMCD}       & \textit{TurnLeft}      & 0.24 & SCAN     & Spider & \textit{Length}        & \textit{Length}        & 0.01  \\
GeoQuery & Spider & \textit{Template}   & \textit{Length}        & 0.24 & COGS     & SCAN   & \textit{Length}        & \textit{Length}        & 0.01  \\
COGS     & SCAN   & \textit{Randcvcv}   & \textit{Simple}        & 0.24 & SCAN     & SCAN   & \textit{Simple}        & \textit{MCD3}          & 0.01  \\
SCAN     & SCAN   & \textit{MCD1}       & \textit{Template}      & 0.24 & SCAN     & Spider & \textit{Simple}        & \textit{Length}        & 0.01  \\
SCAN     & SCAN   & \textit{TurnLeft}   & \textit{TurnLeftRStr}  & 0.23 & SCAN     & SCAN   & \textit{TurnLeft}      & \textit{Template}      & 0.01  \\
GeoQuery & SCAN   & \textit{Template}   & \textit{TurnLeft}      & 0.23 & SCAN     & SCAN   & \textit{Simple}        & \textit{Jump}          & 0.0   \\
GeoQuery & Spider & \textit{TMCD}       & \textit{Length}        & 0.23 & SCAN     & Spider & \textit{TurnLeft}      & \textit{Rand}          & -0.0  \\
GeoQuery & Spider & \textit{Length}     & \textit{Length}        & 0.23 & COGS     & SCAN   & \textit{Randcvcv}      & \textit{Length}        & -0.01 \\
GeoQuery &
  Spider &
  \textit{TMCD-Rcvcv} &
  \textit{Length} &
  0.22 &
  GeoQuery &
  SCAN &
  \textit{Std-Rcvcv} &
  \textit{TurnLeftRStr} &
  -0.01 \\
SCAN     & SCAN   & \textit{Length}     & \textit{Jump}          & 0.22 & GeoQuery & SCAN   & \textit{Std}           & \textit{MCD1}          & -0.02 \\
COGS     & SCAN   & \textit{Length}     & \textit{Template}      & 0.22 & SCAN     & Spider & \textit{MCD1}          & \textit{Template}      & -0.02 \\
GeoQuery & Spider & \textit{TMCD-Rstr}  & \textit{Length}        & 0.22 & GeoQuery & SCAN   & \textit{TMCD}          & \textit{MCD1}          & -0.02 \\
GeoQuery & Spider & \textit{TMCD-Rcvcv} & \textit{Rand}          & 0.22 & COGS     & SCAN   & \textit{Std}           & \textit{TurnLeftRcvcv} & -0.02 \\
GeoQuery & Spider & \textit{TMCD-Rstr}  & \textit{Rand}          & 0.21 & COGS     & SCAN   & \textit{RandStr}       & \textit{MCD1}          & -0.02 \\
COGS     & SCAN   & \textit{RandStr}    & \textit{Simple}        & 0.21 & COGS     & SCAN   & \textit{Std}           & \textit{Simple}        & -0.03 \\
SCAN     & SCAN   & \textit{MCD1}       & \textit{Jump}          & 0.21 & COGS     & SCAN   & \textit{Length}        & \textit{TurnLeftRStr}  & -0.03 \\
SCAN     & Spider & \textit{MCD2}       & \textit{Template}      & 0.2  & SCAN     & Spider & \textit{TurnLeftRStr}  & \textit{Length}        & -0.03 \\
GeoQuery & SCAN   & \textit{Std}        & \textit{MCD2}          & 0.2  & GeoQuery & SCAN   & \textit{TMCD}          & \textit{MCD3}          & -0.03 \\
COGS     & SCAN   & \textit{RandStr}    & \textit{TurnLeftRcvcv} & 0.2  & SCAN     & Spider & \textit{MCD1}          & \textit{TMCD}          & -0.03 \\
SCAN     & SCAN   & \textit{Simple}     & \textit{TurnLeft}      & 0.2  & GeoQuery & SCAN   & \textit{TMCD-Rcvcv}    & \textit{Simple}        & -0.04 \\
SCAN     & Spider & \textit{MCD1}       & \textit{Rand}          & 0.19 & GeoQuery & SCAN   & \textit{Template}      & \textit{MCD3}          & -0.04 \\
SCAN     & Spider & \textit{MCD2}       & \textit{TMCD}          & 0.19 & GeoQuery & SCAN   & \textit{TMCD}          & \textit{Length}        & -0.04 \\
GeoQuery & Spider & \textit{Std-Rcvcv}  & \textit{Rand}          & 0.18 & COGS     & SCAN   & \textit{RandStr}       & \textit{Length}        & -0.04 \\
GeoQuery & SCAN   & \textit{TMCD-Rcvcv} & \textit{Template}      & 0.18 & SCAN     & SCAN   & \textit{MCD3}          & \textit{Template}      & -0.05 \\
COGS     & Spider & \textit{RandStr}    & \textit{Rand}          & 0.18 & GeoQuery & SCAN   & \textit{TMCD-Rcvcv}    & \textit{TurnLeftRcvcv} & -0.05 \\
GeoQuery & SCAN   & \textit{TMCD-Rstr}  & \textit{Template}      & 0.18 & GeoQuery & SCAN   & \textit{Std-Rcvcv}     & \textit{Simple}        & -0.06 \\
SCAN     & SCAN   & \textit{MCD3}       & \textit{Jump}          & 0.18 & GeoQuery & SCAN   & \textit{Std}           & \textit{MCD3}          & -0.06 \\
GeoQuery & SCAN   & \textit{TMCD}       & \textit{MCD2}          & 0.18 & SCAN     & Spider & \textit{MCD3}          & \textit{Template}      & -0.06 \\
SCAN     & Spider & \textit{MCD2}       & \textit{Length}        & 0.18 & COGS     & SCAN   & \textit{Randcvcv}      & \textit{MCD3}          & -0.06 \\
GeoQuery & SCAN   & \textit{Template}   & \textit{MCD2}          & 0.17 & GeoQuery & SCAN   & \textit{TMCD-Rstr}     & \textit{TurnLeftRStr}  & -0.06 \\
SCAN     & SCAN   & \textit{MCD3}       & \textit{TurnLeft}      & 0.17 & GeoQuery & SCAN   & \textit{Template}      & \textit{Length}        & -0.06 \\
COGS     & Spider & \textit{Std}        & \textit{Rand}          & 0.17 & COGS     & SCAN   & \textit{Length}        & \textit{Simple}        & -0.07 \\
GeoQuery & Spider & \textit{Std-Rcvcv}  & \textit{Length}        & 0.17 & SCAN     & SCAN   & \textit{Length}        & \textit{Template}      & -0.07 \\
COGS     & Spider & \textit{RandStr}    & \textit{Length}        & 0.15 & SCAN     & Spider & \textit{MCD3}          & \textit{TMCD}          & -0.07 \\
GeoQuery & SCAN   & \textit{Std-Rstr}   & \textit{TurnLeftRStr}  & 0.15 & GeoQuery & SCAN   & \textit{Std}           & \textit{Length}        & -0.07 \\
COGS     & SCAN   & \textit{RandStr}    & \textit{MCD2}          & 0.15 & SCAN     & Spider & \textit{Length}        & \textit{Template}      & -0.07 \\
SCAN     & SCAN   & \textit{Length}     & \textit{TurnLeftRcvcv} & 0.14 & COGS     & SCAN   & \textit{RandStr}       & \textit{MCD3}          & -0.07 \\
COGS     & SCAN   & \textit{Std}        & \textit{Length}        & 0.14 & GeoQuery & SCAN   & \textit{Length}        & \textit{MCD3}          & -0.08 \\
COGS     & SCAN   & \textit{RandStr}    & \textit{Template}      & 0.14 & SCAN     & Spider & \textit{MCD3}          & \textit{Rand}          & -0.08 \\
COGS     & Spider & \textit{Std}        & \textit{Length}        & 0.14 & COGS     & SCAN   & \textit{Randcvcv}      & \textit{MCD1}          & -0.09 \\
GeoQuery & SCAN   & \textit{TMCD-Rcvcv} & \textit{Length}        & 0.14 & GeoQuery & SCAN   & \textit{Length}        & \textit{Length}        & -0.09 \\
COGS     & SCAN   & \textit{Std}        & \textit{Template}      & 0.13 & SCAN     & Spider & \textit{Length}        & \textit{TMCD}          & -0.09 \\
GeoQuery & SCAN   & \textit{Std-Rcvcv}  & \textit{Template}      & 0.13 & SCAN     & SCAN   & \textit{MCD1}          & \textit{TurnLeftRStr}  & -0.09 \\
COGS     & SCAN   & \textit{Randcvcv}   & \textit{MCD2}          & 0.13 & SCAN     & Spider & \textit{Length}        & \textit{Rand}          & -0.1  \\
GeoQuery & SCAN   & \textit{TMCD-Rstr}  & \textit{Length}        & 0.12 & SCAN     & Spider & \textit{TurnLeftRStr}  & \textit{Template}      & -0.11 \\
SCAN &
  SCAN &
  \textit{Length} &
  \textit{TurnLeftRStr} &
  0.12 &
  GeoQuery &
  SCAN &
  \textit{Std-Rcvcv} &
  \textit{TurnLeftRcvcv} &
  -0.11 \\
COGS     & SCAN   & \textit{Std}        & \textit{MCD3}          & 0.12 & SCAN     & SCAN   & \textit{Simple}        & \textit{MCD1}          & -0.11 \\
GeoQuery & SCAN   & \textit{Std-Rcvcv}  & \textit{Length}        & 0.12 & SCAN     & Spider & \textit{TurnLeftRStr}  & \textit{TMCD}          & -0.12 \\
GeoQuery & SCAN   & \textit{TMCD-Rstr}  & \textit{MCD1}          & 0.11 & SCAN     & Spider & \textit{Simple}        & \textit{Rand}          & -0.12 \\
COGS     & Spider & \textit{Randcvcv}   & \textit{Rand}          & 0.11 & COGS     & SCAN   & \textit{Length}        & \textit{TurnLeftRcvcv} & -0.12 \\
GeoQuery & SCAN   & \textit{TMCD-Rcvcv} & \textit{MCD3}          & 0.11 & GeoQuery & SCAN   & \textit{TMCD-Rstr}     & \textit{Simple}        & -0.13 \\
GeoQuery & SCAN   & \textit{Std-Rcvcv}  & \textit{MCD3}          & 0.11 & SCAN     & SCAN   & \textit{MCD1}          & \textit{TurnLeftRcvcv} & -0.13 \\
GeoQuery & SCAN   & \textit{TMCD-Rstr}  & \textit{MCD3}          & 0.11 & SCAN     & SCAN   & \textit{Simple}        & \textit{Template}      & -0.13 \\
GeoQuery & SCAN   & \textit{Std-Rcvcv}  & \textit{MCD1}          & 0.1  & SCAN     & Spider & \textit{TurnLeftRStr}  & \textit{Rand}          & -0.14 \\
GeoQuery & SCAN   & \textit{Std-Rstr}   & \textit{MCD1}          & 0.1  & GeoQuery & SCAN   & \textit{TMCD-Rstr}     & \textit{TurnLeftRcvcv} & -0.14 \\
GeoQuery & SCAN   & \textit{Std-Rstr}   & \textit{Simple}        & 0.09 & SCAN     & Spider & \textit{Simple}        & \textit{Template}      & -0.15 \\
GeoQuery & SCAN   & \textit{Std-Rstr}   & \textit{Length}        & 0.09 & SCAN     & SCAN   & \textit{TurnLeftRStr}  & \textit{Template}      & -0.15 \\
GeoQuery &
  SCAN &
  \textit{Std-Rstr} &
  \textit{TurnLeftRcvcv} &
  0.08 &
  SCAN &
  Spider &
  \textit{TurnLeftRcvcv} &
  \textit{Length} &
  -0.15 \\ 
COGS     & SCAN   & \textit{Randcvcv}   & \textit{Template}      & 0.08 & GeoQuery & SCAN   & \textit{Std}           & \textit{TurnLeftRStr}  & -0.15 \\
SCAN     & SCAN   & \textit{MCD2}       & \textit{TurnLeftRStr}  & 0.08 & SCAN     & Spider & \textit{Simple}        & \textit{TMCD}          & -0.16 \\
SCAN     & SCAN   & \textit{Simple}     & \textit{Length}        & 0.08 & GeoQuery & SCAN   & \textit{Length}        & \textit{MCD1}          & -0.18 \\
COGS     & Spider & \textit{Randcvcv}   & \textit{Length}        & 0.07 & GeoQuery & SCAN   & \textit{Std}           & \textit{Simple}        & -0.19 \\
SCAN     & SCAN   & \textit{MCD2}       & \textit{TurnLeftRcvcv} & 0.07 & SCAN     & Spider & \textit{TurnLeftRcvcv} & \textit{Template}      & -0.2  \\
SCAN     & SCAN   & \textit{MCD3}       & \textit{TurnLeftRcvcv} & 0.06 & GeoQuery & SCAN   & \textit{TMCD}          & \textit{TurnLeftRStr}  & -0.21 \\
GeoQuery & SCAN   & \textit{Length}     & \textit{MCD2}          & 0.06 & GeoQuery & SCAN   & \textit{Template}      & \textit{TurnLeftRStr}  & -0.21 \\
SCAN     & SCAN   & \textit{Simple}     & \textit{MCD2}          & 0.05 & SCAN     & Spider & \textit{TurnLeftRcvcv} & \textit{TMCD}          & -0.22 \\
GeoQuery & SCAN   & \textit{TMCD-Rcvcv} & \textit{MCD1}          & 0.05 & GeoQuery & SCAN   & \textit{Length}        & \textit{TurnLeftRStr}  & -0.24 \\
SCAN     & SCAN   & \textit{MCD3}       & \textit{TurnLeftRStr}  & 0.05 & GeoQuery & SCAN   & \textit{Std}           & \textit{TurnLeftRcvcv} & -0.25 \\
SCAN     & SCAN   & \textit{Jump}       & \textit{TurnLeftRStr}  & 0.05 & SCAN     & SCAN   & \textit{TurnLeftRcvcv} & \textit{Template}      & -0.26 \\
SCAN     & Spider & \textit{MCD2}       & \textit{Rand}          & 0.05 & GeoQuery & SCAN   & \textit{TMCD}          & \textit{Simple}        & -0.26 \\
SCAN     & Spider & \textit{TurnLeft}   & \textit{Length}        & 0.05 & GeoQuery & SCAN   & \textit{Template}      & \textit{Simple}        & -0.27 \\
GeoQuery & SCAN   & \textit{Std-Rstr}   & \textit{MCD3}          & 0.05 & SCAN     & Spider & \textit{TurnLeftRcvcv} & \textit{Rand}          & -0.27 \\
SCAN     & SCAN   & \textit{MCD2}       & \textit{Template}      & 0.04 & GeoQuery & SCAN   & \textit{Length}        & \textit{TurnLeftRcvcv} & -0.28 \\
COGS     & SCAN   & \textit{Length}     & \textit{MCD1}          & 0.04 & GeoQuery & SCAN   & \textit{TMCD}          & \textit{TurnLeftRcvcv} & -0.29 \\
COGS     & SCAN   & \textit{Std}        & \textit{TurnLeftRStr}  & 0.03 & GeoQuery & SCAN   & \textit{Template}      & \textit{TurnLeftRcvcv} & -0.3  \\
GeoQuery & SCAN   & \textit{Template}   & \textit{MCD1}          & 0.02 & GeoQuery & SCAN   & \textit{Length}        & \textit{Simple}        & -0.3     
\\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Concurrence Values (Cont).}
\label{tab:app:allconur}
\end{table*}

==> CompositionalitySub_arXiv/tables/app_all_perf.tex <==

\begin{table*}[ht]
\centering
\scriptsize
\begin{adjustbox}{max width=0.9\textwidth}
\begin{tabular}{clrlrlrlrlrlrlr}
\toprule
\textbf{Dataset} &
  \textbf{Split} &
  \multicolumn{2}{c}{\textbf{LSTM Uni}} &
  \multicolumn{2}{c}{\textbf{LSTM Bi}} &
  \multicolumn{2}{c}{\textbf{Transformer}} &
  \multicolumn{2}{c}{\textbf{T5}} &
  \multicolumn{2}{c}{\textbf{BART}} &
  \multicolumn{2}{c}{\textbf{BTG}} &
  \multicolumn{1}{c}{\textbf{Avg}} \\ \midrule
\multirow{7}{*}{COGS}   & \textit{Std-Test}      & 99.3  & ±.0  & 99.1  & ±.01 & 99.5  & ±.0  & 99.7 & ±.0  & 99.7  & ±.0  & 68.8 & ±.01 & 94.3 \\
                        & \textit{Rcvcv-Test}    & 99.4  & ±.0  & 99.1  & ±.0  & 99.5  & ±.0  & 99.7 & ±.0  & 99.7  & ±.0  & 68.1 & ±.0  & 94.2 \\
                        & \textit{Rstr-Test}     & 99.4  & ±.0  & 99.0  & ±.01 & 99.6  & ±.0  & 99.8 & ±.0  & 99.7  & ±.0  & 68.4 & ±.0  & 94.3 \\
                        & \textit{Std-Gen}       & 21.3  & ±.05 & 14.8  & ±.08 & 56.1  & ±.06 & 82.9 & ±.0  & 78.6  & ±.0  & 2.8  & ±.01 & 42.8 \\
                        & \textit{Rcvcv-Gen}     & 22.6  & ±.04 & 10.1  & ±.02 & 57.6  & ±.02 & 50.0 & ±.02 & 44.5  & ±.07 & 0.0  & ±.0  & 30.8 \\
                        & \textit{Rstr-Gen}      & 22.3  & ±.07 & 14.7  & ±.03 & 56.6  & ±.03 & 48.0 & ±.01 & 33.5  & ±.03 & 0.0  & ±.0  & 29.2 \\
                        & \textit{Length}        & 20.7  & ±.01 & 24.9  & ±.01 & 28.7  & ±.02 & 37.9 & ±.0  & 34.1  & ±.01 & 20.5 & ±.0  & 27.8 \\ \midrule
\multirow{10}{*}{SCAN}  & \textit{Simple}        & 99.9  & ±.0  & 99.9  & ±.0  & 100.0 & ±.0  & 94.9 & ±.01 & 99.1  & ±.01 & 12.3 & ±.01 & 84.4 \\
                        & \textit{Jump}          & 0.4   & ±.01 & 0.0   & ±.0  & 0.1   & ±.0  & 95.0 & ±.01 & 0.4   & ±.01 & 0.0  & ±.0  & 16.0 \\
                        & \textit{Template}      & 0.2   & ±.0  & 0.3   & ±.01 & 1.1   & ±.0  & 34.3 & ±.03 & 0.0   & ±.0  & 0.9  & ±.01 & 6.1  \\
                        & \textit{MCD1}          & 5.9   & ±.06 & 12.2  & ±.07 & 1.1   & ±.0  & 24.6 & ±.01 & 0.4   & ±.01 & 1.8  & ±.01 & 7.7  \\
                        & \textit{MCD2}          & 6.7   & ±.03 & 5.8   & ±.03 & 1.2   & ±.0  & 34.1 & ±.01 & 1.6   & ±.0  & 0.5  & ±.0  & 8.3  \\
                        & \textit{MCD3}          & 8.7   & ±.04 & 7.8   & ±.02 & 0.7   & ±.0  & 11.1 & ±.01 & 1.2   & ±.01 & 0.8  & ±.01 & 5.0  \\
                        & \textit{Length}        & 15.3  & ±.04 & 11.8  & ±.01 & 0.0   & ±.0  & 14.1 & ±.01 & 0.7   & ±.01 & 0.0  & ±.0  & 7.0  \\
                        & \textit{TurnLeft}      & 61.1  & ±.13 & 34.1  & ±.06 & 64.8  & ±.11 & 70.3 & ±.12 & 63.1  & ±.19 & 8.9  & ±.01 & 50.4 \\
                        & \textit{TurnLeftRcvcv} & 69.4  & ±.14 & 42.8  & ±.14 & 60.4  & ±.12 & 20.0 & ±.03 & 37.7  & ±.15 & 3.5  & ±.01 & 39.0 \\
                        & \textit{TurnLeftRStr}  & 59.0  & ±.18 & 43.5  & ±.1  & 61.9  & ±.1  & 17.7 & ±.02 & 23.9  & ±.17 & 2.4  & ±.0  & 34.7 \\ \midrule
\multirow{4}{*}{NACS}   & \textit{Simple}        & 100.0 & ±.0  & 100.0 & ±.0  & 100.0 & ±.0  & 94.6 & ±.0  & 100.0 & ±.0  & 6.1  & ±.01 & 83.5 \\
                        & \textit{Jump}          & 0.1   & ±.0  & 0.2   & ±.0  & 0.2   & ±.0  & 95.8 & ±.01 & 67.6  & ±.04 & 0.0  & ±.0  & 27.3 \\
                        & \textit{TurnLeft}      & 63.3  & ±.12 & 62.0  & ±.13 & 54.4  & ±.11 & 64.9 & ±.04 & 82.4  & ±.13 & 9.2  & ±.01 & 56.0 \\
                        & \textit{Length}        & 12.7  & ±.02 & 13.2  & ±.01 & 0.0   & ±.0  & 14.3 & ±.0  & 9.3   & ±.02 & 0.0  & ±.0  & 8.2  \\ \midrule
\multirow{4}{*}{Spider} & \textit{Rand}          & 33.4  & ±.02 & 36.9  & ±.01 & 42.5  & ±.01 & 68.0 & ±.0  & 32.7  & ±.01 & 40.1 & ±.01 & 42.3 \\
                        & \textit{Template}      & 1.0   & ±.0  & 2.2   & ±.01 & 4.6   & ±.0  & 39.6 & ±.01 & 21.6  & ±.01 & 1.9  & ±.0  & 11.8 \\
                        & \textit{TMCD}          & 4.6   & ±.01 & 6.0   & ±.01 & 7.5   & ±.01 & 47.2 & ±.01 & 31.2  & ±.03 & 5.5  & ±.0  & 17.0 \\
                        & \textit{Length}        & 12.7  & ±.01 & 14.0  & ±.01 & 17.5  & ±.01 & 35.4 & ±.01 & 7.4   & ±.0  & 14.0 & ±.01 & 16.8 \\ \midrule
\multirow{8}{*}{GeoQuery} &
  \textit{Std} &
  74.0 &
  ±.06 &
  78.9 &
  ±.04 &
  82.3 &
  ±.02 &
  92.5 &
  ±.01 &
  89.2 &
  ±.01 &
  79.0 &
  ±.01 &
  82.6 \\
                        & \textit{Std-Rcvcv}     & 76.7  & ±.03 & 78.9  & ±.02 & 80.5  & ±.01 & 89.4 & ±.0  & 84.2  & ±.0  & 69.0 & ±.03 & 79.8 \\
                        & \textit{Std-Rstr}      & 77.1  & ±.01 & 78.6  & ±.02 & 82.7  & ±.01 & 88.8 & ±.01 & 79.9  & ±.0  & 65.8 & ±.01 & 78.8 \\
                        & \textit{Template}      & 46.5  & ±.06 & 55.9  & ±.07 & 56.7  & ±.04 & 91.0 & ±.0  & 77.1  & ±.06 & 53.5 & ±.06 & 63.5 \\
                        & \textit{Length}        & 18.5  & ±.03 & 16.2  & ±.02 & 22.0  & ±.01 & 41.1 & ±.01 & 36.1  & ±.01 & 20.7 & ±.02 & 25.8 \\
                        & \textit{TMCD}          & 35.8  & ±.02 & 37.1  & ±.02 & 37.9  & ±.01 & 54.1 & ±.0  & 48.2  & ±.0  & 36.9 & ±.0  & 41.7 \\
                        & \textit{TMCD-Rcvcv}    & 35.9  & ±.01 & 36.7  & ±.01 & 37.5  & ±.0  & 43.3 & ±.0  & 40.8  & ±.01 & 34.3 & ±.0  & 38.1 \\
                        & \textit{TMCD-Rstr}     & 35.5  & ±.01 & 37.7  & ±.01 & 37.6  & ±.0  & 43.1 & ±.0  & 41.4  & ±.0  & 35.3 & ±.01 & 38.4     \\
                        \bottomrule
\end{tabular}
\end{adjustbox}
    \caption{Model exact-match accuracy on datasets averaged across random seeds, with standard deviation.}%
\label{app:tab:all-perf}
\end{table*}

==> CompositionalitySub_arXiv/tables/app_dataset_examples.tex <==
\begin{table*}[ht]
\scriptsize
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{p{4em}p{5em}p{0.8\textwidth}}
\toprule
\multirow{2}{*}{\textbf{COGS}} & \textbf{Input:} & Mila liked that the cake was offered to Emma . \\
& \textbf{Output:} & \texttt{* cake ( x \_ 4 ) ; like . agent ( x \_ 1 , Mila ) AND like . ccomp ( x \_ 1 , x \_ 6 ) AND offer . theme ( x \_ 6 , x \_ 4 ) AND offer . recipient ( x \_ 6 , Emma )}
\\ \midrule
\multirow{2}{*}{\textbf{SCAN}}  &  \textbf{Input:} & turn left after jump twice \\
 & \textbf{Output:} & \texttt{I\_JUMP I\_JUMP I\_TURN\_LEFT}
\\ \midrule
\multirow{2}{*}{\textbf{NACS}}  &  \textbf{Input:} & run thrice after jump around left \\
 & \textbf{Output:} & \texttt{I\_TURN\_LEFT I\_JUMP I\_TURN\_LEFT I\_JUMP I\_TURN\_LEFT I\_JUMP I\_TURN\_LEFT I\_JUMP I\_RUN I\_RUN I\_RUN}
\\ \midrule
\multirow{2}{*}{\textbf{GeoQuery}}  &  \textbf{Input:} & how much population does m0 have \\
&  \textbf{Output:} & \texttt{answer ( intersection ( river , loc\_2 ( m0 ) ) )} \\ \midrule
\multirow{2}{*}{\textbf{Spider}}  &  \textbf{Input:} & flight\_1: what is the average distance and price for all flights from la?  \\
&  \textbf{Output:} & \texttt{select avg(distance) , avg(price) from flight where origin = "los angeles"} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Examples of instances in each dataset used in our experiments.}\label{tab:examples}

\end{table*}

==> CompositionalitySub_arXiv/tables/app_genbench_eval_card.tex <==
\newcommand{\tabularwidth}{\textwidth}

\newcommand{\expone}{$\square$}
\newcommand{\exptwo}{$\bigtriangleup$}
\newcommand{\expthree}{$\bigcirc$}
\newcommand{\expfour}{$\odot$}
        
\renewcommand{\arraystretch}{1.1}         
\setlength{\tabcolsep}{0mm}        
\begin{table*}[ht]
\begin{adjustbox}{max width=\textwidth}

\begin{tabular}{|p{\tabularwidth}<{\centering}|}         
\hline
               
\rowcolor{gray!60}               
\textbf{Motivation} \\               
\footnotesize
\begin{tabular}{p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering}}                        
\textit{Practical} & \textit{Cognitive} & \textit{Intrinsic} & \textit{Fairness}\\
& \expone\hspace{0.8mm}\exptwo\hspace{0.8mm}\expthree\hspace{0.8mm}\expfour\hspace{0.8mm}		%
& 		%
& 		%

\vspace{2mm} \\
\end{tabular}\\
               
\rowcolor{gray!60}               
\textbf{Generalisation type} \\               
\footnotesize
\begin{tabular}{m{0.21\tabularwidth}<{\centering} m{0.2\tabularwidth}<{\centering} m{0.13\tabularwidth}<{\centering} m{0.13\tabularwidth}<{\centering} m{0.13\tabularwidth}<{\centering} m{0.2\tabularwidth}<{\centering}}                   
\textit{Compositional} & \textit{Structural} & \textit{Cross Task} & \textit{Cross Language} & \textit{Cross Domain} & \textit{Robustness}\\
\expone\hspace{0.8mm}\exptwo\hspace{0.8mm}\expthree\hspace{0.8mm}\expfour\hspace{0.8mm}		%
& 		%
& 		%
& 		%
& 		%
& 		%

\vspace{2mm} \\
\end{tabular}\\
             
\rowcolor{gray!60}             
\textbf{Shift type} \\             
\footnotesize
\begin{tabular}{p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering}}                        
\textit{Covariate} & \textit{Label} & \textit{Full} & \textit{Assumed}\\  
\expone\hspace{0.8mm}\exptwo\hspace{0.8mm}\expthree\hspace{0.8mm}\expfour\hspace{0.8mm}		%
& 		%
& 		%
& 		%

\vspace{2mm} \\
\end{tabular}\\
             
\rowcolor{gray!60}             
\textbf{Shift source} \\             
\footnotesize
\begin{tabular}{p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering}}                          
\textit{Naturally occuring} & \textit{Partitioned natural} & \textit{Generated shift} & \textit{Fully generated}\\
& \expone\hspace{0.8mm}\exptwo\hspace{0.8mm}		%
& 		%
& \hspace{11mm}\expthree\hspace{0.8mm}\expfour\hspace{0.8mm}		%

\vspace{2mm} \\
\end{tabular}\\
             
\rowcolor{gray!60}             
\textbf{Shift locus}\\             
\footnotesize
\begin{tabular}{p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering}}                         
\textit{Train--test} & \textit{Finetune train--test} & \textit{Pretrain--train} & \textit{Pretrain--test}\\
\expone\hspace{0.8mm}\expthree\hspace{0.8mm}		%
& \exptwo\hspace{0.8mm}\expfour\hspace{0.8mm}		%
& 		%
& 		%

\vspace{2mm} \\
\end{tabular} \\
\hline

\end{tabular}
\end{adjustbox}
\caption{A GenBench evaluation card \citep{Hupkes2023} that summarizes our experiments. \expone = Experiments of LSTM and Transformer on GeoQuery and Spider; \exptwo = Experiments of T5 and BART on GeoQuery and Spider; \expthree = Experiments of LSTM and Transformer on COGS and SCAN; \expfour = Experiments of T5 and BART on COGS and SCAN.}
\label{tab:eval_card}
\end{table*}

==> CompositionalitySub_arXiv/tables/app_license.tex <==
\begin{table*}[ht]
\scriptsize
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lll}
\toprule
\textbf{Artifact} & \textbf{License} & \textbf{Intended Usage}                                       \\
\midrule
COGS              & MIT              & A dataset focuses on compositional generalization \\
SCAN & BSD & A dataset focuses on compositional generalization. \\
GeoQuery & ODC-BY 1.0 license & A database query datasets for U.S. geography. \\
Spider & CC BY-SA 4.0 & A cross-domain semantic parsing and text-to-SQL dataset. \\ 
NACS & CC-NC & A dataset focuses on compositional generalization. \\ \midrule
Neural-BTG              & MIT       & \begin{tabular}[c]{@{}l@{}}A neural transducer for sequence-to-sequence tasks.\end{tabular}   \\
\begin{tabular}[c]{@{}l@{}}LSTM, Transformer \\ (OpenNMT-py \cite{klein-etal-2017-opennmt}) \end{tabular}           & MIT       &  Models for  sequence-to-sequence tasks. \\
T5              & Apache-2.0       & \begin{tabular}[c]{@{}l@{}}A pre-trained model for sequence-to-sequence tasks.\end{tabular}   \\
BART              & Apache-2.0       & \begin{tabular}[c]{@{}l@{}}A pre-trained model for sequence-to-sequence tasks.\end{tabular}   \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{License and intended usage for the artifacts we used.}
\label{app:tab:licenses}
\end{table*}

==> CompositionalitySub_arXiv/tables/app_spider_table.tex <==
\begin{table}[H]
\centering
\scriptsize
\begin{tabular}{p{0.1\columnwidth}p{0.09\columnwidth}p{0.09\columnwidth}p{0.09\columnwidth}p{0.09\columnwidth}p{0.09\columnwidth}p{0.09\columnwidth}}
\toprule
\textbf{Split} &
   \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}LSTM\\  Uni\end{tabular}}} &
  \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}LSTM\\  Bi\end{tabular}}} &
  \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Trans-\\ former\end{tabular}}} &
  \multicolumn{1}{l}{\textbf{T5}} &
  \multicolumn{1}{l}{\textbf{BART}} &
  \multicolumn{1}{l}{\textbf{BTG}} \\ \midrule
\textit{Rand}     & 0.0 & 0.0 & 0.0 & 77.8 & 34.8 & 46.2 \\
\textit{Template} & 1.4 & 2.7 & 3.2 & 52.5 & 25.5 & 3.5  \\
\textit{TMCD}     & 0.1 & 0.1 & 0.1 & 57.6 & 37.9 & 6.9  \\
\textit{Length}   & 0.9 & 0.6 & 0.3 & 44.4 & 9.0  & 16.5 \\ \bottomrule
\end{tabular}
\caption{Model exact-match accuracy with Spider EM. A large amount of output of LSTM and Transformer are deemed as invalid SQL due to special tokens.}
\label{tab:app:spider-perf}
\end{table}

==> CompositionalitySub_arXiv/tables/app_split_intro.tex <==
\begin{table*}[ht]
\small
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lll}
\toprule
\textbf{Split} & \textbf{Dataset} & \textbf{Description}                                       \\
\midrule
\textit{random/standard/simple}              & COGS, SCAN, GeoQuery, Spider              & Split the dataset randomly. \\
\textit{length} & COGS, SCAN, GeoQuery, Spider & Split the dataset according to the input length. \\
\textit{template} & SCAN, GeoQuery, Spider & Split the dataset based on a given string template. \\
\textit{TurnLeft} & SCAN & Compositional commands of \texttt{TurnLeft} are isolated in training set. \\
\textit{Jump} & SCAN & Compositional commands of \texttt{Jump} are isolated in training set. \\
\textit{MCD} & SCAN & Split according to maximum compound divergence. \\
\textit{TMCD} & GeoQuery, Spider & Natural counterpart of MCD, split the data based on target MCD. \\
\textit{Gen} & COGS & \begin{tabular}[c]{@{}l@{}}Not a splitting strategy, but a collection of specially generated samples \\ designed to test 21 cases of generalization in COGS. \end{tabular}
 \\

\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Summary of each split and their designated dataset we use.}
\label{app:tab:splitintro}
\end{table*}

==> CompositionalitySub_arXiv/tables/concurrence_table.tex <==
\begin{table}[t]
\centering
\scriptsize
\begin{tabular}{llllc}
\toprule
\textbf{Dataset A} & \textbf{Dataset B} & \textbf{Split A} & \textbf{Split B} & \textbf{Concur} \\ \midrule
Spider   & Spider   & \textit{Template} & \textit{TMCD}     & 0.88 \\
GeoQuery & Spider   & \textit{Std}      & \textit{Template} & 0.84 \\
GeoQuery & Spider   & \textit{Std}      & \textit{TMCD}     & 0.83 \\
SCAN     & Spider   & \textit{Template} & \textit{Rand}     & 0.76 \\
SCAN     & Spider   & \textit{Template} & \textit{Length}   & 0.76 \\
Spider   & Spider   & \textit{Rand}     & \textit{Length}   & 0.75 \\
GeoQuery & Spider   & \textit{Template} & \textit{Template} & 0.74 \\
GeoQuery & Spider   & \textit{Template} & \textit{TMCD}     & 0.73 \\
GeoQuery & GeoQuery & \textit{Std}      & \textit{Template} & 0.73 \\
SCAN     & SCAN     & \textit{Length}   & \textit{MCD3}     & 0.72 \\
\bottomrule
\end{tabular}
\caption{High concurrence values ($\geq 0.7$) among all pairs of dataset splits, excluding self-concurrence.}
\label{tab:concurrence}
\end{table}




==> CompositionalitySub_arXiv/tables/data_examples.tex <==
\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{p{3em}p{4em}p{0.28\textwidth}}
\toprule
\multirow{2}{*}{\textbf{COGS}} & \texttt{Input:} & Mila liked that the cake was offered to Emma . \\
& \texttt{Output:} & \texttt{* cake ( x \_ 4 ) ; like . agent ( x \_ 1 , Mila ) AND like . ccomp ( x \_ 1 , x \_ 6 ) AND offer . theme ( x \_ 6 , x \_ 4 ) AND offer . recipient ( x \_ 6 , Emma )}
\\ \midrule
\multirow{2}{*}{\textbf{SCAN}}  &  \texttt{Input:} & turn left after jump twice \\
 & \texttt{Output:} & \texttt{I\_JUMP I\_JUMP I\_TURN\_LEFT}
\\ \midrule
\multirow{2}{*}{\textbf{GeoQuery }}  &  \texttt{Input:} & how much population does m0 have \\
&  \texttt{Output:} & \texttt{answer ( intersection ( river , loc\_2 ( m0 ) ) )} \\ \midrule
\multirow{2}{*}{\textbf{Spider}}  &  \texttt{Input:} & flight\_1: what is the average distance and price for all flights from la?  \\
&  \texttt{Output:} & \texttt{select avg(distance) , avg(price) from flight where origin = "los angeles"} \\
\bottomrule
\end{tabular}
\caption{Examples of instances in each dataset used in our experiments.}\label{tab:mainexamples}

\end{table}

==> CompositionalitySub_arXiv/tables/harmless_error_example.tex <==
\begin{table*}[ht]
\scriptsize
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{p{7em}p{0.8\textwidth}}
\toprule
\textbf{Example 1.}  & BART on GeoQuery \textit{standard} and \textit{template} \\
\textbf{Input:} & what are the highest points of all the states \\
\textbf{Output:} & answer ( highest ( intersection ( place , loc\_2 ( state ) ) ) ) \\
\textbf{Prediction:} & answer ( highest ( intersection ( place , loc\_2 ( state ) ) ) ) \hlc[cyan!50]{)}  \\
\hline
\textbf{Input:} & what is the adjacent state of m0 \\
\textbf{Output:} & answer ( intersection ( state , next\_to\_2 ( m0 ) ) ) \\
\textbf{Prediction:} & answer ( intersection ( state , next\_to\_2 ( m0 ) ) ) \hlc[cyan!50]{)} \\ \midrule
\textbf{Example 2.}  & BTG on GeoQuery \textit{simple} and \textit{TurnLeft} \\
\textbf{Input:} & run left thrice and look opposite right thrice \\
\textbf{Output:} & TURN\_LEFT RUN TURN\_LEFT RUN TURN\_LEFT RUN TURN\_\hlc[cyan!50]{RIGHT} TURN\_\hlc[cyan!50]{RIGHT} LOOK TURN\_\hlc[cyan!50]{RIGHT} TURN\_\hl{RIGHT} LOOK TURN\_\hlc[cyan!50]{RIGHT} TURN\_\hlc[cyan!50]{RIGHT} I\_LOOK \\
\textbf{Prediction:} & TURN\_LEFT RUN TURN\_LEFT RUN TURN\_LEFT RUN TURN\_\hlc[cyan!50]{LEFT} TURN\_\hlc[cyan!50]{LEFT} LOOK TURN\_\hlc[cyan!50]{LEFT} TURN\_\hlc[cyan!50]{LEFT} LOOK TURN\_\hlc[cyan!50]{LEFT} TURN\_\hlc[cyan!50]{LEFT} LOOK \\ \hline
\textbf{Input:} & look right after turn left \\
\textbf{Output:} & TURN\_LEFT TURN\_\hlc[cyan!50]{RIGHT} LOOK \\
\textbf{Prediction:} & TURN\_LEFT TURN\_\hlc[cyan!50]{LEFT} LOOK \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Examples of instance where the model makes both mistakes in random split and generalization split. The first instance is the output of BART on \textit{standard} split of GeoQuery, and the second entry is BART making a similar mistake on \textit{template} split of GeoQuery; the second instance is output of BTG on \textit{simple} split of SCAN, and a similar instance making the same directional mistake on the \textit{TurnLeft} split.}
\label{tab:harmless-example}

\end{table*}

==> CompositionalitySub_arXiv/tables/length_split_concurrences.tex <==
\newcommand{\phstar}[0]{\phantom{$^*$}}

\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{llllll}
\toprule
\textbf{Dataset A} & \textbf{Dataset B} & \textbf{Concur} & \textbf{Dataset A} & \textbf{Dataset B} & \textbf{Concur} \\ 
\cmidrule(lr){1-3} \cmidrule(lr){4-6}
COGS      & GeoQuery  & \phstar  0.54  & COGS      & SCAN      & \phstar  0.01  \\
COGS      & Spider    & \phstar  0.26 & SCAN      & Spider    & \phstar  0.01   \\
GeoQuery  & Spider    & \phstar  0.23  & GeoQuery  & SCAN      &  - 0.09  \\
 \bottomrule
\end{tabular}
\caption{Concurrence between length splits of datasets.}
\label{tab:length}
\end{table}



==> CompositionalitySub_arXiv/tables/lexical_split.tex <==
\begin{table}[t]
\begin{subtable}[h]{\the\columnwidth}
    \centering
\scriptsize
\begin{tabular}{llll}
\toprule
\textbf{Dataset}          & \textbf{Split A}          & \textbf{Split B} & \textbf{Concur} \\ \midrule
\multirow{4}{*}{GeoQuery} & \multirow{2}{*}{Std}      & Std-Rcvcv        & 0.69            \\
                          &                           & Std-Rstr         & 0.54            \\
                          & \multirow{2}{*}{TMCD}     & TMCD-Rstr        & 0.65            \\
                          &                           & TMCD-Rcvcv       & 0.63            \\ \midrule
\multirow{2}{*}{COGS}     & \multirow{2}{*}{Std}      & RandStr          & 0.60            \\
                          &                           & Randcvcv         & 0.59            \\ \midrule
\multirow{2}{*}{SCAN}     & \multirow{2}{*}{TurnLeft} & TurnLeftRcvcv    & 0.29            \\
                          &                           & TurnLeftRStr     & 0.23 \\ \bottomrule       
\end{tabular}
\caption{Concurrence between the original split and lexically-processed splits.}
\label{tab:sub:lex-concur}
\end{subtable}
\hfill
\begin{subtable}[h]{\the\columnwidth}

\begin{adjustbox}{max width=\columnwidth}
\scriptsize

\begin{tabular}{lllll}
\toprule
\textbf{Dataset A} & \textbf{Split A} & \textbf{Dataset B} & \textbf{Split B} & \textbf{Concur} \\ \midrule
COGS     & \textit{Length}     & GeoQuery & \textit{TMCD-Rcvcv} & 0.84 \\
GeoQuery & \textit{Std-Rcvcv}  & GeoQuery & \textit{TMCD-Rcvcv} & 0.83 \\
COGS     & \textit{Std}        & GeoQuery & \textit{TMCD-Rcvcv} & 0.82 \\
GeoQuery & \textit{TMCD-Rstr}  & Spider   & \textit{Template}   & 0.82 \\
GeoQuery & \textit{TMCD-Rcvcv} & Spider   & \textit{Template}   & 0.81 \\
COGS     & \textit{Length}     & GeoQuery & \textit{TMCD-Rstr}  & 0.81 \\
COGS     & \textit{Length}     & GeoQuery & \textit{Std-Rcvcv}  & 0.8  \\
GeoQuery & \textit{Std-Rcvcv}  & GeoQuery & \textit{TMCD-Rstr}  & 0.8  \\
\textbf{GeoQuery}  & \textit{\textbf{TMCD-Rstr}}  & \textbf{Spider}    & \textit{\textbf{TMCD}} & \textbf{0.79}   \\
\textbf{GeoQuery}  & \textit{\textbf{TMCD-Rcvcv}} & \textbf{Spider}    & \textit{\textbf{TMCD}} & \textbf{0.79}   \\
COGS     & \textit{Std}        & GeoQuery & \textit{Std-Rcvcv}  & 0.78 \\
GeoQuery & \textit{Std}        & GeoQuery & \textit{TMCD-Rstr}  & 0.77 \\
GeoQuery & \textit{Std}        & GeoQuery & \textit{TMCD-Rcvcv} & 0.75 \\
COGS     & \textit{Std}        & GeoQuery & \textit{TMCD-Rstr}  & 0.74 \\
GeoQuery & \textit{Template}   & Spider   & \textit{TMCD}       & 0.73 \\
GeoQuery & \textit{Std-Rcvcv}  & Spider   & \textit{Template}   & 0.73 \\
COGS     & \textit{RandStr}    & GeoQuery & \textit{Std-Rstr}   & 0.73 \\
COGS     & \textit{Std}        & GeoQuery & \textit{Std-Rstr}   & 0.72 \\
GeoQuery & \textit{Std-Rstr}   & GeoQuery & \textit{TMCD-Rcvcv} & 0.71 \\
GeoQuery & \textit{Std-Rcvcv}  & Spider   & \textit{TMCD}       & 0.71 \\
COGS     & \textit{Randcvcv}   & GeoQuery & \textit{Std-Rstr}   & 0.7  \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{High concurrence values after introducing lexically-processed splits, excluding self-concurrence or concurrence between lexically-processed splits that share the same origin.}
\label{tab:sub:lex-high-concur}
\end{subtable}

\caption{Performance and Concurrence between the lexically-processed splits of datasets.}
\label{tab:lexical}
\end{table}

==> CompositionalitySub_arXiv/tables/num_instances.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lllllll}
\toprule
\textbf{Dataset} & \textbf{Split}          & \textbf{Train} & \textbf{Validation} & \textbf{Test}  & \textbf{Overall} \\
\midrule
\multirow{4}{*}{COGS}     & no\_mod                  & 24155 & 3000       & 3000  & 21000 & 51155   \\
                          & random\_cvcv             & 24155 & 3000       & 3000  & 21000 & 51155   \\
                          & random\_str              & 24155 & 3000       & 3000  & 21000 & 51155   \\
                          & length                   & 24156 & -          & 23999 & -     & 48155   \\
                          \midrule
\multirow{4}{*}{GeoQuery} & standard                 & 600   & -          & 280   & -     & 880     \\
                          & length                   & 440   & -          & 440   & -     & 880     \\
                          & template                 & 441   & -          & 439   & -     & 880     \\
                          & tmcd                     & 440   & -          & 440   & -     & 880     \\
                          \midrule
\multirow{11}{*}{SCAN}    & simple                   & 16728 & -          & 4182  & -     & 20910   \\
                          & length                   & 16990 & -          & 3920  & -     & 20910   \\
                          & mcd1                     & 8365  & 1045       & 1045  & -     & 10455   \\
                          & mcd2                     & 8365  & 1045       & 1045  & -     & 10455   \\
                          & mcd3                     & 8365  & 1045       & 1045  & -     & 10455   \\
                          & addprim\_jump            & 14670 & -          & 7706  & -     & 22376   \\
                          & addprim\_turn\_left      & 21890 & -          & 1208  & -     & 23098   \\
                          & jump\_random\_cvcv       & 14670 & -          & 7706  & -     & 22376   \\
                          & jump\_random\_str        & 14670 & -          & 7706  & -     & 22376   \\
                          & turn\_left\_random\_cvcv & 21890 & -          & 1208  & -     & 23098   \\
                          & turn\_left\_random\_str  & 21890 & -          & 1208  & -     & 23098   \\
                          \midrule
\multirow{4}{*}{Spider}   & random                   & 3282  & -          & 1094  & -     & 4376    \\
                          & length                   & 3282  & -          & 1094  & -     & 4376    \\
                          & template                 & 3280  & -          & 1096  & -     & 4376    \\
                          & tmcd                     & 3282  & -          & 1094  & -     & 4376    \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Number of instances for each dataset in each optimization split.}
\label{tab:num_instances}
\end{table*}

==> CompositionalitySub_arXiv/tables/perf_difference.tex <==
\begin{table}[H]
\scriptsize
\centering
\begin{tabular}{llrrr}
\toprule
\textbf{Dataset}      & \textbf{Split}    & \multicolumn{1}{l}{\textbf{T5}} & \multicolumn{1}{l}{\textbf{BART}} & \multicolumn{1}{l}{\textbf{BTG}} \\ \midrule
\multirow{7}{*}{COGS} & \textit{Std-Test} & 99.7                            & 0.0                               & 0.0                              \\
                          & \textit{Std-Gen}    & 82.9 & 0.0  & 0.0  \\
                          & \textit{Rcvcv-Test} & 99.7 & 0.0  & 0.0  \\
                          & \textit{Rstr-Test}  & 99.8 & 0.0  & 0.0  \\
                          & \textit{Rcvcv-Gen}  & 50.0 & 0.0  & 0.0  \\
                          & \textit{Rstr-Gen}   & 48.0 & 0.0  & 0.0  \\
                          & \textit{Length}     & 37.9 & 0.0  & 0.0  \\ \midrule
\multirow{4}{*}{Spider}   & Rand                & 60.1 & 26.2 & 32.4 \\
                          & Template            & 34.9 & 18.1 & 1.8  \\
                          & TMCD                & 38.3 & 23.5 & 4.9  \\
                          & Length              & 33.9 & 6.1  & 11.9 \\ \midrule
\multirow{8}{*}{GeoQuery} & Std                 & 77.1 & 0.0  & 0.0  \\
                          & Std-Rcvcv           & 74.3 & 0.0  & 0.0  \\
                          & Std-Rstr            & 73.5 & 0.0  & 0.0  \\
                          & Template            & 76.5 & 0.0  & 0.0  \\
                          & Length              & 39.5 & 0.0  & 0.0  \\
                          & TMCD                & 40.7 & 0.0  & 0.0  \\
                          & TMCD-Rcvcv          & 31.6 & 0.0  & 0.0  \\
                          & TMCD-Rstr           & 31.4 & 0.0  & 0.0  \\ \bottomrule
\end{tabular}
\caption{Percentage difference between raw EM implementation and EM implementation that ignore harmless space (space-lenient EM - raw EM). SCAN and NACS are omitted because models do not have this issue on them. LSTMs do not display this issue; the difference for Transformer is under 0.1\% for each datset.}
\label{tab:perf_difference}
\end{table}

==> CompositionalitySub_arXiv/tables/perf_table_v2.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{clrlrlrlrlrlrlr}
\toprule
\textbf{Dataset} &
  \textbf{Split} &
  \multicolumn{2}{c}{\textbf{LSTM Uni}} &
  \multicolumn{2}{c}{\textbf{LSTM Bi}} &
  \multicolumn{2}{c}{\textbf{Transformer}} &
  \multicolumn{2}{c}{\textbf{T5}} &
  \multicolumn{2}{c}{\textbf{BART}} &
  \multicolumn{2}{c}{\textbf{BTG}} &
  \multicolumn{1}{c}{\textbf{Avg}} \\ \midrule
\multirow{2}{*}{COGS}     & \textit{Std-Test} & 99.3 & ±.0  & 99.1 & ±.01 & 99.5  & ±.0  & 99.7 & ±.0  & 99.7 & ±.0  & 68.8 & ±.01 & 94.3 \\
                          & \textit{Std-Gen}  & 21.3 & ±.05 & 14.8 & ±.08 & 56.1  & ±.06 & 82.9 & ±.0  & 78.6 & ±.0  & 2.8  & ±.01 & 42.8 \\ \midrule
\multirow{8}{*}{SCAN}     & \textit{Simple}   & 99.9 & ±.0  & 99.9 & ±.0  & 100.0 & ±.0  & 94.9 & ±.01 & 99.1 & ±.01 & 12.3 & ±.01 & 84.4 \\
                          & \textit{Jump}     & 0.4  & ±.01 & 0.0  & ±.0  & 0.1   & ±.0  & 95.0 & ±.01 & 0.4  & ±.01 & 0.0  & ±.0  & 16.0 \\
                          & \textit{TurnLeft} & 61.1 & ±.13 & 34.1 & ±.06 & 64.8  & ±.11 & 70.3 & ±.12 & 63.1 & ±.19 & 8.9  & ±.01 & 50.4 \\
                          & \textit{Template} & 0.2  & ±.0  & 0.3  & ±.01 & 1.1   & ±.0  & 34.3 & ±.03 & 0.0  & ±.0  & 0.9  & ±.01 & 6.1  \\
                          & \textit{MCD1}     & 5.9  & ±.06 & 12.2 & ±.07 & 1.1   & ±.0  & 24.6 & ±.01 & 0.4  & ±.01 & 1.8  & ±.01 & 7.7  \\
                          & \textit{MCD2}     & 6.7  & ±.03 & 5.8  & ±.03 & 1.2   & ±.0  & 34.1 & ±.01 & 1.6  & ±.0  & 0.5  & ±.0  & 8.3  \\
                          & \textit{MCD3}     & 8.7  & ±.04 & 7.8  & ±.02 & 0.7   & ±.0  & 11.1 & ±.01 & 1.2  & ±.01 & 0.8  & ±.01 & 5.0  \\
                          & \textit{Length}   & 15.3 & ±.04 & 11.8 & ±.01 & 0.0   & ±.0  & 14.1 & ±.01 & 0.7  & ±.01 & 0.0  & ±.0  & 7.0  \\ \midrule
\multirow{4}{*}{GeoQuery} & \textit{Std}      & 74.0 & ±.06 & 78.9 & ±.04 & 82.3  & ±.02 & 92.5 & ±.01 & 89.2 & ±.01 & 79.0 & ±.01 & 82.6 \\
                          & \textit{Template} & 46.5 & ±.06 & 55.9 & ±.07 & 56.7  & ±.04 & 91.0 & ±.0  & 77.1 & ±.06 & 53.5 & ±.06 & 63.5 \\
                          & \textit{TMCD}     & 35.8 & ±.02 & 37.1 & ±.02 & 37.9  & ±.01 & 54.1 & ±.0  & 48.2 & ±.0  & 36.9 & ±.0  & 41.7 \\
                          & \textit{Length}   & 18.5 & ±.03 & 16.2 & ±.02 & 22.0  & ±.01 & 41.1 & ±.01 & 36.1 & ±.01 & 20.7 & ±.02 & 25.8 \\ \midrule
\multirow{4}{*}{Spider}   & \textit{Rand}     & 33.4 & ±.02 & 36.9 & ±.01 & 42.5  & ±.01 & 68.0 & ±.0  & 32.7 & ±.01 & 40.1 & ±.01 & 42.3 \\
                          & \textit{Template} & 1.0  & ±.0  & 2.2  & ±.01 & 4.6   & ±.0  & 39.6 & ±.01 & 21.6 & ±.01 & 1.9  & ±.0  & 11.8 \\
                          & \textit{TMCD}     & 4.6  & ±.01 & 6.0  & ±.01 & 7.5   & ±.01 & 47.2 & ±.01 & 31.2 & ±.03 & 5.5  & ±.0  & 17.0 \\
                          & \textit{Length}   & 12.7 & ±.01 & 14.0 & ±.01 & 17.5  & ±.01 & 35.4 & ±.01 & 7.4  & ±.0  & 14.0 & ±.01 & 16.8
 \\
                        \bottomrule
\end{tabular}
\end{adjustbox}
    \caption{Model exact-match accuracy on datasets averaged across random seeds, with standard deviation.}%
\label{tab:perfStd}
\end{table*}




==> CompositionalitySub_arXiv/tables/space_example.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{p{7em}p{0.8\textwidth}}
\toprule
\textbf{Input:} & Zoe thought that a hippo cleaned . \\
\textbf{Output:} & think\hl{ }. agent ( x \_ 1\hl{ }, Zoe ) AND think\hl{ }. ccomp ( x \_ 1\hl{ }, x \_ 5 ) AND hippo ( x \_ 4 ) AND clean\hl{ }. agent ( x \_ 5\hl{ }, x \_ 4 ) \\
\textbf{Prediction:} & think. agent ( x \_ 1, Zoe ) AND think. ccomp ( x \_ 1, x \_ 5 ) AND hippo ( x \_ 4 ) AND clean. agent ( x \_ 5, x \_ 4 ) \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Examples of instance where the model is only mistaken on the space.}
\label{tab:space-example}

\end{table*}

==> CompositionalitySub_arXiv_2/1_Introduction.tex <==

\input{figures/default_conf_matrix}

Over the past few years, NLP has made astonishing progress on almost all language-related tasks proposed by the community. %
Concurrently, %
a plethora of benchmark datasets has emerged for evaluating the skills of NLP models and exposing their strengths and weaknesses (\citealt{chowdhery-etal-2022-scaling}, \textit{inter alia}).
These datasets focus on a variety of different aspects of model capabilities, that are increasingly not mutually exclusive: oftentimes, multiple benchmarks are available that target the same capability or skill, using (slightly) different metrics, design choices, and/or conceptual approaches. 
For instance, \citet{Hupkes2023} report that many recent studies on generalization  used  different \emph{shift sources} to study the same types of \emph{generalization} (see \cref{fig:generalisation_vs_source}).\footnote{Plot generated using the visualisation tool on \url{https://genbench.org/visualisations}.} 

However, somewhat surprisingly, despite a wealth of work in the domain of evaluation and generalization, there is very little research that assesses whether multiple datasets designed to measure the same ability also yield the same conclusions.
This makes it difficult for practitioners to conduct informed evaluation dataset selection and, perhaps even more concerning, impedes our understanding of how well different datasets measure what they intend to measure.
While establishing \emph{construct validity} and \emph{construct reliability} -- for instance through comparing the results of tests with other tests that intend to measure the same thing -- is common practice in the social sciences \citep{westen2003quantifying, jacobs-wallach-2021-measurement}, it is not the standard in the field of NLP.

In this work, we argue that establishing such standards is much needed in our field, and we present a detailed set of experiments that assesses construct validity in the domain of \emph{compositional generalization}. 
Following \citet{liu2021question}, we use \emph{concurrence} to measure the extent to which 8 different \emph{compositional splitting strategies} for 4 different datasets -- SCAN, GeoQuery, COGS, and Spider -- %
provide similar rankings for 6 different modeling approaches -- BART, T5, Transformer, uni- and biLSTMS, and Neural-BTG.
We find that, in general, the conclusions drawn from one dataset split typically do not align with the results from another dataset split.
In a range of experiments, we explore if that could be attributed to whether the underlying data are synthetic or human-generated, to the compositional splitting strategy is used to create the data (a.k.a.\ what interpretation of compositionality), or to uncontrolled exposure to lexical items that also occurred during pretraining.

We find that concurrence values are generally low: only 10 out of 153 pairs of dataset splits have a concurrence value that surpasses the threshold for high concurrence.
Furthermore, results from human-authored datasets concur much more than results from synthetic datasets.
On the contrary, dataset splits that share the same interpretation of compositionality -- as defined by their splitting strategy -- hardly concur with each other:  the underlying data plays a more important role in model rankings.
Lastly, aligned with the findings of \citet{kim2022uncontrolled}, we find that carefully controlling the lexical items in a compositional split has a positive impact on concurrence.
Overall, our results suggest that much work remains to be done to evaluate compositional generalization, and more generally that having more rigorous standards for establishing the validity of evaluation sets should be prioritized in the future.


\input{figures/generalization_studies}





==> CompositionalitySub_arXiv_2/2_RelatedWork.tex <==
In this section, we provide an overview of datasets commonly used for assessing compositional generalization, and we discuss previous attempts to compare performance across benchmarks.

\paragraph{Datasets for Compositional Generalization}
Since the introduction of \emph{SCAN} in 2018 \citep{lake2018generalization}, many datasets have been proposed to assess compositional generalization in neural networks.
Several of them were direct follow-ups to SCAN that aimed to extend the original dataset or mitigate various issues perceived with it.
For instance, \citet{bastings-etal-2018-jump} introduced NACS, a `reversed' version of SCAN; \citet{loula-etal-2018-rearranging} introduced new splits using the original dataset; \citet{ruis-etal-2020-gscan} introduced a multimodal, grounded version of the benchmark; and \citet{patel-etal-2022-revisiting} increased the number of primitives.
Recently, \citet{valvoda-etal-2022-benchmarking} proposed a transducer-based procedure for generating myriad synthetic datasets similar to SCAN to investigate which formal properties impact the results.
Other artificially generated datasets available to evaluate compositionality are PCFG SET \citep{hupkes2020compositionality}, %
COGS \citep{kim-linzen-2020-cogs}, %
and the dataset proposed by \citet{oren-etal-2021-finding}.

Datasets that use more natural (but often still templated) data are typically situated in the domain of machine translation -- such as \citet{li-etal-2021-compositional}, \citet{dankers-etal-2022-paradox} and \citet{raunak2019compositionality} -- or semantic parsing -- e.g.\ \citet{finegan2018improving,keysers2019measuring,shaw-etal-2021-compositional,cui-etal-2022-compositional}.
Finally, \citet{thrush-etal-2022-winoground} introduce Winoground, aimed to assess compositionality in text-to-image models.
In our work, we focus on datasets that target compositionality in the domain of semantic parsing, with the addition of SCAN for its sheer popularity.


\paragraph{Performance across benchmarks}
Several recent works across NLP have been interested in the extent to which strong performance on one task, setting, or dataset transfers to strong performance on another.
Typically, such experiments are motivated by transfer learning, rather than establishing the validity of evaluation results.
For instance, \citet{vu-etal-2020-exploring}, \citet{ye-etal-2021-crossfit}, \citet{luo-etal-2022-cogtaskonomy}, \citet{padmakumar-etal-2022-exploring}, and \citet{weber-etal-2021-language} all investigate to what extent performance transfers across tasks.
More closely related to our study, is the work presented by \citet{liu2021question}, who quantify the measurement of benchmark agreement on model rankings and compare it in question answering.
In our work, we adopt their definition of comparability across datasets.

In the context of compositional generalization, the work most closely related to ours is the study presented by \citet{chaabouni-etal-2021-transformers}, in which they investigate whether the performance improvements on the synthetic dataset SCAN transfer to the naturalistic setting.
We largely confirm their results, but consider compositionality benchmarks more broadly, not only considering the synthetic v.s\ natural dimension, but also interpretations of compositionality and lexical items exposed during pretraining.







==> CompositionalitySub_arXiv_2/4_ExperimenalSetup.tex <==
We compare how the conclusions drawn from 18 different compositional generalization splits -- defined over 4 different datasets with 8 compositional splitting strategies -- compare across 6 modeling approaches.
In this section, we describe the datasets and modeling approaches we consider and provide details on training and hyperparameter selection.

\subsection{Models}\label{subsec:models}
For our experiments, we consider both pretrained and train-from-scratch approaches that have previously been considered in the context of compositional generalization.

\paragraph{BART \& T5}
We use the pretrained seq2seq models BART \cite{lewis-etal-2020-bart} and T5 \cite{raffel2020exploring} to enable easy comparison with prior work. 
In the case of BART, order-based noising strategies are used, which may encourage the model to learn to better represent linguistic structure. 

\paragraph{LSTM \& Transformer} 
To ensure coverage of models without pre-trained knowledge, we use a uni-directional LSTM \cite{hochreiter1997long}, a bi-directional LSTM, and a vanilla transformer \cite{vaswani2017attention}.

\paragraph{Neural-BTG}
We include one modeling approach specifically designed to address compositionality: Neural-BTG \cite{wang-etal-2022-hierarchical-phrase}, %
composed of a discriminative parser based on a bracketing transduction grammar (BTG; \citealp{wu-1997-stochastic}) %
and a neural seq2seq model. %


\subsection{Data}\label{subsec:data}
We consider four different datasets designed to test compositional generalization.
We focus on datasets for semantic parsing and include SCAN as the most commonly used dataset for compositionality overall.
Three of these datasets contain different curated \emph{splits} that target different interpretations of compositionality.
Two of the datasets (SCAN and COGS) are synthetic datasets that are generated with rules, while the other two (Spider and GeoQuery) are natural datasets, authored by humans.
Examples for all datasets and descriptions of all curated splits can be found in \cref{app:sec:data}.

\input{tables/data_examples}

\paragraph{SCAN} Consisting of a set of commands and the corresponding action sequences, SCAN \cite{lake2018generalization} is one of the most popular synthetic datasets to study compositional generalization.
We include the \textit{simple}, \textit{length}, \textit{add primitive}, \textit{template} splits from \citet{lake2018generalization}.
In addition to original SCAN splits, we also use the maximum compound divergence (MCD) splits of SCAN proposed by \citet{keysers2020measuring}.

\paragraph{COGS} 
\citet{kim-linzen-2020-cogs} introduced COGS, a synthetic semantic parsing dataset generated by a rule-based approach, which covers a larger variety of grammar rules than SCAN does.
The inputs in COGS are English sentences, generated by a probabilistic context-free grammar. 
The corresponding output, which is the semantic interpretation of the input, is annotated with the logical formalism of \citet{reddy-etal-2017-universal}.
COGS includes a randomly sampled test set and an out-of-distribution compositional generalization set.

\paragraph{GeoQuery} GeoQuery \cite{tang2001using, zelle1996learning} is a text-to-QL dataset containing naturalistic examples.
We use the four compositional generalization splits defined on this dataset by \citet{shaw-etal-2021-compositional}: 
\textit{random/standard}, \textit{length}, \textit{template}, and \textit{Target Maximum Compound Divergence (TMCD)}.

\paragraph{Spider} Spider \cite{yu-etal-2018-Spider} is originally designed for cross-domain semantic parsing. %
We use the compositional generalization splits for Spider defined by \citet{shaw-etal-2021-compositional}, which match their splits for GeoQuery: 
\textit{random/standard}, \textit{length}, \textit{template}, and \textit{TMCD}.

\subsection{Training Setup}
We train/fine-tune the models on the train partition of each dataset described above and evaluate them on the corresponding test set.
For T5 on GeoQuery and Spider as well as LSTM and Transformers on COGS, we use the hyperparameters provided in \citet{shaw-etal-2021-compositional} and \citet{kim-linzen-2020-cogs}, respectively. 
We followed \citet{orhan2021compositional} to train T5 and \citet{yao-koller-2022-structural} to train BART on COGS. 
For the remaining model-dataset combinations, we perform a hyperparameter search for each dataset, with 10\% of instances randomly chosen to be used for tuning. 
Details can be found in \cref{app:hp_tuning}. 
We use three different random seeds for each training run and use five random seeds for each training run of LSTM, to compensate for LSTM's higher variation in performance across seeds.
For models with existing evaluations on a dataset, we compare to these previous measures of performance to ensure that our replication results align with previously reported numbers \cite{keysers2020measuring, kim-linzen-2020-cogs, orhan2021compositional, shaw-etal-2021-compositional, yao-koller-2022-structural, sun-etal-2023-resp}.

\subsection{Evaluation}
\label{sec:expsetup:eval}
For most datasets, we use exact match (EM) accuracy.
EM is a binary metric that only counts an output as correct if it matches the target output exactly, and is most frequently used for the datasets we consider.
During initial experiments, we found that, in many cases, EM accuracy may be too strict for our purposes.
In some cases, models' tokenizers may prefer slightly different spacing -- a phenomenon also reported by \citet{sun2022tokenization} -- in others, models lack specific tokens in their vocabulary.
Neither of these things is indicative of a model's compositional generalization capability, and we therefore choose to normalize model outputs before applying EM accuracy.
In \cref{app:sec:EM}, we include examples of such cases, and we report the differences between EM scores with and without our normalization step.
For Spider, the original dataset also uses a more lenient EM implementation.
For consistency reasons, we use the same implementation across all datasets, but we report Spider EM scores in \cref{app:sec:spider} to compare with previous work. 

\subsection{Measuring Concurrence}
To measure how similarly different dataset splits rank different modeling approaches, we use the concept of \emph{concurrence} introduced by \citet{liu2021question}.
The concurrence between two dataset splits is defined as the correlation between the performances of different modeling approaches for those splits.
More specifically, the concurrence $\text{CONCUR}(D_1, D_2; \mathcal{A}, \text{Eval})$ between two dataset splits $D_1$ and $D_2$, given a set of modeling approaches $\mathcal{A}$ and evaluation function $\text{Eval}$, is defined as:%
\begin{equation*}
    \text{CONCUR}(D_1, D_2; \mathcal{A}, \text{Eval})=\text{CORR}(P_1, P_2),
\end{equation*}
where $\text{CORR}$ is some correlation function and $P_i$ is the variable that holds the scores of Eval($a, D_i$) for all $a\in\mathcal{A}$.
For \text{CORR}, \citet{liu2021question} considered both Pearson ($r$) and Kendall rank ($\tau$). 
Because we are interested in how benchmarks rank model performance, we report the concurrence values under Kendall's $\tau$ unless specified otherwise.
We refer to the concurrence between the dataset split and itself as \emph{self-concurrence}, the value of which is purely affected by seed variation across training runs. 
We see self-concurrence, which would be $1.0$ if there is no variation across seeds, as an upper bound for the concurrence values across dataset splits.



==> CompositionalitySub_arXiv_2/5_Findings.tex <==

We now present our results, starting with a discussion of the performance of models on the datasets (\cref{sec:overall_perf}) and the concurrence scores between the performances (\cref{sec:predictivity}), we then proceed to look at the relationship between synthetic and natural compositionality datasets (\cref{sec:synvnat}), and how this interacts with the choice of definition of compositionality and underlying dataset (\cref{sec:comp_def}). We finish our results section with a short investigation into the impact of the choice of lexical items in data (\cref{sec:lex_exposure}).

\input{tables/perf_table_v2}
\subsection{Overall Performance}
\input{Results/1_OverallPerf}


\subsection{Overall Concurrence}
\input{Results/2_Predictivity}

\subsection{Synthetic vs natural data}\label{sec:synvnat}
\input{Results/3_Synthetic_vs_natural}

\subsection{Interpretations of compositionality}
\input{Results/4_CompType}

\subsection{The influence of lexical items}
\label{sec:lex_exposure}
\input{figures/std_v_lex}
\input{tables/lexical_split}
\input{Results/5_Lex_Exposure}

\subsection{Other confounding factors}\label{sec:confounding_factors}
\input{Results/7_other_confounding_factors.tex}










==> CompositionalitySub_arXiv_2/7_Conclusion.tex <==
In this paper, we explored how different evaluation choices impact the conclusions drawn from the experiments evaluating compositionality.
Using compositional generalization datasets and models ranging from trained-from-scratch to pretrained, we conduct a series of experiments to understand whether datasets consistently rank models in terms of their generalizability, and we find little consistency. When we perform further analysis to try to better understand this inconsistency, we find that comparing within the training setting (pretrained v.s.\ trained-from-scratch) or data creation type (synthetically generated v. naturally generated) does not increase consistency.
However, better controlling the lexical items can help us draw more consistent conclusions, at least for datasets that share the same notion of compositionality.
We leave the investigation into how task selection might affect evaluation results for compositional generalization to further research.
Overall, our results suggest that to evaluate compositional generalization consistently, clearer definitions of compositionality are needed, as well as %
more careful consideration of evaluation design and more thorough dataset evaluations.



==> CompositionalitySub_arXiv_2/8_Limitations.tex <==


While we explore the consequences of the modeling approach on concurrence, we have focused mainly on models trained from scratch to perform compositional generalization or pretrained models which have been finetuned. Another possible area of investigation would be to explore the extent to which a model's compositional generalization abilities also transfer to in-context evaluations \citep{hosseini-etal-2022-compositional}. We leave this question for future work.  


==> CompositionalitySub_arXiv_2/Results/1_OverallPerf.tex <==
\label{sec:overall_perf}
In \cref{tab:perfStd}, we show the performance of all models on all dataset splits under consideration, as well as the average performance per dataset split (last column).
Our scores are generally close to the scores reported in previous work, for the (dataset split, architecture) combinations for which previous results exist \citep{sun-etal-2023-resp}, with the exception of the results for Spider, for which we use a different metric.
All models perform reasonably well on the random splits of each datasets (first row for each dataset in \cref{tab:perfStd}), but most struggle with various generalization splits. 
While some splits are difficult across the board, other difficulties appear more model-dependent.
For instance, while all models are weak on the \textit{length} and \textit{MCD} splits of SCAN and \textit{length} split of Spider, COGS is difficult for some models (e.g., BTG) but much less for others (e.g., T5).
Similarly, some models perform well on one of the datasets or one of the splits, but perform poorly on the others. 
BART, for instance, maintains high performance on GeoQuery and COGS, but performs even worse than non-pretrained models on some splits of SCAN, while BTG performs well on GeoQuery but fails on many splits of SCAN.
T5 has high performance on most datasets, but is outperformed by the unidirectional LSTM on the \textit{length} split of SCAN.
SCAN, in particular, appears to be challenging for all models, with the \textit{TurnLeft} split being the only exception.%
\footnote{While architectures exist that obtain high scores on SCAN, such as the ones introduced by \citet{shaw-etal-2021-compositional} and \citet{kim2021sequencetosequence}, they are too narrowly scoped for our current study and we thus do not consider them.}



==> CompositionalitySub_arXiv_2/Results/2_Predictivity.tex <==
\label{sec:predictivity}
\input{tables/concurrence_table}

It is not difficult to tell from Table~\ref{tab:perfStd} that the performance of a model on one dataset is not predictive of its performance on the others.  
To quantitatively substantiate this observation, we compute the concurrences between the different dataset splits, which we visualize in \cref{fig:default_conf_matrix}.
On average, the concurrence between dataset splits is low: a mere $0.22$, far below the average self-concurrence of $0.76$ that (model, split) combinations have across different seeds.
Interestingly, even these average self-concurrence values are lower than the $0.8$ that \citet{liu2021question} used as a threshold for ``high'' concurrence, indicating that performance on the same compositional dataset is not very stable across runs.\footnote{This finding is in line with results reported by \citet{liska2018memorize}, who find a range of different generalization performances on a simple but highly compositional look-up table task.}
Consequently, we lower the threshold to $0.7$ here, which is approximately 90\% of the average self-concurrence.
Of the 153 pairs of dataset split we compare in this experiment, only 10 pairs surpass this threshold.
Somewhat surprisingly, perhaps, many of the highest values (reported in \cref{tab:concurrence}), are concurrences between i.i.d.\ splits and compositional splits.

Considering the concurrence of each dataset with all other datasets (excluding self-concurrence, values are reported below \cref{fig:default_conf_matrix}), we can see that performance COGS, with an average $\tau$ of $0.36$ is most predictive of performance on other datasets.
Furthermore, the three semantic parsing datasets have much higher average concurrence than SCAN, suggesting that compositionality on one task may not be predictive of compositionality on another.







==> CompositionalitySub_arXiv_2/Results/3_Synthetic_vs_natural.tex <==
\input{figures/perf_v_perf}

Why are these concurrence values so low? %
The first hypothesis that we explore is that performance on strongly structured templated data may not correlate with performance on datasets that are authored by humans. To this end, we compute the average concurrence values of three combinations of dataset split pairs, natural-natural, natural-synthetic and synthetic-synthetic, and include an example of each pair type in \cref{fig:perfvperf}. 
We find that splits of natural datasets concur much better than splits of synthetic datasets ($0.54$ v.s.\ $0.22$); the worst is concurrence between synthetic and natural dataset splits ($0.19$).
The same finding can be observed in \cref{fig:perfvconcur}, which we will use later to explore the relationship between concurrence values and performance in \cref{sec:perf:confounding}.

These results are in line with earlier studies that suggested that performance on synthetic compositionality datasets may not transfer to more realistic scenarios \citep{chaabouni-etal-2021-transformers, shaw-etal-2021-compositional}, and underline the point made by \citet{dankers-etal-2022-paradox}, who argue that compositionality should be studied in its natural habitat.
Also the concurrence between dataset splits with naturalistic data is well below the threshold for high concurrence, suggesting that there exist factors beyond dataset creation strategy that can affect how compositionality benchmarks rank modeling approaches.




==> CompositionalitySub_arXiv_2/Results/4_CompType.tex <==
\input{figures/pair_type_bar_plot}
\label{sec:comp_def}

The next hypothesis that we consider is that concurrence values are low because different dataset splits investigate different types of compositionality \citep[cf.][]{hupkes2020compositionality}.
In compositional evaluation datasets, the interpretation of compositionality is operationalized through its \emph{splitting strategy}.
One splitting strategy may, for instance, define compositional generalization as generalization to longer lengths, whereas another instead focuses on generalization to novel vocabulary items.
These different interpretations of compositionality could potentially require different model capabilities.
Could it be that our concurrence values are low because different splits in fact focus on different types of compositional generalization?


To investigate this, we group the concurrence values by four dataset pair types -- different datasets with the same splitting strategy, the same dataset with different splitting strategies, different datasets with different splitting strategies, and the same dataset with the same splitting strategy -- and plot them in \cref{fig:pairtype-bar}.
Predictably, datasets concur most with themselves (red line).
We also see that which data a splitting approach is applied to is more important than the interpretation of compositionality (cyan and dark blue lines, respectively): concurrence between experiments that share the same source of data averages at $0.38$, whereas different data but the same splitting strategy results in an average concurrence of $0.32$.
However, when both the source of data and splitting strategy are different (yellow line), the concurrence values  shift leftward, suggesting that the data type and splitting strategy pose different kinds of difficulties for the modelling approaches considered.

\input{tables/length_split_concurrences}

\paragraph{Length Generalization}
Because not every dataset in previous work applied all the splitting strategies, we follow-up with a small experiment in a split shared across all datasets: \emph{length generalization} splits.\footnote{As the original COGS dataset did not come with a length generalization split, we generate one ourselves.}
The concurrence values between the different length splits, shown in \cref{tab:length}, are generally low, ranging from $-0.09$ to $0.54$ and averaging at 0.16.
This additional experiment confirms that even when benchmarks maintain the same interpretation of compositionality, there may still be substantial differences in model rankings, depending on the underlying data.



==> CompositionalitySub_arXiv_2/Results/5_Lex_Exposure.tex <==

In \cref{tab:perfStd}, we can see that pretrained models achieve the highest accuracies and in \cref{tab:concurrence} that the highest concurrence values are between two natural datasets. 
In this section, we dive into the differences between pretrained and trained-from-scratch models,  and investigate the extent to which those differences affect the concurrence results.
In particular, we investigate whether the presence of uncontrolled lexical exposure during pretraining may impact the performance of pretrained models, implying their accuracy numbers may not solely reflect their compositional abilities, as suggested by \citet{kim2022uncontrolled}.
Were this to happen, a misalignment in the evaluation between pretrained and non-pretrained models would contribute to variation in the concurrence values, where the performance of pretrained models is overestimated due to lexical exposure in pretraining.

To test for possible effects of lexical exposure, we extend the experiment from \citet{kim2022uncontrolled} -- who conducted it for COGS -- to the TMCD and Std split of GeoQueory, and the TurnLeft split of SCAN\footnote{In both these cases, particular lexical items are purposefully left out of the training set, to be evaluated at test time. If those lexical items were also present in the uncontrolled pretraining corpus, this would thus break the test.}
In both cases, we swap out lexical items with strings of similar length that act as ``wug words'' \citep{berko-1958-child}, or, in other words, previously unattested and therefore meaningless lexical items.
Following \citet{kim2022uncontrolled}, we generate the strings in two ways:
\begin{compactitem}
    \item \textit{Rstr:} We randomly sample lowercase characters from the Latin script with replacements.
    \item \textit{Rcvcv:} We alternately sample a vowel after a consonant from the Latin script.
\end{compactitem}

\noindent We train the models on all modified splits and compute the performance (\cref{fig:std_v_lex}). 
We also compute the concurrence between the original split and the modified split (\cref{tab:sub:lex-concur} and \cref{tab:sub:lex-high-concur}).

In \cref{fig:std_v_lex}, we see that the performance of the pretrained models drops drastically when the lexical items are replaced, while the non-pretrained models' performance does not, confirming the results of \citet{kim2022uncontrolled}.
In addition, the concurrence between the original splits and the modified splits for all datasets is below our set threshold -- albeit higher than other comparisons we have seen before (Table~\ref{tab:sub:lex-concur}) -- implying that replacing lexical items results in yet another new ranking of modeling approaches for compositionality.

We then compute the concurrence between the same set of splits before and after the lexical exposure edits: \emph{within} the group of splits that are selected for the lexical changes, the concurrence values decrease from $0.49$ to $0.41$, while the average concurrence values of these splits with \emph{other} splits that haven't undergone lexical edits slightly increase from $0.25$ to $0.26$ (e.g. concurrence between GeoQuery and Spider TMCD splits increases when GeoQuery TMCD split applies the lexical changes), with many more dataset split pairs surpassing the $\tau=0.7$ bar for high concurrence (\cref{tab:sub:lex-high-concur}).

A closer look explains this apparent contrast: the overall low-concurring dataset SCAN -- which makes up 12.5\% of the lexically edited splits, drags down the concurrence values within that group.
Excluding SCAN, the within-group concurrence values also increase, from $0.63$ to $0.66$.
These results do thus not only confirm that controlling lexical exposure is important when evaluating compositionality in pretrained models, but also further exemplify our earlier finding that compositionality scores -- for neural models -- strongly depend task and dataset. We further analyze the influence of tasks to compositionality results in \cref{app:sec:nacs}.




==> CompositionalitySub_arXiv_2/Results/6_Eval_Metric.tex <==



Despite of data source and exposed lexical items, other confounding factors can appear during the evaluation of compositionality.
As we have observed in \cref{fig:default_conf_matrix}, splits of SCAN obtain low concurrence with most of splits from other datasets.
In the mean time, the task of SCAN, grounded navigation, is most distant from the others, which are based on semantic parsing.
This and our finding in \cref{sec:comp_def} are \textit{in pari materia}: the source of data (regardless of the task) contributes more to the resulting model rankings compared to the interpretation of generalization, and gives hints about the degree to which datasets disagree with each other when considering two more distant pairs of datasets in terms of their task.
We leave the investigation on how the selection of specific tasks affect evaluation result of compositionality to further research.

The in-distribution performance may also become a confounder when model performs poorly on the random split of the data.
Qualitatively, we observe that models sometimes make the same trivial mistakes in both a random split and a generalization split, making the evaluation result unrepresentative of compositionality.
We leave such examples in \cref{app:sec:mistakes}.





==> CompositionalitySub_arXiv_2/Results/7_other_confounding_factors.tex <==
\label{sec:perf:confounding}
We have explored a range of factors that may impact the evaluation of compositionality, such as the nature of the underlying data and task, the interpretation of compositionality, and the choice of lexical items.
We wrap up our analysis by verifying that our results are not driven by specific performance scores: we verify that concurrence values are not skewed by datasets for which performances are saturated or close to random.
To assess this, we compute the correlation between the average performance between two datasets and their concurrence, as plotted in \cref{fig:perfvconcur}.
As can be seen, there is no apparent relation between average performance and concurrence: difficult datasets do not concur less or more than easier ones, and dataset saturation (or the opposite: random performance) appears not to impact the results.
A correlation test confirms this visually observed pattern: the Pearson correlation coefficient between performance and concurrence is near zero ($r=0.026$).

\input{figures/perf_vs_concur}


==> CompositionalitySub_arXiv_2/Results/8_app_NACS.tex <==
\label{app:sec:nacs}
As briefly mentioned in \cref{sec:lex_exposure}, task formulation can be another factor that affects the agreement between datasets.
To understand the effect of task similarity on the conclusion obtained from compositionality benchmarks, we add in the NACS dataset \cite{bastings-etal-2018-jump} for existing experiments, as all three datasets except for SCAN are semantic parsing tasks, while SCAN falls under a navigation task.
NACS is introduced as a dataset that is similar to SCAN but requires mapping actions back to the original commands, and it is thus more complex for models compared to SCAN and will not allow simple models to gain unintended high performance.
We train models on NACS with the same hyperparameter tuning and training strategy as in \cref{sec:Methods}, compute the concurrence between NACS and other datasets, and look at the effect of different splitting strategy between SCAN and NACS. 
The results are discussed below.

\subsection{Overall Performance and Concurrence}
\input{figures/app_NACS/conf_matrix_nacs}
\input{figures/app_NACS/density_by_type}
\input{tables/app_NACS/NACS_high_concur}
The overall performance and concurrence including NACS are shown in \cref{app:tab:all-perf} and \cref{app:fig:nacs-default_conf_matrix}.
The concurrence values between NACS and SCAN is surprisingly low compared to the concurrence values between NACS and other datasets, with the \textit{length} split being the only exception, suggesting that even when the underlying tasks are the same, the datasets may provide very different model rankings.
In terms of the distribution of concurrence values by type of data split pairs (\cref{app:fig:nacs-pairtype-bar}), the conclusion in \cref{sec:comp_def} persists: the source of the dataset matters more than the interpretation of compositonality (splitting strategy).

\subsection{Length Split of NACS}
\input{tables/app_NACS/NACS_length}
Out of the four splits of NACS, the \textit{length} split is the only split that results in a high concurrence with tsplits of SCAN (\cref{app:fig:nacs-default_conf_matrix}).
The \textit{length} split of SCAN and NACS is also the only length splits pair that exceed the boundary set for high concurrence (\cref{app:tab:nacs-length}).
It is likely because that both \textit{length} split of NACS and the splits that it has high concurrence with are extremely difficult split that many models fail on.


==> CompositionalitySub_arXiv_2/abstract.tex <==
\begin{abstract}
NLP models have progressed drastically in recent years, according to numerous datasets proposed to evaluate performance.
Questions remain, however, about how particular dataset design choices may impact the conclusions we draw about model capabilities.
In this work, we investigate this question in the domain of compositional generalization. 
We examine the performance of six modeling approaches across 4 datasets, split according to 8 compositional splitting strategies, ranking models by 18 compositional generalization splits in total.
Our results show that:
i) the datasets, although all designed to evaluate compositional generalization, rank modeling approaches differently;
ii) datasets generated by humans align better with each other than they with synthetic datasets, or than synthetic datasets among themselves;
iii) generally, whether datasets are sampled from the same source is more predictive of the resulting model ranking than whether they maintain the same interpretation of compositionality; and
iv) which lexical items are used in the data can strongly impact conclusions.
Overall, our results demonstrate that much work remains to be done when it comes to assessing whether popular evaluation datasets measure what they intend to measure, and suggests that elucidating more rigorous standards for establishing the validity of evaluation sets could benefit the field.\footnote{Code to reproduce the experiments can be found at \url{https://github.com/facebookresearch/CompositionalityValidity}.}
\end{abstract}


==> CompositionalitySub_arXiv_2/figures/app_NACS/conf_matrix_nacs.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\the\columnwidth]{figures/app_NACS/conf_matrix_default.pdf}
    \caption{Distribution of concurrence values between each dataset and split pairs.}
\label{app:fig:nacs-default_conf_matrix}
\end{figure}

==> CompositionalitySub_arXiv_2/figures/app_NACS/density_by_type.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.85\columnwidth]{figures/app_NACS/density_by_type_app.pdf}
\caption{Distribution of concurrence values among all dataset splits. The color of the bar indicates whether the splits in the pair share the same dataset origin and/or the same splitting strategy.}
\label{app:fig:nacs-pairtype-bar}
\end{figure}

==> CompositionalitySub_arXiv_2/figures/app_NACS/perf_vs_concur.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.85\columnwidth]{figures/app_NACS/perf_vs_concur_app.pdf}
\caption{Values of concurrences with respect to pairwise averaged performance among the splits shown in \cref{app:tab:nacs-all-perf}. The color of dots indicates the type of split pairs. The triangle-shape dots indicates the values of self-concurrence.}
\label{fig:perfvconcur}
\end{figure}

==> CompositionalitySub_arXiv_2/figures/app_overall_concur.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=0.9\textwidth]{figures/fig_files/conf_matrix.pdf}
\caption{Distribution of concurrence values between each dataset and split pairs.}
\label{fig:app:conf_matrix}
\end{figure*}

==> CompositionalitySub_arXiv_2/figures/default_conf_matrix.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\the\columnwidth]{figures/fig_files/default_conf_matrix_avg.pdf}
    \caption{Pairwise concurrence values averaged across models for each dataset--split pair. Values closer to 1.0 (blue) denote a more similar ranking of models according to their performance on the dataset and split. The dataset and split font color indicate whether the data was generated by humans (purple) or synthetically using rules (green).}
\label{fig:default_conf_matrix}
\end{figure}


==> CompositionalitySub_arXiv_2/figures/generalization_studies.tex <==
\begin{figure}
\centering
\includegraphics[width=0.8\columnwidth]{figures/fig_files/pub_count.pdf}
    \caption{Generalization studies published in the ACL anthology (2015-2022), across different \emph{shift sources}.}\label{fig:generalisation_vs_source}
\end{figure}


==> CompositionalitySub_arXiv_2/figures/pair_type_bar_plot.tex <==

\begin{figure}[t]
\centering
\includegraphics[width=0.85\columnwidth]{figures/fig_files/density_by_type.pdf}
\caption{Distribution of concurrence values among all dataset splits. The color of the bar indicates whether the splits in the pair share the same dataset origin and/or the same splitting strategy.}
\label{fig:pairtype-bar}
\end{figure}

==> CompositionalitySub_arXiv_2/figures/perf_v_perf.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{figures/fig_files/pretrained_nonpretrained.pdf}
\caption{Performance of one dataset split versus another. Upper left is an example of high concurrence pair between a synthetic and a natural dataset; upper right is an example of low concurrence within synthetic datasets; lower left is an example of high concurrence within natural datasets; lower right is an example of low concurrence between natural and synthetic datasets.}
\label{fig:perfvperf}
\end{figure}

==> CompositionalitySub_arXiv_2/figures/perf_vs_concur.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.85\columnwidth]{figures/fig_files/perf_alignment.pdf}
\caption{Values of concurrences with respect to pairwise averaged performance among the splits shown in Table~\ref{tab:perfStd}. The color of dots indicates the type of split pairs. The triangle-shape dots indicates the values of self-concurrence.}
\label{fig:perfvconcur}
\end{figure}

==> CompositionalitySub_arXiv_2/figures/std_v_lex.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.85\columnwidth]{figures/fig_files/std_vs_lex.pdf}
\caption{Performance of the original split versus the splits with lexical items replaced. Performance of pretrained models decreases when train on the splits with lexical items that are not previously seen in pretraining.}
\label{fig:std_v_lex}
\end{figure}

==> CompositionalitySub_arXiv_2/tables/app_NACS/NACS_high_concur.tex <==
\begin{table}[t]
\centering
\scriptsize
\begin{tabular}{llllc}
\toprule
\textbf{Dataset A} & \textbf{Dataset B} & \textbf{Split A} & \textbf{Split B} & \textbf{Concur} \\ \midrule
Spider   & Spider   & \textit{Template} & \textit{TMCD}     & 0.88 \\
GeoQuery & Spider   & \textit{Std}      & \textit{Template} & 0.84 \\
GeoQuery & Spider   & \textit{Std}      & \textit{TMCD}     & 0.83 \\
SCAN     & Spider   & \textit{Template} & \textit{Rand}     & 0.76 \\
SCAN     & Spider   & \textit{Template} & \textit{Length}   & 0.76 \\
Spider   & Spider   & \textit{Rand}     & \textit{Length}   & 0.75 \\
GeoQuery & Spider   & \textit{Template} & \textit{Template} & 0.74 \\
SCAN     & NACS     & \textit{MCD2}     & \textit{Length}   & 0.74 \\
GeoQuery & Spider   & \textit{Template} & \textit{TMCD}     & 0.73 \\
SCAN     & NACS     & \textit{Length}   & \textit{Length}   & 0.73 \\
GeoQuery & GeoQuery & \textit{Std}      & \textit{Template} & 0.73 \\
SCAN     & SCAN     & \textit{Length}   & \textit{MCD3}     & 0.72 \\
\bottomrule
\end{tabular}
\caption{High concurrence values ($\geq 0.7$) among all pairs of dataset splits, excluding self-concurrence.}
\label{app:tab:NACS:concurrence}
\end{table}

==> CompositionalitySub_arXiv_2/tables/app_NACS/NACS_length.tex <==

\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{llllll}
\toprule
\textbf{Dataset A} & \textbf{Dataset B} & \textbf{Concur} & \textbf{Dataset A} & \textbf{Dataset B} & \textbf{Concur} \\ 
\cmidrule(lr){1-3} \cmidrule(lr){4-6}

SCAN      & NACS      & \phstar 0.73   & GeoQuery & NACS   & \phstar 0.08  \\
COGS      & GeoQuery  & \phstar 0.54   & Spider   & NACS   & \phstar 0.04  \\
COGS      & Spider    & \phstar 0.26   & SCAN     & Spider & \phstar 0.01  \\
COGS      & NACS      & \phstar 0.24   & COGS     & SCAN   & \phstar 0.01  \\
GeoQuery  & Spider    & \phstar 0.23   & GeoQuery & SCAN   & \phstar -0.09 \\
 \bottomrule
\end{tabular}
\caption{Concurrence between length splits of datasets.}
\label{app:tab:nacs-length}
\end{table}

==> CompositionalitySub_arXiv_2/tables/app_all_concur.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lllllllllc}
\toprule
\textbf{Dataset A} &
  \textbf{Dataset B} &
  \textbf{Split B} &
  \textbf{Split A} &
  \textbf{Concur} &
  \textbf{Dataset A} &
  \textbf{Dataset B} &
  \textbf{Split A} &
  \textbf{Split B} &
  \textbf{Concur} \\ \midrule
Spider   & Spider   & \textit{TMCD}          & \textit{Template}      & 0.88 & COGS     & GeoQuery & \textit{RandStr}    & \textit{TMCD-Rstr}     & 0.54 \\
COGS     & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{Length}        & 0.84 & GeoQuery & SCAN     & \textit{Std-Rstr}   & \textit{TurnLeft}      & 0.54 \\
GeoQuery & Spider   & \textit{Template}      & \textit{Std}           & 0.84 & COGS     & SCAN     & \textit{Std}        & \textit{TurnLeft}      & 0.53 \\
GeoQuery & Spider   & \textit{Template}      & \textit{TMCD-Rstr}     & 0.84 & COGS     & SCAN     & \textit{Randcvcv}   & \textit{TurnLeft}      & 0.52 \\
GeoQuery & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{Std-Rcvcv}     & 0.83 & SCAN     & SCAN     & \textit{MCD1}       & \textit{MCD2}          & 0.52 \\
GeoQuery & Spider   & \textit{TMCD}          & \textit{Std}           & 0.83 & SCAN     & SCAN     & \textit{Length}     & \textit{MCD1}          & 0.52 \\
COGS     & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{Std}           & 0.82 & COGS     & GeoQuery & \textit{Randcvcv}   & \textit{TMCD-Rcvcv}    & 0.51 \\
COGS     & COGS     & \textit{RandStr}       & \textit{Randcvcv}      & 0.82 & GeoQuery & SCAN     & \textit{TMCD-Rcvcv} & \textit{TurnLeft}      & 0.51 \\
GeoQuery & Spider   & \textit{Template}      & \textit{TMCD-Rcvcv}    & 0.81 & SCAN     & SCAN     & \textit{MCD1}       & \textit{MCD3}          & 0.51 \\
COGS     & Spider   & \textit{Template}      & \textit{Length}        & 0.81 & COGS     & SCAN     & \textit{Std}        & \textit{Jump}          & 0.5  \\
GeoQuery & Spider   & \textit{TMCD}          & \textit{TMCD-Rstr}     & 0.81 & GeoQuery & GeoQuery & \textit{Std-Rstr}   & \textit{Template}      & 0.5  \\
GeoQuery & GeoQuery & \textit{TMCD-Rstr}     & \textit{TMCD-Rcvcv}    & 0.81 & GeoQuery & SCAN     & \textit{TMCD-Rcvcv} & \textit{Jump}          & 0.49 \\
COGS     & GeoQuery & \textit{TMCD-Rstr}     & \textit{Length}        & 0.8  & COGS     & GeoQuery & \textit{Randcvcv}   & \textit{Std-Rcvcv}     & 0.49 \\
COGS     & GeoQuery & \textit{Std-Rcvcv}     & \textit{Length}        & 0.8  & GeoQuery & GeoQuery & \textit{Std-Rcvcv}  & \textit{Length}        & 0.48 \\
COGS     & Spider   & \textit{TMCD}          & \textit{Length}        & 0.79 & COGS     & Spider   & \textit{RandStr}    & \textit{Template}      & 0.47 \\
GeoQuery & Spider   & \textit{TMCD}          & \textit{TMCD-Rcvcv}    & 0.79 & COGS     & SCAN     & \textit{RandStr}    & \textit{TurnLeft}      & 0.47 \\
GeoQuery & GeoQuery & \textit{TMCD-Rstr}     & \textit{Std}           & 0.79 & COGS     & COGS     & \textit{Randcvcv}   & \textit{Length}        & 0.47 \\
GeoQuery &
  GeoQuery &
  \textit{TMCD-Rstr} &
  \textit{Std-Rcvcv} &
  0.78 &
  GeoQuery &
  GeoQuery &
  \textit{Std-Rstr} &
  \textit{TMCD} &
  0.46 \\
COGS     & GeoQuery & \textit{Std-Rcvcv}     & \textit{Std}           & 0.78 & COGS     & GeoQuery & \textit{Randcvcv}   & \textit{TMCD-Rstr}     & 0.46 \\
COGS     & COGS     & \textit{Length}        & \textit{Std}           & 0.76 & COGS     & Spider   & \textit{RandStr}    & \textit{TMCD}          & 0.46 \\
SCAN     & Spider   & \textit{Rand}          & \textit{Template}      & 0.76 & GeoQuery & GeoQuery & \textit{Std-Rstr}   & \textit{Length}        & 0.44 \\
SCAN     & Spider   & \textit{Length}        & \textit{Template}      & 0.76 & GeoQuery & SCAN     & \textit{Std-Rcvcv}  & \textit{TurnLeft}      & 0.43 \\
COGS     & GeoQuery & \textit{Std}           & \textit{Length}        & 0.75 & COGS     & SCAN     & \textit{Length}     & \textit{Jump}          & 0.43 \\
GeoQuery & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{Std}           & 0.75 & GeoQuery & SCAN     & \textit{Std-Rcvcv}  & \textit{Jump}          & 0.42 \\
Spider   & Spider   & \textit{Length}        & \textit{Rand}          & 0.75 & COGS     & GeoQuery & \textit{RandStr}    & \textit{Std}           & 0.42 \\
GeoQuery & Spider   & \textit{Template}      & \textit{Template}      & 0.74 & COGS     & SCAN     & \textit{Randcvcv}   & \textit{Jump}          & 0.41 \\
GeoQuery & Spider   & \textit{TMCD}          & \textit{Template}      & 0.73 & GeoQuery & SCAN     & \textit{TMCD-Rstr}  & \textit{TurnLeft}      & 0.41 \\
GeoQuery & Spider   & \textit{Template}      & \textit{Std-Rcvcv}     & 0.73 & COGS     & SCAN     & \textit{Length}     & \textit{TurnLeft}      & 0.41 \\
GeoQuery & GeoQuery & \textit{Template}      & \textit{Std}           & 0.73 & COGS     & SCAN     & \textit{RandStr}    & \textit{Jump}          & 0.41 \\
COGS     & GeoQuery & \textit{Std-Rstr}      & \textit{RandStr}       & 0.73 & COGS     & GeoQuery & \textit{RandStr}    & \textit{Template}      & 0.4  \\
COGS     & GeoQuery & \textit{TMCD-Rstr}     & \textit{Std}           & 0.72 & GeoQuery & SCAN     & \textit{TMCD-Rstr}  & \textit{Jump}          & 0.4  \\
SCAN     & SCAN     & \textit{MCD3}          & \textit{Length}        & 0.72 & SCAN     & Spider   & \textit{Jump}       & \textit{Length}        & 0.4  \\
COGS     & GeoQuery & \textit{Std-Rstr}      & \textit{Std}           & 0.72 & SCAN     & SCAN     & \textit{Jump}       & \textit{TurnLeft}      & 0.4  \\
GeoQuery & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{Std-Rstr}      & 0.71 & COGS     & Spider   & \textit{Randcvcv}   & \textit{Template}      & 0.39 \\
GeoQuery & Spider   & \textit{TMCD}          & \textit{Std-Rcvcv}     & 0.71 & GeoQuery & SCAN     & \textit{Length}     & \textit{Jump}          & 0.39 \\
COGS     & GeoQuery & \textit{Std-Rstr}      & \textit{Randcvcv}      & 0.7  & SCAN     & SCAN     & \textit{Jump}       & \textit{Template}      & 0.39 \\
GeoQuery & GeoQuery & \textit{TMCD-Rstr}     & \textit{Template}      & 0.7  & SCAN     & Spider   & \textit{Jump}       & \textit{Template}      & 0.39 \\
COGS     & Spider   & \textit{Template}      & \textit{Std}           & 0.69 & SCAN     & Spider   & \textit{Jump}       & \textit{Rand}          & 0.38 \\
GeoQuery & GeoQuery & \textit{Std-Rcvcv}     & \textit{Std}           & 0.69 & SCAN     & Spider   & \textit{Jump}       & \textit{TMCD}          & 0.38 \\
SCAN     & SCAN     & \textit{TurnLeftRStr}  & \textit{Simple}        & 0.68 & COGS     & Spider   & \textit{Randcvcv}   & \textit{TMCD}          & 0.38 \\
GeoQuery & GeoQuery & \textit{Std-Rstr}      & \textit{Std-Rcvcv}     & 0.68 & GeoQuery & SCAN     & \textit{Std-Rcvcv}  & \textit{MCD2}          & 0.37 \\
GeoQuery & Spider   & \textit{Template}      & \textit{TMCD}          & 0.68 & Spider   & Spider   & \textit{Rand}       & \textit{TMCD}          & 0.36 \\
GeoQuery & Spider   & \textit{TMCD}          & \textit{TMCD}          & 0.68 & GeoQuery & SCAN     & \textit{TMCD-Rstr}  & \textit{MCD2}          & 0.36 \\
SCAN     & SCAN     & \textit{TurnLeftRcvcv} & \textit{Simple}        & 0.68 & GeoQuery & Spider   & \textit{Length}     & \textit{Rand}          & 0.35 \\
GeoQuery & GeoQuery & \textit{TMCD}          & \textit{Std}           & 0.68 & GeoQuery & SCAN     & \textit{TMCD-Rcvcv} & \textit{MCD2}          & 0.35 \\
COGS     & Spider   & \textit{TMCD}          & \textit{Std}           & 0.67 & Spider   & Spider   & \textit{Rand}       & \textit{Template}      & 0.35 \\
COGS     & GeoQuery & \textit{Std-Rstr}      & \textit{Length}        & 0.67 & GeoQuery & SCAN     & \textit{Length}     & \textit{Template}      & 0.35 \\
COGS     & GeoQuery & \textit{Template}      & \textit{Length}        & 0.67 & GeoQuery & SCAN     & \textit{Std}        & \textit{Jump}          & 0.35 \\
GeoQuery & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{Template}      & 0.66 & GeoQuery & Spider   & \textit{Std}        & \textit{Rand}          & 0.35 \\
GeoQuery & GeoQuery & \textit{TMCD}          & \textit{Template}      & 0.65 & SCAN     & SCAN     & \textit{MCD2}       & \textit{Jump}          & 0.35 \\
GeoQuery & GeoQuery & \textit{TMCD-Rstr}     & \textit{TMCD}          & 0.65 & COGS     & GeoQuery & \textit{RandStr}    & \textit{TMCD}          & 0.34 \\
GeoQuery & GeoQuery & \textit{TMCD-Rstr}     & \textit{Std-Rstr}      & 0.65 & Spider   & Spider   & \textit{Length}     & \textit{TMCD}          & 0.34 \\
SCAN     & SCAN     & \textit{MCD2}          & \textit{Length}        & 0.64 & Spider   & Spider   & \textit{Length}     & \textit{Template}      & 0.34 \\
SCAN     & SCAN     & \textit{TurnLeftRStr}  & \textit{TurnLeftRcvcv} & 0.64 & COGS     & GeoQuery & \textit{Randcvcv}   & \textit{Std}           & 0.34 \\
COGS     & GeoQuery & \textit{Std}           & \textit{Std}           & 0.64 & SCAN     & Spider   & \textit{TurnLeft}   & \textit{Template}      & 0.34 \\
GeoQuery & Spider   & \textit{TMCD}          & \textit{Length}        & 0.63 & COGS     & GeoQuery & \textit{Randcvcv}   & \textit{Length}        & 0.34 \\
GeoQuery & GeoQuery & \textit{TMCD}          & \textit{Length}        & 0.63 & GeoQuery & SCAN     & \textit{TMCD}       & \textit{Jump}          & 0.33 \\
GeoQuery & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{TMCD}          & 0.63 & COGS     & SCAN     & \textit{Std}        & \textit{MCD2}          & 0.33 \\
COGS     & GeoQuery & \textit{TMCD}          & \textit{Length}        & 0.63 & COGS     & GeoQuery & \textit{Randcvcv}   & \textit{Template}      & 0.33 \\
GeoQuery & Spider   & \textit{Template}      & \textit{Length}        & 0.63 & COGS     & GeoQuery & \textit{RandStr}    & \textit{Length}        & 0.32 \\
GeoQuery & GeoQuery & \textit{Length}        & \textit{Std}           & 0.62 & SCAN     & Spider   & \textit{TurnLeft}   & \textit{TMCD}          & 0.32 \\
GeoQuery & GeoQuery & \textit{Template}      & \textit{Length}        & 0.62 & GeoQuery & Spider   & \textit{Std}        & \textit{Length}        & 0.32 \\
GeoQuery & GeoQuery & \textit{Template}      & \textit{Std-Rcvcv}     & 0.62 & SCAN     & Spider   & \textit{Template}   & \textit{TMCD}          & 0.32 \\
GeoQuery & Spider   & \textit{Template}      & \textit{Std-Rstr}      & 0.6  & SCAN     & Spider   & \textit{MCD1}       & \textit{Length}        & 0.31 \\
COGS     & COGS     & \textit{RandStr}       & \textit{Std}           & 0.6  & GeoQuery & Spider   & \textit{Template}   & \textit{Rand}          & 0.31 \\
GeoQuery & GeoQuery & \textit{TMCD}          & \textit{Std-Rcvcv}     & 0.6  & GeoQuery & SCAN     & \textit{Template}   & \textit{Jump}          & 0.31 \\
COGS     & COGS     & \textit{Randcvcv}      & \textit{Std}           & 0.59 & GeoQuery & Spider   & \textit{TMCD}       & \textit{Rand}          & 0.31 \\
GeoQuery & Spider   & \textit{TMCD}          & \textit{Std-Rstr}      & 0.58 & SCAN     & Spider   & \textit{Template}   & \textit{Template}      & 0.31 \\
GeoQuery & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{Length}        & 0.57 & GeoQuery & SCAN     & \textit{Std}        & \textit{Template}      & 0.3  \\
COGS     & GeoQuery & \textit{TMCD-Rcvcv}    & \textit{RandStr}       & 0.57 & GeoQuery & Spider   & \textit{Std-Rstr}   & \textit{Rand}          & 0.3  \\
SCAN     & SCAN     & \textit{MCD3}          & \textit{MCD2}          & 0.57 & COGS     & SCAN     & \textit{Randcvcv}   & \textit{TurnLeftRStr}  & 0.29 \\
COGS     & GeoQuery & \textit{Length}        & \textit{Std}           & 0.56 & SCAN     & SCAN     & \textit{TurnLeft}   & \textit{TurnLeftRcvcv} & 0.29 \\
COGS     & GeoQuery & \textit{TMCD}          & \textit{Std}           & 0.56 & GeoQuery & SCAN     & \textit{Template}   & \textit{Template}      & 0.28 \\
COGS     & GeoQuery & \textit{Template}      & \textit{Std}           & 0.56 & SCAN     & SCAN     & \textit{MCD2}       & \textit{TurnLeft}      & 0.28 \\
COGS     & GeoQuery & \textit{Std-Rcvcv}     & \textit{RandStr}       & 0.56 & COGS     & GeoQuery & \textit{Randcvcv}   & \textit{TMCD}          & 0.28 \\
GeoQuery & GeoQuery & \textit{TMCD-Rstr}     & \textit{Length}        & 0.55 & GeoQuery & SCAN     & \textit{Std}        & \textit{TurnLeft}      & 0.28 \\
COGS     & COGS     & \textit{Length}        & \textit{RandStr}       & 0.55 & COGS     & SCAN     & \textit{Length}     & \textit{MCD2}          & 0.28 \\
GeoQuery & SCAN     & \textit{Jump}          & \textit{Std-Rstr}      & 0.54 & GeoQuery & SCAN     & \textit{Length}     & \textit{TurnLeft}      & 0.28 \\
COGS     & GeoQuery & \textit{Length}        & \textit{Length}        & 0.54 & GeoQuery & SCAN     & \textit{TMCD}       & \textit{Template}      & 0.28 \\
GeoQuery & GeoQuery & \textit{Std-Rstr}      & \textit{Std}           & 0.54 & GeoQuery & Spider   & \textit{Std-Rstr}   & \textit{Length}        & 0.27      \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Concurrence Values.}
\label{tab:app:Concurrence}
\end{table*}

\begin{table*}[ht]
\centering
\scriptsize
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{llllllllll}
\toprule
\textbf{Dataset A} &
  \textbf{Dataset B} &
  \textbf{Split A} &
  \textbf{Split B} &
  \textbf{Concur} &
  \textbf{Dataset A} &
  \textbf{Dataset B} &
  \textbf{Split A} &
  \textbf{Split B} &
  \textbf{Concur} \\ \midrule
COGS     & Spider & \textit{Length}     & \textit{Rand}          & 0.27 & SCAN     & SCAN   & \textit{Jump}          & \textit{TurnLeftRcvcv} & 0.02  \\
GeoQuery & SCAN   & \textit{Std-Rstr}   & \textit{Template}      & 0.27 & COGS     & SCAN   & \textit{Std}           & \textit{MCD1}          & 0.02  \\
GeoQuery & SCAN   & \textit{Std-Rstr}   & \textit{MCD2}          & 0.27 & SCAN     & Spider & \textit{MCD3}          & \textit{Length}        & 0.02  \\
COGS     & SCAN   & \textit{RandStr}    & \textit{TurnLeftRStr}  & 0.27 & COGS     & SCAN   & \textit{Length}        & \textit{MCD3}          & 0.02  \\
COGS     & Spider & \textit{Length}     & \textit{Length}        & 0.26 & GeoQuery & SCAN   & \textit{TMCD-Rcvcv}    & \textit{TurnLeftRStr}  & 0.02  \\
SCAN     & SCAN   & \textit{Length}     & \textit{TurnLeft}      & 0.25 & SCAN     & SCAN   & \textit{MCD1}          & \textit{TurnLeft}      & 0.02  \\
GeoQuery & SCAN   & \textit{TMCD}       & \textit{TurnLeft}      & 0.24 & SCAN     & Spider & \textit{Length}        & \textit{Length}        & 0.01  \\
GeoQuery & Spider & \textit{Template}   & \textit{Length}        & 0.24 & COGS     & SCAN   & \textit{Length}        & \textit{Length}        & 0.01  \\
COGS     & SCAN   & \textit{Randcvcv}   & \textit{Simple}        & 0.24 & SCAN     & SCAN   & \textit{Simple}        & \textit{MCD3}          & 0.01  \\
SCAN     & SCAN   & \textit{MCD1}       & \textit{Template}      & 0.24 & SCAN     & Spider & \textit{Simple}        & \textit{Length}        & 0.01  \\
SCAN     & SCAN   & \textit{TurnLeft}   & \textit{TurnLeftRStr}  & 0.23 & SCAN     & SCAN   & \textit{TurnLeft}      & \textit{Template}      & 0.01  \\
GeoQuery & SCAN   & \textit{Template}   & \textit{TurnLeft}      & 0.23 & SCAN     & SCAN   & \textit{Simple}        & \textit{Jump}          & 0.0   \\
GeoQuery & Spider & \textit{TMCD}       & \textit{Length}        & 0.23 & SCAN     & Spider & \textit{TurnLeft}      & \textit{Rand}          & -0.0  \\
GeoQuery & Spider & \textit{Length}     & \textit{Length}        & 0.23 & COGS     & SCAN   & \textit{Randcvcv}      & \textit{Length}        & -0.01 \\
GeoQuery &
  Spider &
  \textit{TMCD-Rcvcv} &
  \textit{Length} &
  0.22 &
  GeoQuery &
  SCAN &
  \textit{Std-Rcvcv} &
  \textit{TurnLeftRStr} &
  -0.01 \\
SCAN     & SCAN   & \textit{Length}     & \textit{Jump}          & 0.22 & GeoQuery & SCAN   & \textit{Std}           & \textit{MCD1}          & -0.02 \\
COGS     & SCAN   & \textit{Length}     & \textit{Template}      & 0.22 & SCAN     & Spider & \textit{MCD1}          & \textit{Template}      & -0.02 \\
GeoQuery & Spider & \textit{TMCD-Rstr}  & \textit{Length}        & 0.22 & GeoQuery & SCAN   & \textit{TMCD}          & \textit{MCD1}          & -0.02 \\
GeoQuery & Spider & \textit{TMCD-Rcvcv} & \textit{Rand}          & 0.22 & COGS     & SCAN   & \textit{Std}           & \textit{TurnLeftRcvcv} & -0.02 \\
GeoQuery & Spider & \textit{TMCD-Rstr}  & \textit{Rand}          & 0.21 & COGS     & SCAN   & \textit{RandStr}       & \textit{MCD1}          & -0.02 \\
COGS     & SCAN   & \textit{RandStr}    & \textit{Simple}        & 0.21 & COGS     & SCAN   & \textit{Std}           & \textit{Simple}        & -0.03 \\
SCAN     & SCAN   & \textit{MCD1}       & \textit{Jump}          & 0.21 & COGS     & SCAN   & \textit{Length}        & \textit{TurnLeftRStr}  & -0.03 \\
SCAN     & Spider & \textit{MCD2}       & \textit{Template}      & 0.2  & SCAN     & Spider & \textit{TurnLeftRStr}  & \textit{Length}        & -0.03 \\
GeoQuery & SCAN   & \textit{Std}        & \textit{MCD2}          & 0.2  & GeoQuery & SCAN   & \textit{TMCD}          & \textit{MCD3}          & -0.03 \\
COGS     & SCAN   & \textit{RandStr}    & \textit{TurnLeftRcvcv} & 0.2  & SCAN     & Spider & \textit{MCD1}          & \textit{TMCD}          & -0.03 \\
SCAN     & SCAN   & \textit{Simple}     & \textit{TurnLeft}      & 0.2  & GeoQuery & SCAN   & \textit{TMCD-Rcvcv}    & \textit{Simple}        & -0.04 \\
SCAN     & Spider & \textit{MCD1}       & \textit{Rand}          & 0.19 & GeoQuery & SCAN   & \textit{Template}      & \textit{MCD3}          & -0.04 \\
SCAN     & Spider & \textit{MCD2}       & \textit{TMCD}          & 0.19 & GeoQuery & SCAN   & \textit{TMCD}          & \textit{Length}        & -0.04 \\
GeoQuery & Spider & \textit{Std-Rcvcv}  & \textit{Rand}          & 0.18 & COGS     & SCAN   & \textit{RandStr}       & \textit{Length}        & -0.04 \\
GeoQuery & SCAN   & \textit{TMCD-Rcvcv} & \textit{Template}      & 0.18 & SCAN     & SCAN   & \textit{MCD3}          & \textit{Template}      & -0.05 \\
COGS     & Spider & \textit{RandStr}    & \textit{Rand}          & 0.18 & GeoQuery & SCAN   & \textit{TMCD-Rcvcv}    & \textit{TurnLeftRcvcv} & -0.05 \\
GeoQuery & SCAN   & \textit{TMCD-Rstr}  & \textit{Template}      & 0.18 & GeoQuery & SCAN   & \textit{Std-Rcvcv}     & \textit{Simple}        & -0.06 \\
SCAN     & SCAN   & \textit{MCD3}       & \textit{Jump}          & 0.18 & GeoQuery & SCAN   & \textit{Std}           & \textit{MCD3}          & -0.06 \\
GeoQuery & SCAN   & \textit{TMCD}       & \textit{MCD2}          & 0.18 & SCAN     & Spider & \textit{MCD3}          & \textit{Template}      & -0.06 \\
SCAN     & Spider & \textit{MCD2}       & \textit{Length}        & 0.18 & COGS     & SCAN   & \textit{Randcvcv}      & \textit{MCD3}          & -0.06 \\
GeoQuery & SCAN   & \textit{Template}   & \textit{MCD2}          & 0.17 & GeoQuery & SCAN   & \textit{TMCD-Rstr}     & \textit{TurnLeftRStr}  & -0.06 \\
SCAN     & SCAN   & \textit{MCD3}       & \textit{TurnLeft}      & 0.17 & GeoQuery & SCAN   & \textit{Template}      & \textit{Length}        & -0.06 \\
COGS     & Spider & \textit{Std}        & \textit{Rand}          & 0.17 & COGS     & SCAN   & \textit{Length}        & \textit{Simple}        & -0.07 \\
GeoQuery & Spider & \textit{Std-Rcvcv}  & \textit{Length}        & 0.17 & SCAN     & SCAN   & \textit{Length}        & \textit{Template}      & -0.07 \\
COGS     & Spider & \textit{RandStr}    & \textit{Length}        & 0.15 & SCAN     & Spider & \textit{MCD3}          & \textit{TMCD}          & -0.07 \\
GeoQuery & SCAN   & \textit{Std-Rstr}   & \textit{TurnLeftRStr}  & 0.15 & GeoQuery & SCAN   & \textit{Std}           & \textit{Length}        & -0.07 \\
COGS     & SCAN   & \textit{RandStr}    & \textit{MCD2}          & 0.15 & SCAN     & Spider & \textit{Length}        & \textit{Template}      & -0.07 \\
SCAN     & SCAN   & \textit{Length}     & \textit{TurnLeftRcvcv} & 0.14 & COGS     & SCAN   & \textit{RandStr}       & \textit{MCD3}          & -0.07 \\
COGS     & SCAN   & \textit{Std}        & \textit{Length}        & 0.14 & GeoQuery & SCAN   & \textit{Length}        & \textit{MCD3}          & -0.08 \\
COGS     & SCAN   & \textit{RandStr}    & \textit{Template}      & 0.14 & SCAN     & Spider & \textit{MCD3}          & \textit{Rand}          & -0.08 \\
COGS     & Spider & \textit{Std}        & \textit{Length}        & 0.14 & COGS     & SCAN   & \textit{Randcvcv}      & \textit{MCD1}          & -0.09 \\
GeoQuery & SCAN   & \textit{TMCD-Rcvcv} & \textit{Length}        & 0.14 & GeoQuery & SCAN   & \textit{Length}        & \textit{Length}        & -0.09 \\
COGS     & SCAN   & \textit{Std}        & \textit{Template}      & 0.13 & SCAN     & Spider & \textit{Length}        & \textit{TMCD}          & -0.09 \\
GeoQuery & SCAN   & \textit{Std-Rcvcv}  & \textit{Template}      & 0.13 & SCAN     & SCAN   & \textit{MCD1}          & \textit{TurnLeftRStr}  & -0.09 \\
COGS     & SCAN   & \textit{Randcvcv}   & \textit{MCD2}          & 0.13 & SCAN     & Spider & \textit{Length}        & \textit{Rand}          & -0.1  \\
GeoQuery & SCAN   & \textit{TMCD-Rstr}  & \textit{Length}        & 0.12 & SCAN     & Spider & \textit{TurnLeftRStr}  & \textit{Template}      & -0.11 \\
SCAN &
  SCAN &
  \textit{Length} &
  \textit{TurnLeftRStr} &
  0.12 &
  GeoQuery &
  SCAN &
  \textit{Std-Rcvcv} &
  \textit{TurnLeftRcvcv} &
  -0.11 \\
COGS     & SCAN   & \textit{Std}        & \textit{MCD3}          & 0.12 & SCAN     & SCAN   & \textit{Simple}        & \textit{MCD1}          & -0.11 \\
GeoQuery & SCAN   & \textit{Std-Rcvcv}  & \textit{Length}        & 0.12 & SCAN     & Spider & \textit{TurnLeftRStr}  & \textit{TMCD}          & -0.12 \\
GeoQuery & SCAN   & \textit{TMCD-Rstr}  & \textit{MCD1}          & 0.11 & SCAN     & Spider & \textit{Simple}        & \textit{Rand}          & -0.12 \\
COGS     & Spider & \textit{Randcvcv}   & \textit{Rand}          & 0.11 & COGS     & SCAN   & \textit{Length}        & \textit{TurnLeftRcvcv} & -0.12 \\
GeoQuery & SCAN   & \textit{TMCD-Rcvcv} & \textit{MCD3}          & 0.11 & GeoQuery & SCAN   & \textit{TMCD-Rstr}     & \textit{Simple}        & -0.13 \\
GeoQuery & SCAN   & \textit{Std-Rcvcv}  & \textit{MCD3}          & 0.11 & SCAN     & SCAN   & \textit{MCD1}          & \textit{TurnLeftRcvcv} & -0.13 \\
GeoQuery & SCAN   & \textit{TMCD-Rstr}  & \textit{MCD3}          & 0.11 & SCAN     & SCAN   & \textit{Simple}        & \textit{Template}      & -0.13 \\
GeoQuery & SCAN   & \textit{Std-Rcvcv}  & \textit{MCD1}          & 0.1  & SCAN     & Spider & \textit{TurnLeftRStr}  & \textit{Rand}          & -0.14 \\
GeoQuery & SCAN   & \textit{Std-Rstr}   & \textit{MCD1}          & 0.1  & GeoQuery & SCAN   & \textit{TMCD-Rstr}     & \textit{TurnLeftRcvcv} & -0.14 \\
GeoQuery & SCAN   & \textit{Std-Rstr}   & \textit{Simple}        & 0.09 & SCAN     & Spider & \textit{Simple}        & \textit{Template}      & -0.15 \\
GeoQuery & SCAN   & \textit{Std-Rstr}   & \textit{Length}        & 0.09 & SCAN     & SCAN   & \textit{TurnLeftRStr}  & \textit{Template}      & -0.15 \\
GeoQuery &
  SCAN &
  \textit{Std-Rstr} &
  \textit{TurnLeftRcvcv} &
  0.08 &
  SCAN &
  Spider &
  \textit{TurnLeftRcvcv} &
  \textit{Length} &
  -0.15 \\ 
COGS     & SCAN   & \textit{Randcvcv}   & \textit{Template}      & 0.08 & GeoQuery & SCAN   & \textit{Std}           & \textit{TurnLeftRStr}  & -0.15 \\
SCAN     & SCAN   & \textit{MCD2}       & \textit{TurnLeftRStr}  & 0.08 & SCAN     & Spider & \textit{Simple}        & \textit{TMCD}          & -0.16 \\
SCAN     & SCAN   & \textit{Simple}     & \textit{Length}        & 0.08 & GeoQuery & SCAN   & \textit{Length}        & \textit{MCD1}          & -0.18 \\
COGS     & Spider & \textit{Randcvcv}   & \textit{Length}        & 0.07 & GeoQuery & SCAN   & \textit{Std}           & \textit{Simple}        & -0.19 \\
SCAN     & SCAN   & \textit{MCD2}       & \textit{TurnLeftRcvcv} & 0.07 & SCAN     & Spider & \textit{TurnLeftRcvcv} & \textit{Template}      & -0.2  \\
SCAN     & SCAN   & \textit{MCD3}       & \textit{TurnLeftRcvcv} & 0.06 & GeoQuery & SCAN   & \textit{TMCD}          & \textit{TurnLeftRStr}  & -0.21 \\
GeoQuery & SCAN   & \textit{Length}     & \textit{MCD2}          & 0.06 & GeoQuery & SCAN   & \textit{Template}      & \textit{TurnLeftRStr}  & -0.21 \\
SCAN     & SCAN   & \textit{Simple}     & \textit{MCD2}          & 0.05 & SCAN     & Spider & \textit{TurnLeftRcvcv} & \textit{TMCD}          & -0.22 \\
GeoQuery & SCAN   & \textit{TMCD-Rcvcv} & \textit{MCD1}          & 0.05 & GeoQuery & SCAN   & \textit{Length}        & \textit{TurnLeftRStr}  & -0.24 \\
SCAN     & SCAN   & \textit{MCD3}       & \textit{TurnLeftRStr}  & 0.05 & GeoQuery & SCAN   & \textit{Std}           & \textit{TurnLeftRcvcv} & -0.25 \\
SCAN     & SCAN   & \textit{Jump}       & \textit{TurnLeftRStr}  & 0.05 & SCAN     & SCAN   & \textit{TurnLeftRcvcv} & \textit{Template}      & -0.26 \\
SCAN     & Spider & \textit{MCD2}       & \textit{Rand}          & 0.05 & GeoQuery & SCAN   & \textit{TMCD}          & \textit{Simple}        & -0.26 \\
SCAN     & Spider & \textit{TurnLeft}   & \textit{Length}        & 0.05 & GeoQuery & SCAN   & \textit{Template}      & \textit{Simple}        & -0.27 \\
GeoQuery & SCAN   & \textit{Std-Rstr}   & \textit{MCD3}          & 0.05 & SCAN     & Spider & \textit{TurnLeftRcvcv} & \textit{Rand}          & -0.27 \\
SCAN     & SCAN   & \textit{MCD2}       & \textit{Template}      & 0.04 & GeoQuery & SCAN   & \textit{Length}        & \textit{TurnLeftRcvcv} & -0.28 \\
COGS     & SCAN   & \textit{Length}     & \textit{MCD1}          & 0.04 & GeoQuery & SCAN   & \textit{TMCD}          & \textit{TurnLeftRcvcv} & -0.29 \\
COGS     & SCAN   & \textit{Std}        & \textit{TurnLeftRStr}  & 0.03 & GeoQuery & SCAN   & \textit{Template}      & \textit{TurnLeftRcvcv} & -0.3  \\
GeoQuery & SCAN   & \textit{Template}   & \textit{MCD1}          & 0.02 & GeoQuery & SCAN   & \textit{Length}        & \textit{Simple}        & -0.3     
\\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Concurrence Values (Cont).}
\label{tab:app:allconur}
\end{table*}

==> CompositionalitySub_arXiv_2/tables/app_all_perf.tex <==

\begin{table*}[ht]
\centering
\scriptsize
\begin{adjustbox}{max width=0.9\textwidth}
\begin{tabular}{clrlrlrlrlrlrlr}
\toprule
\textbf{Dataset} &
  \textbf{Split} &
  \multicolumn{2}{c}{\textbf{LSTM Uni}} &
  \multicolumn{2}{c}{\textbf{LSTM Bi}} &
  \multicolumn{2}{c}{\textbf{Transformer}} &
  \multicolumn{2}{c}{\textbf{T5}} &
  \multicolumn{2}{c}{\textbf{BART}} &
  \multicolumn{2}{c}{\textbf{BTG}} &
  \multicolumn{1}{c}{\textbf{Avg}} \\ \midrule
\multirow{7}{*}{COGS}   & \textit{Std-Test}      & 99.3  & ±.0  & 99.1  & ±.01 & 99.5  & ±.0  & 99.7 & ±.0  & 99.7  & ±.0  & 68.8 & ±.01 & 94.3 \\
                        & \textit{Rcvcv-Test}    & 99.4  & ±.0  & 99.1  & ±.0  & 99.5  & ±.0  & 99.7 & ±.0  & 99.7  & ±.0  & 68.1 & ±.0  & 94.2 \\
                        & \textit{Rstr-Test}     & 99.4  & ±.0  & 99.0  & ±.01 & 99.6  & ±.0  & 99.8 & ±.0  & 99.7  & ±.0  & 68.4 & ±.0  & 94.3 \\
                        & \textit{Std-Gen}       & 21.3  & ±.05 & 14.8  & ±.08 & 56.1  & ±.06 & 82.9 & ±.0  & 78.6  & ±.0  & 2.8  & ±.01 & 42.8 \\
                        & \textit{Rcvcv-Gen}     & 22.6  & ±.04 & 10.1  & ±.02 & 57.6  & ±.02 & 50.0 & ±.02 & 44.5  & ±.07 & 0.0  & ±.0  & 30.8 \\
                        & \textit{Rstr-Gen}      & 22.3  & ±.07 & 14.7  & ±.03 & 56.6  & ±.03 & 48.0 & ±.01 & 33.5  & ±.03 & 0.0  & ±.0  & 29.2 \\
                        & \textit{Length}        & 20.7  & ±.01 & 24.9  & ±.01 & 28.7  & ±.02 & 37.9 & ±.0  & 34.1  & ±.01 & 20.5 & ±.0  & 27.8 \\ \midrule
\multirow{10}{*}{SCAN}  & \textit{Simple}        & 99.9  & ±.0  & 99.9  & ±.0  & 100.0 & ±.0  & 94.9 & ±.01 & 99.1  & ±.01 & 12.3 & ±.01 & 84.4 \\
                        & \textit{Jump}          & 0.4   & ±.01 & 0.0   & ±.0  & 0.1   & ±.0  & 95.0 & ±.01 & 0.4   & ±.01 & 0.0  & ±.0  & 16.0 \\
                        & \textit{Template}      & 0.2   & ±.0  & 0.3   & ±.01 & 1.1   & ±.0  & 34.3 & ±.03 & 0.0   & ±.0  & 0.9  & ±.01 & 6.1  \\
                        & \textit{MCD1}          & 5.9   & ±.06 & 12.2  & ±.07 & 1.1   & ±.0  & 24.6 & ±.01 & 0.4   & ±.01 & 1.8  & ±.01 & 7.7  \\
                        & \textit{MCD2}          & 6.7   & ±.03 & 5.8   & ±.03 & 1.2   & ±.0  & 34.1 & ±.01 & 1.6   & ±.0  & 0.5  & ±.0  & 8.3  \\
                        & \textit{MCD3}          & 8.7   & ±.04 & 7.8   & ±.02 & 0.7   & ±.0  & 11.1 & ±.01 & 1.2   & ±.01 & 0.8  & ±.01 & 5.0  \\
                        & \textit{Length}        & 15.3  & ±.04 & 11.8  & ±.01 & 0.0   & ±.0  & 14.1 & ±.01 & 0.7   & ±.01 & 0.0  & ±.0  & 7.0  \\
                        & \textit{TurnLeft}      & 61.1  & ±.13 & 34.1  & ±.06 & 64.8  & ±.11 & 70.3 & ±.12 & 63.1  & ±.19 & 8.9  & ±.01 & 50.4 \\
                        & \textit{TurnLeftRcvcv} & 69.4  & ±.14 & 42.8  & ±.14 & 60.4  & ±.12 & 20.0 & ±.03 & 37.7  & ±.15 & 3.5  & ±.01 & 39.0 \\
                        & \textit{TurnLeftRStr}  & 59.0  & ±.18 & 43.5  & ±.1  & 61.9  & ±.1  & 17.7 & ±.02 & 23.9  & ±.17 & 2.4  & ±.0  & 34.7 \\ \midrule
\multirow{4}{*}{NACS}   & \textit{Simple}        & 100.0 & ±.0  & 100.0 & ±.0  & 100.0 & ±.0  & 94.6 & ±.0  & 100.0 & ±.0  & 6.1  & ±.01 & 83.5 \\
                        & \textit{Jump}          & 0.1   & ±.0  & 0.2   & ±.0  & 0.2   & ±.0  & 95.8 & ±.01 & 67.6  & ±.04 & 0.0  & ±.0  & 27.3 \\
                        & \textit{TurnLeft}      & 63.3  & ±.12 & 62.0  & ±.13 & 54.4  & ±.11 & 64.9 & ±.04 & 82.4  & ±.13 & 9.2  & ±.01 & 56.0 \\
                        & \textit{Length}        & 12.7  & ±.02 & 13.2  & ±.01 & 0.0   & ±.0  & 14.3 & ±.0  & 9.3   & ±.02 & 0.0  & ±.0  & 8.2  \\ \midrule
\multirow{4}{*}{Spider} & \textit{Rand}          & 33.4  & ±.02 & 36.9  & ±.01 & 42.5  & ±.01 & 68.0 & ±.0  & 32.7  & ±.01 & 40.1 & ±.01 & 42.3 \\
                        & \textit{Template}      & 1.0   & ±.0  & 2.2   & ±.01 & 4.6   & ±.0  & 39.6 & ±.01 & 21.6  & ±.01 & 1.9  & ±.0  & 11.8 \\
                        & \textit{TMCD}          & 4.6   & ±.01 & 6.0   & ±.01 & 7.5   & ±.01 & 47.2 & ±.01 & 31.2  & ±.03 & 5.5  & ±.0  & 17.0 \\
                        & \textit{Length}        & 12.7  & ±.01 & 14.0  & ±.01 & 17.5  & ±.01 & 35.4 & ±.01 & 7.4   & ±.0  & 14.0 & ±.01 & 16.8 \\ \midrule
\multirow{8}{*}{GeoQuery} &
  \textit{Std} &
  74.0 &
  ±.06 &
  78.9 &
  ±.04 &
  82.3 &
  ±.02 &
  92.5 &
  ±.01 &
  89.2 &
  ±.01 &
  79.0 &
  ±.01 &
  82.6 \\
                        & \textit{Std-Rcvcv}     & 76.7  & ±.03 & 78.9  & ±.02 & 80.5  & ±.01 & 89.4 & ±.0  & 84.2  & ±.0  & 69.0 & ±.03 & 79.8 \\
                        & \textit{Std-Rstr}      & 77.1  & ±.01 & 78.6  & ±.02 & 82.7  & ±.01 & 88.8 & ±.01 & 79.9  & ±.0  & 65.8 & ±.01 & 78.8 \\
                        & \textit{Template}      & 46.5  & ±.06 & 55.9  & ±.07 & 56.7  & ±.04 & 91.0 & ±.0  & 77.1  & ±.06 & 53.5 & ±.06 & 63.5 \\
                        & \textit{Length}        & 18.5  & ±.03 & 16.2  & ±.02 & 22.0  & ±.01 & 41.1 & ±.01 & 36.1  & ±.01 & 20.7 & ±.02 & 25.8 \\
                        & \textit{TMCD}          & 35.8  & ±.02 & 37.1  & ±.02 & 37.9  & ±.01 & 54.1 & ±.0  & 48.2  & ±.0  & 36.9 & ±.0  & 41.7 \\
                        & \textit{TMCD-Rcvcv}    & 35.9  & ±.01 & 36.7  & ±.01 & 37.5  & ±.0  & 43.3 & ±.0  & 40.8  & ±.01 & 34.3 & ±.0  & 38.1 \\
                        & \textit{TMCD-Rstr}     & 35.5  & ±.01 & 37.7  & ±.01 & 37.6  & ±.0  & 43.1 & ±.0  & 41.4  & ±.0  & 35.3 & ±.01 & 38.4     \\
                        \bottomrule
\end{tabular}
\end{adjustbox}
    \caption{Model exact-match accuracy on datasets averaged across random seeds, with standard deviation.}%
\label{app:tab:all-perf}
\end{table*}

==> CompositionalitySub_arXiv_2/tables/app_dataset_examples.tex <==
\begin{table*}[ht]
\scriptsize
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{p{4em}p{5em}p{0.8\textwidth}}
\toprule
\multirow{2}{*}{\textbf{COGS}} & \textbf{Input:} & Mila liked that the cake was offered to Emma . \\
& \textbf{Output:} & \texttt{* cake ( x \_ 4 ) ; like . agent ( x \_ 1 , Mila ) AND like . ccomp ( x \_ 1 , x \_ 6 ) AND offer . theme ( x \_ 6 , x \_ 4 ) AND offer . recipient ( x \_ 6 , Emma )}
\\ \midrule
\multirow{2}{*}{\textbf{SCAN}}  &  \textbf{Input:} & turn left after jump twice \\
 & \textbf{Output:} & \texttt{I\_JUMP I\_JUMP I\_TURN\_LEFT}
\\ \midrule
\multirow{2}{*}{\textbf{NACS}}  &  \textbf{Input:} & run thrice after jump around left \\
 & \textbf{Output:} & \texttt{I\_TURN\_LEFT I\_JUMP I\_TURN\_LEFT I\_JUMP I\_TURN\_LEFT I\_JUMP I\_TURN\_LEFT I\_JUMP I\_RUN I\_RUN I\_RUN}
\\ \midrule
\multirow{2}{*}{\textbf{GeoQuery}}  &  \textbf{Input:} & how much population does m0 have \\
&  \textbf{Output:} & \texttt{answer ( intersection ( river , loc\_2 ( m0 ) ) )} \\ \midrule
\multirow{2}{*}{\textbf{Spider}}  &  \textbf{Input:} & flight\_1: what is the average distance and price for all flights from la?  \\
&  \textbf{Output:} & \texttt{select avg(distance) , avg(price) from flight where origin = "los angeles"} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Examples of instances in each dataset used in our experiments.}\label{tab:examples}

\end{table*}

==> CompositionalitySub_arXiv_2/tables/app_genbench_eval_card.tex <==
\newcommand{\tabularwidth}{\textwidth}

\newcommand{\expone}{$\square$}
\newcommand{\exptwo}{$\bigtriangleup$}
\newcommand{\expthree}{$\bigcirc$}
\newcommand{\expfour}{$\odot$}
        
\renewcommand{\arraystretch}{1.1}         
\setlength{\tabcolsep}{0mm}        
\begin{table*}[ht]
\begin{adjustbox}{max width=\textwidth}

\begin{tabular}{|p{\tabularwidth}<{\centering}|}         
\hline
               
\rowcolor{gray!60}               
\textbf{Motivation} \\               
\footnotesize
\begin{tabular}{p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering}}                        
\textit{Practical} & \textit{Cognitive} & \textit{Intrinsic} & \textit{Fairness}\\
& \expone\hspace{0.8mm}\exptwo\hspace{0.8mm}\expthree\hspace{0.8mm}\expfour\hspace{0.8mm}		%
& 		%
& 		%

\vspace{2mm} \\
\end{tabular}\\
               
\rowcolor{gray!60}               
\textbf{Generalisation type} \\               
\footnotesize
\begin{tabular}{m{0.21\tabularwidth}<{\centering} m{0.2\tabularwidth}<{\centering} m{0.13\tabularwidth}<{\centering} m{0.13\tabularwidth}<{\centering} m{0.13\tabularwidth}<{\centering} m{0.2\tabularwidth}<{\centering}}                   
\textit{Compositional} & \textit{Structural} & \textit{Cross Task} & \textit{Cross Language} & \textit{Cross Domain} & \textit{Robustness}\\
\expone\hspace{0.8mm}\exptwo\hspace{0.8mm}\expthree\hspace{0.8mm}\expfour\hspace{0.8mm}		%
& 		%
& 		%
& 		%
& 		%
& 		%

\vspace{2mm} \\
\end{tabular}\\
             
\rowcolor{gray!60}             
\textbf{Shift type} \\             
\footnotesize
\begin{tabular}{p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering}}                        
\textit{Covariate} & \textit{Label} & \textit{Full} & \textit{Assumed}\\  
\expone\hspace{0.8mm}\exptwo\hspace{0.8mm}\expthree\hspace{0.8mm}\expfour\hspace{0.8mm}		%
& 		%
& 		%
& 		%

\vspace{2mm} \\
\end{tabular}\\
             
\rowcolor{gray!60}             
\textbf{Shift source} \\             
\footnotesize
\begin{tabular}{p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering}}                          
\textit{Naturally occuring} & \textit{Partitioned natural} & \textit{Generated shift} & \textit{Fully generated}\\
& \expone\hspace{0.8mm}\exptwo\hspace{0.8mm}		%
& 		%
& \hspace{11mm}\expthree\hspace{0.8mm}\expfour\hspace{0.8mm}		%

\vspace{2mm} \\
\end{tabular}\\
             
\rowcolor{gray!60}             
\textbf{Shift locus}\\             
\footnotesize
\begin{tabular}{p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering} p{0.25\tabularwidth}<{\centering}}                         
\textit{Train--test} & \textit{Finetune train--test} & \textit{Pretrain--train} & \textit{Pretrain--test}\\
\expone\hspace{0.8mm}\expthree\hspace{0.8mm}		%
& \exptwo\hspace{0.8mm}\expfour\hspace{0.8mm}		%
& 		%
& 		%

\vspace{2mm} \\
\end{tabular} \\
\hline

\end{tabular}
\end{adjustbox}
\caption{A GenBench evaluation card \citep{Hupkes2023} that summarizes our experiments. \expone = Experiments of LSTM and Transformer on GeoQuery and Spider; \exptwo = Experiments of T5 and BART on GeoQuery and Spider; \expthree = Experiments of LSTM and Transformer on COGS and SCAN; \expfour = Experiments of T5 and BART on COGS and SCAN.}
\label{tab:eval_card}
\end{table*}

==> CompositionalitySub_arXiv_2/tables/app_license.tex <==
\begin{table*}[ht]
\scriptsize
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lll}
\toprule
\textbf{Artifact} & \textbf{License} & \textbf{Intended Usage}                                       \\
\midrule
COGS              & MIT              & A dataset focuses on compositional generalization \\
SCAN & BSD & A dataset focuses on compositional generalization. \\
GeoQuery & ODC-BY 1.0 license & A database query datasets for U.S. geography. \\
Spider & CC BY-SA 4.0 & A cross-domain semantic parsing and text-to-SQL dataset. \\ 
NACS & CC-NC & A dataset focuses on compositional generalization. \\ \midrule
Neural-BTG              & MIT       & \begin{tabular}[c]{@{}l@{}}A neural transducer for sequence-to-sequence tasks.\end{tabular}   \\
\begin{tabular}[c]{@{}l@{}}LSTM, Transformer \\ (OpenNMT-py \cite{klein-etal-2017-opennmt}) \end{tabular}           & MIT       &  Models for  sequence-to-sequence tasks. \\
T5              & Apache-2.0       & \begin{tabular}[c]{@{}l@{}}A pre-trained model for sequence-to-sequence tasks.\end{tabular}   \\
BART              & Apache-2.0       & \begin{tabular}[c]{@{}l@{}}A pre-trained model for sequence-to-sequence tasks.\end{tabular}   \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{License and intended usage for the artifacts we used.}
\label{app:tab:licenses}
\end{table*}

==> CompositionalitySub_arXiv_2/tables/app_spider_table.tex <==
\begin{table}[H]
\centering
\scriptsize
\begin{tabular}{p{0.1\columnwidth}p{0.09\columnwidth}p{0.09\columnwidth}p{0.09\columnwidth}p{0.09\columnwidth}p{0.09\columnwidth}p{0.09\columnwidth}}
\toprule
\textbf{Split} &
   \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}LSTM\\  Uni\end{tabular}}} &
  \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}LSTM\\  Bi\end{tabular}}} &
  \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Trans-\\ former\end{tabular}}} &
  \multicolumn{1}{l}{\textbf{T5}} &
  \multicolumn{1}{l}{\textbf{BART}} &
  \multicolumn{1}{l}{\textbf{BTG}} \\ \midrule
\textit{Rand}     & 0.0 & 0.0 & 0.0 & 77.8 & 34.8 & 46.2 \\
\textit{Template} & 1.4 & 2.7 & 3.2 & 52.5 & 25.5 & 3.5  \\
\textit{TMCD}     & 0.1 & 0.1 & 0.1 & 57.6 & 37.9 & 6.9  \\
\textit{Length}   & 0.9 & 0.6 & 0.3 & 44.4 & 9.0  & 16.5 \\ \bottomrule
\end{tabular}
\caption{Model exact-match accuracy with Spider EM. A large amount of output of LSTM and Transformer are deemed as invalid SQL due to special tokens.}
\label{tab:app:spider-perf}
\end{table}

==> CompositionalitySub_arXiv_2/tables/app_split_intro.tex <==
\begin{table*}[ht]
\small
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lll}
\toprule
\textbf{Split} & \textbf{Dataset} & \textbf{Description}                                       \\
\midrule
\textit{random/standard/simple}              & COGS, SCAN, GeoQuery, Spider              & Split the dataset randomly. \\
\textit{length} & COGS, SCAN, GeoQuery, Spider & Split the dataset according to the input length. \\
\textit{template} & SCAN, GeoQuery, Spider & Split the dataset based on a given string template. \\
\textit{TurnLeft} & SCAN & Compositional commands of \texttt{TurnLeft} are isolated in training set. \\
\textit{Jump} & SCAN & Compositional commands of \texttt{Jump} are isolated in training set. \\
\textit{MCD} & SCAN & Split according to maximum compound divergence. \\
\textit{TMCD} & GeoQuery, Spider & Natural counterpart of MCD, split the data based on target MCD. \\
\textit{Gen} & COGS & \begin{tabular}[c]{@{}l@{}}Not a splitting strategy, but a collection of specially generated samples \\ designed to test 21 cases of generalization in COGS. \end{tabular}
 \\

\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Summary of each split and their designated dataset we use.}
\label{app:tab:splitintro}
\end{table*}

==> CompositionalitySub_arXiv_2/tables/concurrence_table.tex <==
\begin{table}[t]
\centering
\scriptsize
\begin{tabular}{llllc}
\toprule
\textbf{Dataset A} & \textbf{Dataset B} & \textbf{Split A} & \textbf{Split B} & \textbf{Concur} \\ \midrule
Spider   & Spider   & \textit{Template} & \textit{TMCD}     & 0.88 \\
GeoQuery & Spider   & \textit{Std}      & \textit{Template} & 0.84 \\
GeoQuery & Spider   & \textit{Std}      & \textit{TMCD}     & 0.83 \\
SCAN     & Spider   & \textit{Template} & \textit{Rand}     & 0.76 \\
SCAN     & Spider   & \textit{Template} & \textit{Length}   & 0.76 \\
Spider   & Spider   & \textit{Rand}     & \textit{Length}   & 0.75 \\
GeoQuery & Spider   & \textit{Template} & \textit{Template} & 0.74 \\
GeoQuery & Spider   & \textit{Template} & \textit{TMCD}     & 0.73 \\
GeoQuery & GeoQuery & \textit{Std}      & \textit{Template} & 0.73 \\
SCAN     & SCAN     & \textit{Length}   & \textit{MCD3}     & 0.72 \\
\bottomrule
\end{tabular}
\caption{High concurrence values ($\geq 0.7$) among all pairs of dataset splits, excluding self-concurrence.}
\label{tab:concurrence}
\end{table}




==> CompositionalitySub_arXiv_2/tables/data_examples.tex <==
\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{p{3em}p{4em}p{0.28\textwidth}}
\toprule
\multirow{2}{*}{\textbf{COGS}} & \texttt{Input:} & Mila liked that the cake was offered to Emma . \\
& \texttt{Output:} & \texttt{* cake ( x \_ 4 ) ; like . agent ( x \_ 1 , Mila ) AND like . ccomp ( x \_ 1 , x \_ 6 ) AND offer . theme ( x \_ 6 , x \_ 4 ) AND offer . recipient ( x \_ 6 , Emma )}
\\ \midrule
\multirow{2}{*}{\textbf{SCAN}}  &  \texttt{Input:} & turn left after jump twice \\
 & \texttt{Output:} & \texttt{I\_JUMP I\_JUMP I\_TURN\_LEFT}
\\ \midrule
\multirow{2}{*}{\textbf{GeoQuery }}  &  \texttt{Input:} & how much population does m0 have \\
&  \texttt{Output:} & \texttt{answer ( intersection ( river , loc\_2 ( m0 ) ) )} \\ \midrule
\multirow{2}{*}{\textbf{Spider}}  &  \texttt{Input:} & flight\_1: what is the average distance and price for all flights from la?  \\
&  \texttt{Output:} & \texttt{select avg(distance) , avg(price) from flight where origin = "los angeles"} \\
\bottomrule
\end{tabular}
\caption{Examples of instances in each dataset used in our experiments.}\label{tab:mainexamples}

\end{table}

==> CompositionalitySub_arXiv_2/tables/harmless_error_example.tex <==
\begin{table*}[ht]
\scriptsize
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{p{7em}p{0.8\textwidth}}
\toprule
\textbf{Example 1.}  & BART on GeoQuery \textit{standard} and \textit{template} \\
\textbf{Input:} & what are the highest points of all the states \\
\textbf{Output:} & answer ( highest ( intersection ( place , loc\_2 ( state ) ) ) ) \\
\textbf{Prediction:} & answer ( highest ( intersection ( place , loc\_2 ( state ) ) ) ) \hlc[cyan!50]{)}  \\
\hline
\textbf{Input:} & what is the adjacent state of m0 \\
\textbf{Output:} & answer ( intersection ( state , next\_to\_2 ( m0 ) ) ) \\
\textbf{Prediction:} & answer ( intersection ( state , next\_to\_2 ( m0 ) ) ) \hlc[cyan!50]{)} \\ \midrule
\textbf{Example 2.}  & BTG on GeoQuery \textit{simple} and \textit{TurnLeft} \\
\textbf{Input:} & run left thrice and look opposite right thrice \\
\textbf{Output:} & TURN\_LEFT RUN TURN\_LEFT RUN TURN\_LEFT RUN TURN\_\hlc[cyan!50]{RIGHT} TURN\_\hlc[cyan!50]{RIGHT} LOOK TURN\_\hlc[cyan!50]{RIGHT} TURN\_\hl{RIGHT} LOOK TURN\_\hlc[cyan!50]{RIGHT} TURN\_\hlc[cyan!50]{RIGHT} I\_LOOK \\
\textbf{Prediction:} & TURN\_LEFT RUN TURN\_LEFT RUN TURN\_LEFT RUN TURN\_\hlc[cyan!50]{LEFT} TURN\_\hlc[cyan!50]{LEFT} LOOK TURN\_\hlc[cyan!50]{LEFT} TURN\_\hlc[cyan!50]{LEFT} LOOK TURN\_\hlc[cyan!50]{LEFT} TURN\_\hlc[cyan!50]{LEFT} LOOK \\ \hline
\textbf{Input:} & look right after turn left \\
\textbf{Output:} & TURN\_LEFT TURN\_\hlc[cyan!50]{RIGHT} LOOK \\
\textbf{Prediction:} & TURN\_LEFT TURN\_\hlc[cyan!50]{LEFT} LOOK \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Examples of instance where the model makes both mistakes in random split and generalization split. The first instance is the output of BART on \textit{standard} split of GeoQuery, and the second entry is BART making a similar mistake on \textit{template} split of GeoQuery; the second instance is output of BTG on \textit{simple} split of SCAN, and a similar instance making the same directional mistake on the \textit{TurnLeft} split.}
\label{tab:harmless-example}

\end{table*}

==> CompositionalitySub_arXiv_2/tables/length_split_concurrences.tex <==
\newcommand{\phstar}[0]{\phantom{$^*$}}

\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{llllll}
\toprule
\textbf{Dataset A} & \textbf{Dataset B} & \textbf{Concur} & \textbf{Dataset A} & \textbf{Dataset B} & \textbf{Concur} \\ 
\cmidrule(lr){1-3} \cmidrule(lr){4-6}
COGS      & GeoQuery  & \phstar  0.54  & COGS      & SCAN      & \phstar  0.01  \\
COGS      & Spider    & \phstar  0.26 & SCAN      & Spider    & \phstar  0.01   \\
GeoQuery  & Spider    & \phstar  0.23  & GeoQuery  & SCAN      &  - 0.09  \\
 \bottomrule
\end{tabular}
\caption{Concurrence between length splits of datasets.}
\label{tab:length}
\end{table}



==> CompositionalitySub_arXiv_2/tables/lexical_split.tex <==
\begin{table}[t]
\begin{subtable}[h]{\the\columnwidth}
    \centering
\scriptsize
\begin{tabular}{llll}
\toprule
\textbf{Dataset}          & \textbf{Split A}          & \textbf{Split B} & \textbf{Concur} \\ \midrule
\multirow{4}{*}{GeoQuery} & \multirow{2}{*}{Std}      & Std-Rcvcv        & 0.69            \\
                          &                           & Std-Rstr         & 0.54            \\
                          & \multirow{2}{*}{TMCD}     & TMCD-Rstr        & 0.65            \\
                          &                           & TMCD-Rcvcv       & 0.63            \\ \midrule
\multirow{2}{*}{COGS}     & \multirow{2}{*}{Std}      & RandStr          & 0.60            \\
                          &                           & Randcvcv         & 0.59            \\ \midrule
\multirow{2}{*}{SCAN}     & \multirow{2}{*}{TurnLeft} & TurnLeftRcvcv    & 0.29            \\
                          &                           & TurnLeftRStr     & 0.23 \\ \bottomrule       
\end{tabular}
\caption{Concurrence between the original split and lexically-processed splits.}
\label{tab:sub:lex-concur}
\end{subtable}
\hfill
\begin{subtable}[h]{\the\columnwidth}

\begin{adjustbox}{max width=\columnwidth}
\scriptsize

\begin{tabular}{lllll}
\toprule
\textbf{Dataset A} & \textbf{Split A} & \textbf{Dataset B} & \textbf{Split B} & \textbf{Concur} \\ \midrule
COGS     & \textit{Length}     & GeoQuery & \textit{TMCD-Rcvcv} & 0.84 \\
GeoQuery & \textit{Std-Rcvcv}  & GeoQuery & \textit{TMCD-Rcvcv} & 0.83 \\
COGS     & \textit{Std}        & GeoQuery & \textit{TMCD-Rcvcv} & 0.82 \\
GeoQuery & \textit{TMCD-Rstr}  & Spider   & \textit{Template}   & 0.82 \\
GeoQuery & \textit{TMCD-Rcvcv} & Spider   & \textit{Template}   & 0.81 \\
COGS     & \textit{Length}     & GeoQuery & \textit{TMCD-Rstr}  & 0.81 \\
COGS     & \textit{Length}     & GeoQuery & \textit{Std-Rcvcv}  & 0.8  \\
GeoQuery & \textit{Std-Rcvcv}  & GeoQuery & \textit{TMCD-Rstr}  & 0.8  \\
\textbf{GeoQuery}  & \textit{\textbf{TMCD-Rstr}}  & \textbf{Spider}    & \textit{\textbf{TMCD}} & \textbf{0.79}   \\
\textbf{GeoQuery}  & \textit{\textbf{TMCD-Rcvcv}} & \textbf{Spider}    & \textit{\textbf{TMCD}} & \textbf{0.79}   \\
COGS     & \textit{Std}        & GeoQuery & \textit{Std-Rcvcv}  & 0.78 \\
GeoQuery & \textit{Std}        & GeoQuery & \textit{TMCD-Rstr}  & 0.77 \\
GeoQuery & \textit{Std}        & GeoQuery & \textit{TMCD-Rcvcv} & 0.75 \\
COGS     & \textit{Std}        & GeoQuery & \textit{TMCD-Rstr}  & 0.74 \\
GeoQuery & \textit{Template}   & Spider   & \textit{TMCD}       & 0.73 \\
GeoQuery & \textit{Std-Rcvcv}  & Spider   & \textit{Template}   & 0.73 \\
COGS     & \textit{RandStr}    & GeoQuery & \textit{Std-Rstr}   & 0.73 \\
COGS     & \textit{Std}        & GeoQuery & \textit{Std-Rstr}   & 0.72 \\
GeoQuery & \textit{Std-Rstr}   & GeoQuery & \textit{TMCD-Rcvcv} & 0.71 \\
GeoQuery & \textit{Std-Rcvcv}  & Spider   & \textit{TMCD}       & 0.71 \\
COGS     & \textit{Randcvcv}   & GeoQuery & \textit{Std-Rstr}   & 0.7  \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{High concurrence values after introducing lexically-processed splits, excluding self-concurrence or concurrence between lexically-processed splits that share the same origin.}
\label{tab:sub:lex-high-concur}
\end{subtable}

\caption{Performance and Concurrence between the lexically-processed splits of datasets.}
\label{tab:lexical}
\end{table}

==> CompositionalitySub_arXiv_2/tables/num_instances.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lllllll}
\toprule
\textbf{Dataset} & \textbf{Split}          & \textbf{Train} & \textbf{Validation} & \textbf{Test}  & \textbf{Overall} \\
\midrule
\multirow{4}{*}{COGS}     & no\_mod                  & 24155 & 3000       & 3000  & 21000 & 51155   \\
                          & random\_cvcv             & 24155 & 3000       & 3000  & 21000 & 51155   \\
                          & random\_str              & 24155 & 3000       & 3000  & 21000 & 51155   \\
                          & length                   & 24156 & -          & 23999 & -     & 48155   \\
                          \midrule
\multirow{4}{*}{GeoQuery} & standard                 & 600   & -          & 280   & -     & 880     \\
                          & length                   & 440   & -          & 440   & -     & 880     \\
                          & template                 & 441   & -          & 439   & -     & 880     \\
                          & tmcd                     & 440   & -          & 440   & -     & 880     \\
                          \midrule
\multirow{11}{*}{SCAN}    & simple                   & 16728 & -          & 4182  & -     & 20910   \\
                          & length                   & 16990 & -          & 3920  & -     & 20910   \\
                          & mcd1                     & 8365  & 1045       & 1045  & -     & 10455   \\
                          & mcd2                     & 8365  & 1045       & 1045  & -     & 10455   \\
                          & mcd3                     & 8365  & 1045       & 1045  & -     & 10455   \\
                          & addprim\_jump            & 14670 & -          & 7706  & -     & 22376   \\
                          & addprim\_turn\_left      & 21890 & -          & 1208  & -     & 23098   \\
                          & jump\_random\_cvcv       & 14670 & -          & 7706  & -     & 22376   \\
                          & jump\_random\_str        & 14670 & -          & 7706  & -     & 22376   \\
                          & turn\_left\_random\_cvcv & 21890 & -          & 1208  & -     & 23098   \\
                          & turn\_left\_random\_str  & 21890 & -          & 1208  & -     & 23098   \\
                          \midrule
\multirow{4}{*}{Spider}   & random                   & 3282  & -          & 1094  & -     & 4376    \\
                          & length                   & 3282  & -          & 1094  & -     & 4376    \\
                          & template                 & 3280  & -          & 1096  & -     & 4376    \\
                          & tmcd                     & 3282  & -          & 1094  & -     & 4376    \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Number of instances for each dataset in each optimization split.}
\label{tab:num_instances}
\end{table*}

==> CompositionalitySub_arXiv_2/tables/perf_difference.tex <==
\begin{table}[H]
\scriptsize
\centering
\begin{tabular}{llrrr}
\toprule
\textbf{Dataset}      & \textbf{Split}    & \multicolumn{1}{l}{\textbf{T5}} & \multicolumn{1}{l}{\textbf{BART}} & \multicolumn{1}{l}{\textbf{BTG}} \\ \midrule
\multirow{7}{*}{COGS} & \textit{Std-Test} & 99.7                            & 0.0                               & 0.0                              \\
                          & \textit{Std-Gen}    & 82.9 & 0.0  & 0.0  \\
                          & \textit{Rcvcv-Test} & 99.7 & 0.0  & 0.0  \\
                          & \textit{Rstr-Test}  & 99.8 & 0.0  & 0.0  \\
                          & \textit{Rcvcv-Gen}  & 50.0 & 0.0  & 0.0  \\
                          & \textit{Rstr-Gen}   & 48.0 & 0.0  & 0.0  \\
                          & \textit{Length}     & 37.9 & 0.0  & 0.0  \\ \midrule
\multirow{4}{*}{Spider}   & Rand                & 60.1 & 26.2 & 32.4 \\
                          & Template            & 34.9 & 18.1 & 1.8  \\
                          & TMCD                & 38.3 & 23.5 & 4.9  \\
                          & Length              & 33.9 & 6.1  & 11.9 \\ \midrule
\multirow{8}{*}{GeoQuery} & Std                 & 77.1 & 0.0  & 0.0  \\
                          & Std-Rcvcv           & 74.3 & 0.0  & 0.0  \\
                          & Std-Rstr            & 73.5 & 0.0  & 0.0  \\
                          & Template            & 76.5 & 0.0  & 0.0  \\
                          & Length              & 39.5 & 0.0  & 0.0  \\
                          & TMCD                & 40.7 & 0.0  & 0.0  \\
                          & TMCD-Rcvcv          & 31.6 & 0.0  & 0.0  \\
                          & TMCD-Rstr           & 31.4 & 0.0  & 0.0  \\ \bottomrule
\end{tabular}
\caption{Percentage difference between raw EM implementation and EM implementation that ignore harmless space (space-lenient EM - raw EM). SCAN and NACS are omitted because models do not have this issue on them. LSTMs do not display this issue; the difference for Transformer is under 0.1\% for each datset.}
\label{tab:perf_difference}
\end{table}

==> CompositionalitySub_arXiv_2/tables/perf_table_v2.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{clrlrlrlrlrlrlr}
\toprule
\textbf{Dataset} &
  \textbf{Split} &
  \multicolumn{2}{c}{\textbf{LSTM Uni}} &
  \multicolumn{2}{c}{\textbf{LSTM Bi}} &
  \multicolumn{2}{c}{\textbf{Transformer}} &
  \multicolumn{2}{c}{\textbf{T5}} &
  \multicolumn{2}{c}{\textbf{BART}} &
  \multicolumn{2}{c}{\textbf{BTG}} &
  \multicolumn{1}{c}{\textbf{Avg}} \\ \midrule
\multirow{2}{*}{COGS}     & \textit{Std-Test} & 99.3 & ±.0  & 99.1 & ±.01 & 99.5  & ±.0  & 99.7 & ±.0  & 99.7 & ±.0  & 68.8 & ±.01 & 94.3 \\
                          & \textit{Std-Gen}  & 21.3 & ±.05 & 14.8 & ±.08 & 56.1  & ±.06 & 82.9 & ±.0  & 78.6 & ±.0  & 2.8  & ±.01 & 42.8 \\ \midrule
\multirow{8}{*}{SCAN}     & \textit{Simple}   & 99.9 & ±.0  & 99.9 & ±.0  & 100.0 & ±.0  & 94.9 & ±.01 & 99.1 & ±.01 & 12.3 & ±.01 & 84.4 \\
                          & \textit{Jump}     & 0.4  & ±.01 & 0.0  & ±.0  & 0.1   & ±.0  & 95.0 & ±.01 & 0.4  & ±.01 & 0.0  & ±.0  & 16.0 \\
                          & \textit{TurnLeft} & 61.1 & ±.13 & 34.1 & ±.06 & 64.8  & ±.11 & 70.3 & ±.12 & 63.1 & ±.19 & 8.9  & ±.01 & 50.4 \\
                          & \textit{Template} & 0.2  & ±.0  & 0.3  & ±.01 & 1.1   & ±.0  & 34.3 & ±.03 & 0.0  & ±.0  & 0.9  & ±.01 & 6.1  \\
                          & \textit{MCD1}     & 5.9  & ±.06 & 12.2 & ±.07 & 1.1   & ±.0  & 24.6 & ±.01 & 0.4  & ±.01 & 1.8  & ±.01 & 7.7  \\
                          & \textit{MCD2}     & 6.7  & ±.03 & 5.8  & ±.03 & 1.2   & ±.0  & 34.1 & ±.01 & 1.6  & ±.0  & 0.5  & ±.0  & 8.3  \\
                          & \textit{MCD3}     & 8.7  & ±.04 & 7.8  & ±.02 & 0.7   & ±.0  & 11.1 & ±.01 & 1.2  & ±.01 & 0.8  & ±.01 & 5.0  \\
                          & \textit{Length}   & 15.3 & ±.04 & 11.8 & ±.01 & 0.0   & ±.0  & 14.1 & ±.01 & 0.7  & ±.01 & 0.0  & ±.0  & 7.0  \\ \midrule
\multirow{4}{*}{GeoQuery} & \textit{Std}      & 74.0 & ±.06 & 78.9 & ±.04 & 82.3  & ±.02 & 92.5 & ±.01 & 89.2 & ±.01 & 79.0 & ±.01 & 82.6 \\
                          & \textit{Template} & 46.5 & ±.06 & 55.9 & ±.07 & 56.7  & ±.04 & 91.0 & ±.0  & 77.1 & ±.06 & 53.5 & ±.06 & 63.5 \\
                          & \textit{TMCD}     & 35.8 & ±.02 & 37.1 & ±.02 & 37.9  & ±.01 & 54.1 & ±.0  & 48.2 & ±.0  & 36.9 & ±.0  & 41.7 \\
                          & \textit{Length}   & 18.5 & ±.03 & 16.2 & ±.02 & 22.0  & ±.01 & 41.1 & ±.01 & 36.1 & ±.01 & 20.7 & ±.02 & 25.8 \\ \midrule
\multirow{4}{*}{Spider}   & \textit{Rand}     & 33.4 & ±.02 & 36.9 & ±.01 & 42.5  & ±.01 & 68.0 & ±.0  & 32.7 & ±.01 & 40.1 & ±.01 & 42.3 \\
                          & \textit{Template} & 1.0  & ±.0  & 2.2  & ±.01 & 4.6   & ±.0  & 39.6 & ±.01 & 21.6 & ±.01 & 1.9  & ±.0  & 11.8 \\
                          & \textit{TMCD}     & 4.6  & ±.01 & 6.0  & ±.01 & 7.5   & ±.01 & 47.2 & ±.01 & 31.2 & ±.03 & 5.5  & ±.0  & 17.0 \\
                          & \textit{Length}   & 12.7 & ±.01 & 14.0 & ±.01 & 17.5  & ±.01 & 35.4 & ±.01 & 7.4  & ±.0  & 14.0 & ±.01 & 16.8
 \\
                        \bottomrule
\end{tabular}
\end{adjustbox}
    \caption{Model exact-match accuracy on datasets averaged across random seeds, with standard deviation.}%
\label{tab:perfStd}
\end{table*}




==> CompositionalitySub_arXiv_2/tables/space_example.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{p{7em}p{0.8\textwidth}}
\toprule
\textbf{Input:} & Zoe thought that a hippo cleaned . \\
\textbf{Output:} & think\hl{ }. agent ( x \_ 1\hl{ }, Zoe ) AND think\hl{ }. ccomp ( x \_ 1\hl{ }, x \_ 5 ) AND hippo ( x \_ 4 ) AND clean\hl{ }. agent ( x \_ 5\hl{ }, x \_ 4 ) \\
\textbf{Prediction:} & think. agent ( x \_ 1, Zoe ) AND think. ccomp ( x \_ 1, x \_ 5 ) AND hippo ( x \_ 4 ) AND clean. agent ( x \_ 5, x \_ 4 ) \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Examples of instance where the model is only mistaken on the space.}
\label{tab:space-example}

\end{table*}

==> Results/6_Eval_Metric.tex <==



Despite of data source and exposed lexical items, other confounding factors can appear during the evaluation of compositionality.
As we have observed in \cref{fig:default_conf_matrix}, splits of SCAN obtain low concurrence with most of splits from other datasets.
In the mean time, the task of SCAN, grounded navigation, is most distant from the others, which are based on semantic parsing.
This and our finding in \cref{sec:comp_def} are \textit{in pari materia}: the source of data (regardless of the task) contributes more to the resulting model rankings compared to the interpretation of generalization, and gives hints about the degree to which datasets disagree with each other when considering two more distant pairs of datasets in terms of their task.
We leave the investigation on how the selection of specific tasks affect evaluation result of compositionality to further research.

The in-distribution performance may also become a confounder when model performs poorly on the random split of the data.
Qualitatively, we observe that models sometimes make the same trivial mistakes in both a random split and a generalization split, making the evaluation result unrepresentative of compositionality.
We leave such examples in \cref{app:sec:mistakes}.





==> figures/app_NACS/perf_vs_concur.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.85\columnwidth]{figures/app_NACS/perf_vs_concur_app.pdf}
\caption{Values of concurrences with respect to pairwise averaged performance among the splits shown in \cref{app:tab:nacs-all-perf}. The color of dots indicates the type of split pairs. The triangle-shape dots indicates the values of self-concurrence.}
\label{fig:perfvconcur}
\end{figure}
